Representation of Universal Algebra

Theory of representations of universal algebra is a natural development of the theory of universal algebra. Morphism of the representation is the map that conserve the structure of the representation. Exploring of morphisms of the representation leads to the concepts of generating set and basis of representation. In the book I considered the notion of tower of representations of $F_i$-algebras, i=1 ..., n, as the set of coordinated representations of $F_i$-algebras.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Doctor Ouch}
{
Корней Чуковский. Айболит.
\\
Детский мир, ISBN 978-5-91315-875-8, 2012
}%

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau I}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, механика,
М., Наука, 1988
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 3}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $3$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники. ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная универсальная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts{T}представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1111.6035}
{
Александр Клейн,
Базис представления универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/1111.6035}{arXiv:1111.6035} (2011)
}%

\BiblioItem{1201.4158}
{
Александр Клейн, Александер Ложье,
Ортонормированный базис в пространстве Минковского,\\
eprint \href{http://arxiv.org/abs/1201.4158}{arXiv:1201.4158} (2012)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1206.0200}
{
Александр Клейн,
Алгебра частных алгебры с сопряжением,\\
eprint \href{http://arxiv.org/abs/1206.0200}{arXiv:1206.0200} (2012)
}

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\BiblioItem{1302.7204}
{
Александр Клейн,
Многочлен над ассоциативной $D$-алгеброй,\\
eprint \href{http://arxiv.org/abs/1302.7204}{arXiv:1302.7204} (2013)
}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Александр Клейн,
Интеграл отображения в абелевую $\Omega$\Hyph группу,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Александр Клейн.\\
Линейная алгебра над телом: Система линейных уравнений.\\
CreateSpace Independent Publishing Platform, 2014; ISBN-13: 978-1502982476
}%

\BiblioItem{4993-2400}
{
Александр Клейн.\\
Линейная алгебра над телом: Векторное пространство.\\
CreateSpace Independent Publishing Platform, 2014; ISBN-13: 978-1499323948
}%

\BiblioItem{5059-9176}
{
Александр Клейн.\\
Нормированная \(\Omega\)-группа.\\
CreateSpace Independent Publishing Platform, 2015; ISBN-13: 978-1505992359
}%

\BiblioItem{AlgebraE}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2014
}%

\BiblioItem{RepresentationE}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2014
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
Vol 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{CACAA.02.97}
{
Aleks Kleyn,
Polynomial over Associative $D$-Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
Vol 2, Issue 2, pages 97 - 115, 2013
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010).
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008).
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\BiblioItem
{Cohn: Skew Fields}
{
Paul M. Cohn,
Skew Fields,
Cambridge University Press, 1995
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 3,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Convention.Russian.tex <==
%auto-ignore
\input{\FilePrefix Convention.Eq}

\section{Соглашения}

\ePrints{0812.4763,0906.0135,0908.3307,0909.0855,0912.3315,1003.1544}
\Items{1006.2597,AlgebraE}
\ifx\Semafor\ValueOn
\begin{convention}
Функция и отображение - синонимы. Однако существует
традиция соответствие между кольцами или векторными
пространствами называть отображением, а отображение
поля действительных чисел или алгебры кватернионов называть функцией.
Я тоже следую этой традиции,
хотя встречается текст, в котором неясно, какому термину надо
отдать предпочтение.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1001.4852}
\Items{1003.1544,4776-3181,AlgebraE}
\ifx\Semafor\ValueOn
\begin{convention}
В любом выражении, где появляется индекс, я предполагаю,
что этот индекс может иметь внутреннюю структуру.
Например, при рассмотрении алгебры $A$ координаты $a\in A$
относительно базиса $\Basis e$ пронумерованы индексом $i$.
Это означает, что $a$ является вектором. Однако, если $a$
является матрицей, нам необходимо два индекса, один нумерует
строки, другой - столбцы. В том случае, когда мы уточняем структуру
индекса, мы будем начинать индекс с символа $\cdot$ в соответствующей
позиции.
Например, если я рассматриваю матрицу $a^i_j$ как элемент векторного
пространства, то я могу записать элемент матрицы в виде $a^{\cdot}{}^i_j$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1006.2597,1011.3102}
\Items{1211.6965,4910-5816,GJSFRF.Basis,1302.7204,CACAA.02.97}
\Items{4993-2400}
\ifx\Semafor\ValueOn
\begin{convention}
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $s$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855}
\ifx\Semafor\ValueOn
\begin{convention}
Тело $D$ можно рассматривать как $D$\Hyph векторное пространство
размерности $1$. Соответственно этому, мы можем изучать не только
гомоморфизм тела $D_1$ в тело $D_2$, но и линейное отображение тел.
\qed
\end{convention}
\fi

\ePrints{0912.4061}
\ifx\Semafor\ValueOn
\begin{convention}
Для данного поля $F$, если не оговорено противное,
мы будем рассматривать конечномерную $F$\Hyph алгебру.
%без делителей нуля.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
Несмотря на некоммутативность произведения многие утверждения
сохраняются, если заменить например правое представление на
левое представление или правое векторное пространство на левое
векторное пространство.
Чтобы сохранить эту симметрию в формулировках теорем
я пользуюсь симметричными обозначениями.
Например, я рассматриваю \Ds векторное пространство
и \sD векторное пространство.
Запись \Ds векторное пространство можно прочесть
как D\Hyph star\Hyph векторное пространство либо
как левое векторное пространство.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,1211.6965,4910-5816,CACAA.01.195,GJSFRF.Basis,1302.7204}
\Items{CACAA.02.97,4993-2400,AlgebraE}
\ifx\Semafor\ValueOn
\begin{convention}
\label{convention: we use separate color for index of element}
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,GJSFRF.Basis,1302.7204,CACAA.02.97}
\ifx\Semafor\ValueOn
\begin{convention}
%\label{convention: }
Очень трудно провести границу между модулем и алгеброй.
Тем более, иногда в процессе построения мы должны сперва
доказать, что множество $A$ является модулем,
а потом мы доказываем, что это множество является алгеброй.
Поэтому для записи координат элемента модуля
мы также будем пользоваться соглашением
\ref{convention: we use separate color for index of element}.
\qed
\end{convention}
\fi

\ePrints{1302.7204,CACAA.02.97,1310.5591,MSimplex,MBasis,1412.5425,AlgebraE}
\Items{MLinear}
\ifx\Semafor\ValueOn
\begin{convention}
Элемент
$\Omega$\Hyph алгебры
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
\qed
\end{convention}
\fi

\ePrints{MLinear,1305.4547,5059-9176}
\ifx\Semafor\ValueOn
\begin{convention}
Я обозначаю
\ShowEq{set of n-ary operations}
множество $n$\Hyph арных операций $\Omega$\Hyph алгебры.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,4993-2400}
\ifx\Semafor\ValueOn
\begin{convention}
Отождествление вектора и матрицы его координат
может привести к неоднозначности в равенстве
\ShowEq{Identification can lead to ambiguity, 1}
где $\Basis e$ - базис векторного пространства.
Поэтому мы будем записывать равенство
\EqRef{Identification can lead to ambiguity, 1}
в виде
\ShowEq{Identification can lead to ambiguity, 2}
чтобы видеть, где записан вектор.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,CACAA.01.195,AlgebraE}
\ifx\Semafor\ValueOn
\begin{convention}
Если свободная конечномерная алгебра имеет единицу,
то мы будем отождествлять
вектор базиса $\Vector e_{\gi 0}$ с единицей алгебры.
\qed
\end{convention}
\fi

\ePrints{1104.5197,1105.4307}
\ifx\Semafor\ValueOn
\begin{convention}
Хотя алгебра является свободным модулем над некоторым
кольцом, мы не пользуемся векторными обозначениями
при записи элементов алгебры. В тех случаях, когда я рассматриваю
матрицу координат элемента алгебры, я буду пользоваться векторными
обозначениями для записи соответствующего элемента.
Чтобы не возникала неоднозначность при записи сопряжения,
я буду обозначать $a^*$ элемент, сопряжённый элементу $a$.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072,RepresentationE}
\ifx\Semafor\ValueOn
\begin{convention}
Так как число универсальных алгебр в башне представлений переменно,
то мы будем пользоваться векторными обозначениями для башни
представлений. Множество
$(A_1,...,A_n)$ $\Omega_i$\Hyph алгебр $A_i$, $i=1$, ..., $n$
мы будем обозначать $\Vector A$. Множество представлений
$(f_{1,2},...,f_{n-1,n})$ этих алгебр мы будем обозначать $\Vector f$.
Так как разные алгебры имеют разный тип, мы также
будем говорить о множестве $\Vector{\Omega}$\Hyph алгебр.
\ePrints{8443-0072,RepresentationE}
\ifx\Semafor\ValueOn
Символом
\else
По отношению к множеству $\Vector A$
мы также будем пользоваться матричными обозначениями, предложенными
в разделе \xRef{0701.238}{section: Concept of Generalized Index}.
Например, символом
\fi
$\Vector A_{[1]}$ мы будем обозначать
множество $\Vector{\Omega}$\Hyph алгебр $(A_2,...,A_n)$.
В соответствующем обозначении $(\VX A,\Vector f)$ башни
представлений подразумевается, что $\Vector f=(f_{2,3},...,f_{n-1,n})$.
\qed
\end{convention}

\begin{convention}
Так как мы пользуемся векторными обозначениями для элементов
башни представлений, необходимо соглашение о записи операций.
Предполагается, что операции выполняются покомпонентно. Например,
\ShowEq{vector notation in tower of representations}
\qed
\end{convention}
\fi

\ePrints{8443-0072,1111.6035,0906.0135,NewAffine,1102.5168,1305.4547,1310.5591}
\Items{1003.3714,4820-2669,MBasis,4993-2400,1412.5425,5059-9176}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть $A$ - $\Omega_1$\Hyph алгебра.
Пусть $B$ - $\Omega_2$\Hyph алгебра.
Запись
\ShowEq{A->*B}
означает, что определено представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
\qed
\end{convention}
\fi

\ePrints{0702.561,0707.2246,0803.2620}
\ifx\Semafor\ValueOn
\begin{convention}
Я пользуюсь стрелкой $\xymatrix{\arp[r]&}$
на диаграмме для обозначения проекции расслоения.
Я пользуюсь стрелкой $\xymatrix{\ars[r]&}$
на диаграмме для обозначения сечения расслоения.
\qed
\end{convention}
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\begin{remark}
Я считаю диаграммы отображений важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я рассказывал своим коллегам
какие преимущества имеет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.
\qed
\end{remark}
\fi

\ePrints{1001.4852,1003.1544,1006.2597,1011.3102}
\Items{AlgebraE}
\ifx\Semafor\ValueOn
\begin{convention}
Если в некотором выражении используется несколько
операций, среди которых есть операция $\circ$, то предполагается,
что операция $\circ$ выполняется первой.
Ниже приведен пример эквивалентных выражений.
\ShowEq{list circ expressions}
\qed
\end{convention}
\fi

%\ePrints{0906.0135,NewAffine}
%\ifx\Semafor\ValueOn
%\item
%Пусть $\VX X$ - базис башни представлений $(\Vector A,\Vector f)$.
%Мы будем называть $\Omega_n$\Hyph слово
%$w_n(\Vector f,\VX X,x_n)$ координатами $x_n\in A_n$
%относительно базиса $\VX X$.
%\fi

\ePrints{1107.1139}
\ifx\Semafor\ValueOn
\begin{convention}
Для данной $D$\Hyph алгебры $A$
левый сдвиг
\ShowEq{left shift, D algebra}
определён равенством
\ShowEq{left shift 1, D algebra}
и правый сдвиг
\ShowEq{right shift, D algebra}
определён равенством
\ShowEq{right shift 1, D algebra}
\qed
\end{convention}
\fi

\ePrints{1412.5425}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть $A$ ассоциативная $D$\Hyph алгебра.
Представление
\ShowEq{A2->*A}
$D$\Hyph модуля
\ShowEq{A2}
порождает множество линейных отображений.
Это представление порождает произведение $\circ$ в $D$\Hyph модуле
\ShowEq{A2}
согласно правилу
\ShowEq{(pq)a=p(qa)}
\qed
\end{convention}
\fi

\ePrints{MBasis}
\ifx\Semafor\ValueOn
\begin{convention}
Мы будем полагать,
что рассматриваемая мера является полной мерой.
\qed
\end{convention}
\fi

\ifx\PrintPaper\undefined
%Без сомнения, у читателя могут быть вопросы,
%замечания, возражения. Я буду признателен любому отзыву.
\fi



==> Group.Representation.Russian.tex <==
%auto-ignore
\input{Group.Representation.Eq}
\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\chapter{Представление группы}
\label{chapter: Representation of Group}
\fi

\section{Представление группы}
\label{section: Representation of Group}

Группа - одна из немногих алгебр, которая позволяет рассматривать
произведение преобразований $\Omega$\Hyph алгебры $M$ таким образом, что если
преобразования принадлежат представлению, то их произведение также
принадлежит представлению.
При этом следует помнить, что порядок отображений при суперпозиции
зависит от порядка отображений на диаграмме и с какой стороны
отображения действуют на элементы множества.

\begin{definition}
\label{definition: left-side representation of group} 
Пусть ${}^*M$ - группа с произведением
\ShowEq{fg *M Tstar}
и $\delta$ - единица группы ${}^\star M$.
Пусть $G$ - группа.
Мы будем называть гомоморфизм групп
\ShowEq{left-side representation of group, map}
\AddIndex{левосторонним представлением группы $G$}{left-side representation of group}
или
\AddIndex{\Ts{G}представлением группы}{A* representation of algebra}
в $\Omega$\Hyph алгебре $M$, если отображение $f$ удовлетворяет условиям
\ShowEq{left-side representation of group}
\qed
\end{definition}

\begin{remark}
Поскольку отображение \EqRef{left-side representation of group, map}
- гомоморфизм, то
\ShowEq{left-side representation of group, map product}
Мы здесь пользуемся соглашением
\[
f(a)f(b)=f(a)\circ f(b)
\]
Таким образом, концепция представления групп состоит в том,
что в каком порядке мы перемножаем элементы группы,
в том же порядке перемножаются соответствующие преобразования представления.
Из равенств \EqRef{left-side representation of group}
и \EqRef{left-side representation of group, map product}
следует
\ShowEq{left-side representation of group, associativity}
Равенство
\EqRef{left-side representation of group, associativity}
совместно с ассоциативностью произведения преобразований
представляет собой
\AddIndex{закон ассоциативности}{associative law}
для \Ts{G}представления.
Это позволяет записывать равенство
\EqRef{left-side representation of group, associativity}
без использования скобок
\[
f(ab)u=f(a)f(b)u
\]
\qed
\end{remark}

\begin{definition}
\label{definition: right-side representation of group} 
Пусть $M^\star$ - группа с произведением
\ShowEq{fg *M starT}
и $\delta$ - единица группы $M^\star$.
Пусть $G$ - группа.
Мы будем называть гомоморфизм групп
\ShowEq{right-side representation of group, map}
\AddIndex{правосторонним представлением группы $G$}{right-side representation of group}
или
\AddIndex{\sT{G}представлением}{*A representation of algebra}
в $\Omega$\Hyph алгебре $M$, если отображение $f$ удовлетворяет условиям
\ShowEq{right-side representation of group}
\qed
\end{definition}

\begin{remark}
Поскольку отображение \EqRef{right-side representation of group, map}
- гомоморфизм, то
\ShowEq{right-side representation of group, map product}
Из равенств \EqRef{right-side representation of group}
и \EqRef{right-side representation of group, map product}
следует
\ShowEq{right-side representation of group, associativity}
Равенство
\EqRef{right-side representation of group, associativity}
совместно с ассоциативностью произведения преобразований
представляет собой
\AddIndex{закон ассоциативности}{associative law}
для \sT{G}представления.
Это позволяет записывать равенство
\EqRef{right-side representation of group, associativity}
без использования скобок
\[
uf(ab)=uf(a)f(b)
\]
\qed
\end{remark}

\begin{definition}
\label{definition: nonsingular transformation} 
Мы будем называть преобразование
\[
t:M\rightarrow M
\]
\AddIndex{невырожденным преобразованием}{nonsingular transformation},
если существует обратное отображение.
\qed
\end{definition}

\begin{theorem}
\label{theorem: inverse transformation}
Для любого $g\in G$ преобразование $f(g)$ является
невырожденным и удовлетворяет равенству
\begin{equation}
\EqLabel{inverse transformation}
f(g^{-1})=f(g)^{-1}
\end{equation}
\end{theorem}
\begin{proof}
На основании \EqRef{left-side representation of group} и
\ShowEq{f(e)=}
мы можем записать
\[
u=\delta (u)=f(gg^{-1})(u)=f(g)(f(g^{-1})(u))
\]
Это завершает доказательство.
\end{proof}

\begin{theorem}
Групповая операция определяет два различных представления на группе:
\begin{itemize}
\item
\AddIndex{Левый сдвиг}{left shift}
\ShowEq{left shift =}
\ShowEq{left shift}
является \Ts{G}представлением на множестве\footnote{Левый сдвиг
не является представлением группы в группе,
так как преобразование $t_\star$ не является гомоморфизмом
группы.
Аналогичное замечание верно для правого сдвига.
} $G$
\ShowEq{left shift, product}
\item
\AddIndex{Правый сдвиг}{right shift}
\ShowEq{right shift =}
\ShowEq{right shift}
является \sT{G}представлением на множестве $G$
\ShowEq{right shift, product}
\end{itemize}
\end{theorem}
\begin{proof}
Равенство \EqRef{left shift, product}
следует из ассоциативности произведения
\[
t_\star(ab)c=(ab)c=a(bc)=t_\star(a)(t_\star(b)c)
=(t_\star(a)\circ t_\star(b))c
\]
Аналогично доказывается равенство \EqRef{right shift, product}.
\end{proof}

\begin{definition}
\label{definition: orbit of left-side representation of group}
Пусть $G$ - группа.
Пусть $f$ - \Ts{G}представление в $\Omega$\Hyph алгебре $M$.
Для любого $v\in M$ мы определим
\AddIndex{орбиту представления группы $G$}
{orbit of representation of group} как множество
\ShowEq{orbit of representation of group}
\qed
\end{definition}

Так как $f(e)=\delta$, то $v\in f(G)v$.

\begin{theorem}
\label{theorem: proper definition of orbit}
Если
\begin{equation}
\EqLabel{orbit, proposition}
v\in f(G)u
\end{equation}
то
\[
f(G)u=f(G)v
\]
\end{theorem}
\begin{proof}
Из \EqRef{orbit, proposition} следует
существование $a\in G$ такого, что
\begin{equation}
v=f(a)u
\EqLabel{orbit, 1}
\end{equation}
Если $w\in f(G)v$, то
существует $b\in G$ такой, что
\begin{equation}
w=f(b)v
\EqLabel{orbit, 2}
\end{equation}
Подставив \EqRef{orbit, 1} в \EqRef{orbit, 2}, мы получим
\begin{equation}
w=f(b)(f(a)u)
\EqLabel{orbit, 3}
\end{equation}
На основании \EqRef{left-side representation of group}
из \EqRef{orbit, 3} следует,
что $w\in f(G)u$.
Таким образом,
\[
f(G)v\subseteq f(G)u
\]

На основании \EqRef{inverse transformation}
из \EqRef{orbit, 1} следует,
что
\begin{equation}
u=f(a)^{-1}v=f(a^{-1})v
\EqLabel{orbit, 4}
\end{equation}
Равенство \EqRef{orbit, 4} означает, что
$u\in f(G)v$ и, следовательно,
\[
f(G)u\subseteq f(G)v
\]
Это завершает доказательство.
\end{proof}

Таким образом, \Ts{G}представление $f$ в $\Omega$\Hyph алгебре $M$
порождает отношение эквивалентности $S$ и
орбита $f(G)u$ является классом эквивалентности.
Мы будем пользоваться обозначением
\symb{M/f(G)}{space of orbits of G* representation}1
для фактор множества $M/S$ и мы будем называть
это множество
\AddIndex{пространством орбит \Ts{G}представления}
{space of orbits of G* representation} $f$.

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: direct product of representations}
Если определены \Ts{G}представление $f_1$ в $\Omega$\Hyph алгебре $M_1$
и \Ts{G}представление $f_2$ в $\Omega$\Hyph алгебре $M_2$,
то мы можем определить
\AddIndex{прямое произведение \Ts{G}представлений}
{direct product of G* representations}
$f_1$ и $f_2$ группы
\begin{align*}
f&=f_1\times f_2:G\rightarrow M_1\otimes M_2\\
f(g)&=(f_1(g),f_2(g))
\end{align*}
\end{theorem}
\begin{proof}
Чтобы показать, что $f$ является представлением,
достаточно показать, что $f$ удовлетворяет определению
\ref{definition: left-side representation of group}.
\[f(e)=(f_1(e),f_2(e))=(\delta_1,\delta_2)=\delta\]
\begin{align*}
f(ab)u&=(f_1(ab)u_1,f_2(ab)u_2)\\
&=(f_1(a)(f_1(b)u_1),f_2(a)(f_2(b)u_2))\\
&=f(a)(f_1(b)u_1,f_2(b)u_2)\\
&=f(a)(f(b)u)
\end{align*}
\end{proof}
\fi

\section{Однотранзитивное правостороннее представление группы}
\label{section: Single Transitive Representation of Group}

\begin{definition}
\label{definition: kernel of inefficiency of representation of group}
Мы будем называть
\AddIndex{ядром неэффективности \Ts{G}представления}
{kernel of inefficiency of G* representation}
множество \[K_f=\{g\in G:f(g)=\delta\}\]
\qed
\end{definition}

\begin{theorem}
\label{theorem: kernel of inefficiency, representation of group}
Ядро неэффективности \Ts{G}представления - это подгруппа группы $G$.
\end{theorem}
\begin{proof}
Допустим
$f(a_1)=\delta$ и $f(a_2)=\delta$. Тогда
\[f(a_1a_2)u=f(a_1)(f(a_2)u)=u\]
\[f(a^{-1})=f^{-1}(a)=\delta\]
\end{proof}

\begin{theorem}
\Ts{G}представление
\AddIndex{эффективно}{effective G* representation}
тогда и только тогда, когда ядро неэффективности $K_f=\{e\}$.
\end{theorem}
\begin{proof}
Утверждение является следствием определений
\ref{definition: effective representation of algebra} и
\ref{definition: kernel of inefficiency of representation of group} и
теоремы \ref{theorem: kernel of inefficiency, representation of group}.
\end{proof}

Если действие не эффективно, мы можем перейти к эффективному
заменив группой $G_1=G|K_f$,
пользуясь факторизацией по ядру неэффективности.
Это означает, что мы можем изучать только эффективное действие.

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{definition}
\label{definition: free representation of group}
Рассмотрим \Ts{G}представление $f$ в $\Omega$\Hyph алгебре $M$.
\AddIndex{Малая группа}{little group} или
\AddIndex{группа стабилизации}{stability group} элемента $x\in M$ -
это множество
\ShowEq{little group}

Мы будем называть \Ts{G}представление $f$
\AddIndex{свободным}{free representation of group},
если для любого $x\in M$ группа стабилизации $G_x=\{e\}$.
\qed
\end{definition}

\begin{theorem}%
\label{theorem: free representation of group}
Если определено свободное \Ts{G}представление $f$ группы $G$ на $\Omega$\Hyph алгебре $A$,
то определено взаимно однозначное соответствие между орбитами представления,
а также между орбитой представления и группой $G$.
\end{theorem}
\begin{proof}
Допустим для точки $a\in A$
существуют $g_1$, $g_2\in G$
\begin{equation}
\EqLabel{free representation of group, 1}
f(g_1)a=f(g_2)a
\end{equation}
Умножим обе части равенства \EqRef{free representation of group, 1}
на $f(g_1^{-1})$
\[
a=f(g_1^{-1})f(g_2)a
\]
Поскольку представление свободное, $g_1=g_2$. Теорема доказана,
так как мы установили взаимно однозначное соответствие между
орбитой и группой $G$.
\end{proof}
\else

\begin{definition}
\label{definition: transitive representation of group}
Мы будем называть представление группы
\AddIndex{транзитивным}{transitive representation of group},
если для любых $a, b \in V$ существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление группы
\AddIndex{однотранзитивным}{single transitive representation of group},
если оно транзитивно и эффективно.
\qed
\end{definition}

\begin{theorem}%однотранзитивное
\Ts{G}представление однотранзитивно тогда и только тогда, когда для любых $a, b \in M$
существует одно и только одно $g\in G$ такое, что $a=f(g)(b)$
\end{theorem}
\begin{proof}
Следствие определений \ref{definition: effective representation of algebra}
и \ref{definition: transitive representation of group}.
\end{proof}
\fi

\begin{definition}
Мы будем называть пространство $V$
\AddIndex{однородным пространством группы}{homogeneous space of group} $G$,
если мы имеем однотранзитивное \Ts{G}представление на $V$.
\qed
\end{definition}

\begin{theorem}%
\label{theorem: single transitive representation of group}
Если мы определим однотранзитивное
представление $f$ группы $G$ на $\Omega$\Hyph алгебре $A$,
то мы можем однозначно определить координаты на $A$, пользуясь координатами на группе $G$.

Если $f$ - левостороннее представление,
то $f(a)$ эквивалентно левому сдвигу $t_\star(a)$ на группе $G$.
Если $f$ - правостороннее представление, то $f(a)$ эквивалентно
правому сдвигу ${}_\star t(a)$ на группе $G$.
\end{theorem}
\begin{proof}
Мы выберем точку $v\in A$
и определим координаты точки $w\in A$
как координаты $a\in G$ такого, что $w=f(a) v$.
Координаты, определённые таким образом, однозначны
с точностью до выбора начальной точки $v\in A$,
так как действие эффективно.

Если $f$ - левостороннее представление,
мы будем пользоваться записью
\[f(a)v=av\]
Так как запись
\[f(a)(f(b)v)=a(bv)=(ab)v=f(ab)v\]
совместима с групповой структурой, мы видим, что
левостороннее представление $f$ эквивалентно левому сдвигу.

Если $f$ - правостороннее представление,
мы будем пользоваться записью
\[vf(a)=va\]
Так как запись
\[(vf(b))f(a)=(vb)a=v(ba)=vf(ba)\]
совместима с групповой структурой, мы видим, что
правостороннее представление $f$ эквивалентно правому сдвигу.
\end{proof}

\begin{remark}
Мы будем записывать эффективное
\Ts{G}представление в форме
\[v'=t_\star(a) v=av\]
Орбита этого представления имеет вид
\ShowEq{orbit of effective G* representation}
Мы будем пользоваться обозначением
\ShowEq{space of orbits of effective G* representation}
для пространства орбит эффективного \Ts{G}представления.
\qed
\end{remark}

\begin{remark}
Мы будем записывать эффективное
\sT{G}представление в форме
\[v'=v\ {}_\star t(a)=va\]
Орбита этого представления имеет вид
\ShowEq{orbit of effective *G representation}
Мы будем пользоваться обозначением
\ShowEq{space of orbits of effective *G representation}
для пространства орбит эффективного \sT{G}представления.
\qed
\end{remark}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: Free representation is single transitive}
Свободное \Ts{G}представление эффективно.
Свободное \Ts{G}представление $f$ в $\Omega$\Hyph алгебре $M$
однотранзитивно на орбите.
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: free representation of group}.
\end{proof}
\fi

\begin{theorem}%
\label{theorem: shifts on group commuting}
Правый и левый сдвиги на группе $G$ перестановочны.
\end{theorem}
\begin{proof}
Это следствие ассоциативности группы $G$
\[(t_\star(a)\circ\ {}_\star t(b))c = a(cb)=(ac)b
=({}_\star t(b)\circ t_\star(a))c\]
\end{proof}

Теорема \ref{theorem: shifts on group commuting} может
быть сформулирована следующим образом.

\begin{theorem}%
\label{theorem: shift is automorphism of representation}
Пусть $G$ - группа. Для любого $a\in G$ отображение
$t_\star(a)$ является автоморфизмом представления ${}_\star t$.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: shifts on group commuting}
\begin{equation}
t_\star(a)\circ {}_\star t(b)={}_\star t(b)\circ t_\star(a)
\EqLabel{shifts on group commuting}
\end{equation}
Равенство \EqRef{shifts on group commuting}
совпадает с равенством
\EqRef{morphism of representations of F algebra, definition, 2}
из определения
\ref{definition: morphism of representations of F algebra}
при условии $r=id$, $R=t_\star(a)$.
\end{proof}

\begin{theorem}%
\label{theorem: two representations of group}
Пусть \Ts{G}представление $f$
на $\Omega$\Hyph алгебре $M$ однотранзитивно.
Тогда мы можем однозначно определить однотранзитивное \sT{G}представление $h$
на $\Omega$\Hyph алгебре $M$
такое, что диаграмма
\[
\xymatrix{
M\ar[rr]^{h(a)}\ar[d]^{f(b)} & & M\ar[d]^{f(b)}\\
M\ar[rr]_{h(a)}& &M
}
\]
коммутативна для любых $a$, $b\in G$.\footnote{Это
утверждение можно также найти в \citeBib{Rashevsky}.}
\end{theorem}
\begin{proof}
Мы будем пользоваться групповыми координатами для точек $v\in M$.
Тогда согласно теореме \ref{theorem: single transitive representation of group}
мы можем записать левый сдвиг $t_\star(a)$ вместо преобразования $f(a)$.

Пусть $v_0, v\in M$. Тогда мы можем найти
одно и только одно $a\in G$ такое, что
\[v=v_0 a=v_0\ {}_\star t(a)\]
Мы предположим
\[h(a)=\ {}_\star t(a)\]
Существует $b\in G$ такое, что
\[w_0=f(b)v_0=t_\star (b)v_0\ \ \ \ w=f(b)v=t_\star(b) v\]
Согласно теореме \ref{theorem: shifts on group commuting} диаграмма
\begin{equation}
\xymatrix{
v_0\ar[rr]^{h(a)=\ {}_\star t(a)}\ar[d]^{f(b)=t_\star(b)}
& & v\ar[d]^{f(b)=t_\star(b)}\\
w_0\ar[rr]_{h(a)=\ {}_\star t(a)}& &w
}
\label{Diagram: two representations of group}
\end{equation}
коммутативна.

Изменяя $b$ мы получим, что $w_0$ - это произвольная точка, принадлежащая $M$.

Мы видим из диаграммы, что, если $v_0=v$, то $w_0=w$ и следовательно $h(e)=\delta$.
С другой стороны, если $v_0\neq v$, то $w_0\neq w$ потому, что
\Ts{G}представление $f$ однотранзитивно.
Следовательно \sT{G}представление $h$ эффективно.

Таким же образам мы можем показать, что для данного $w_0$ мы можем найти $a$
такое, что $w=h(a)w_0$. Следовательно \sT{G}представление $h$ однотранзитивно.

В общем случае, произведение преобразований \Ts{G}представления $f$
не коммутативно и следовательно
\sT{G}представление $h$ отлично от \Ts{G}представления $f$.
Таким же образом мы можем создать \Ts{G}представление $f$, пользуясь \sT{G}представлением $h$.
\end{proof}

Мы будем называть представления $f$ и $h$
\AddIndex{парными представлениями группы}{twin representations of group} $G$.

\begin{remark}
\label{remark: one representation of group}
Очевидно, что преобразования $t_\star(a)$ и ${}_\star t(a)$
отличаются, если группа $G$ неабелева.
Тем не менее, они являются отображениями на.
Теорема \ref{theorem: two representations of group} утверждает, что, если оба
представления правого и левого сдвига существуют на множестве $M$,
то мы можем определить два перестановочных представления на множестве $M$.
Только правый или левый сдвиг не может представлять оба типа представления.
Чтобы понять почему это так, мы можем изменить диаграмму \eqref{Diagram: two representations of group}
и предположить $h(a)v_0=t_\star(a) v_0=v$
вместо $h(a)v_0=v_0{}_\star t(a)=v$ и
проанализировать, какое выражение $h(a)$ имеет в
точке $w_0$. Диаграмма
\[\xymatrix{
v_0\ar[rr]^{h(a)=t_\star(a)}\ar[d]^{f(b)=t_\star(b)}
& & v\ar[d]^{f(b)=t_\star(b)}\\
w_0\ar[rr]_{h(a)}& &w
}\]
эквивалентна диаграмме
\[\xymatrix{
v_0\ar[rr]^{h(a)=t_\star(a)} & & v\ar[d]^{f(b)=t_\star(b)}\\
w_0\ar[rr]_{h(a)}\ar[u]_{f^{-1}(b)=t_\star(b^{-1})}& &w
}\]
и мы имеем $w=bv=bav_0=bab^{-1}w_0$. Следовательно
\[h(a)w_0=(bab^{-1})w_0\] Мы видим, что представление $h$
зависит от его аргумента.\qed  
%There is interesting question. Если I имею преобразование $a\star$ in точке $b$
%what is $c$ такое, что $a\star b = R_c b$. Мы можем find it из равенства
%$ab=bc$, so $c=b^{-1}ab$, следовательно
%\[a\star b = R_{b^{-1}ab} b\]?????
\end{remark}

\begin{theorem}%
\label{theorem: twin representations of group, automorphism}
Пусть $f$ и $h$ - парные преставления группы $G$. Для любого $a\in G$ отображение
$h(a)$ является автоморфизмом представления $f$.
\end{theorem}
\begin{proof}
Следствие теорем
\ref{theorem: shift is automorphism of representation} и
\ref{theorem: two representations of group}.
\end{proof}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{remark}
Существует ли морфизм представлений
из $t_\star$ в $t_\star$, отличный от автоморфизма $(\id,{}_\star t(a))$?
Если мы положим
\[
r(g)=cgc^{-1}
\]
\[
R(a)(m)=cmac^{-1}
\]
то нетрудно убедиться, что отображение $(r,R(a))$ является
морфизмом представлений из $t_\star$ в $t_\star$.
Но это отображение не является
автоморфизмом представления $t_\star$,
так как $r\ne\id$.
\qed
\end{remark}
\fi


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%202%*%*D вектор строка
   {$*D$\Hyph вектор строка}%
   {row *D vector}%
\Index%192%*%*D- векторное пространство
   {$*D$\Hyph векторное пространство}%
   {*D vector space}%
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) map}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%660%A%Astar- модуль
   {$A\star$\Hyph модуль}%
   {Astar-module}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение матриц
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%304%C%crd вектор
   {\crd вектор}%
   {crd vector}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%92%D%D* вектор столбец
   {$D*$\Hyph вектор столбец}%
   {column D* vector}%
\Index%93%D%D* вектор строка
   {$D*$\Hyph вектор строка}%
   {row D* vector}%
\Index%87%D%D*- векторное пространство матриц
   {$D*$\hyph векторное пространство матриц}%
   {matrices vector space}%
\Index%40%D%D*-векторное пространство
   {$D*$\hyph векторное пространство}%
   {D* vector space}%
\Index%156%D%D*-модуль
   {$D*$\Hyph модуль}%
   {D*-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%26%D%Drc базис в векторном расслоении
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%200%D%drc вектор
   {\dcr вектор}%
   {dcr vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главная минорная матрица
   {\RC главная минорная матрица}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение матриц
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%600%R%RCcirc вырожденная матрица
   {$\RCcirc$\Hyph вырожденная матрица}%
   {RCcirc singular matrix}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица
   {$\RCcirc$\Hyph невырожденная матрица}%
   {RCcirc nonsingular matrix}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%111%R%rcd аффинный базис
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%735%S%starD аффинное пространство
   {$\star D$\Hyph аффинное пространство}%
   {starD affine space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%185%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%187%T%Tstar- представление расслоенной группы
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%830%А%абелевая мультипликативная Omega группа
   {абелевая мультипликативная $\Omega$\Hyph группа}%
   {Abelian multiplicative Omega group}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%22%А%автоморфизм векторного пространства
   {автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное *G представление
   {активное \sT{G}представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%569%А%активное представление группы в многообразии базисов представления
   {активное представление группы $G(f)$ в многообразии базисов представления}%
   {active representation in basis manifold}%
\Index%715%А%активное преобразование многообразия базисов башни представлений
   {активное преобразование многообразия базисов башни представлений}%
   {active transformation of basis, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%167%А%алгебра с делением
   {алгебра с делением}%
   {division algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%779%А%антилинейное отображение
   {антилинейное отображение}%
   {antilinear map}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%89%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%579%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%203%Б%базис crd векторного пространства
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Index%197%Б%базис D векторного пространства
   {базис $D$\Hyph векторного пространства}%
   {basis, D vector space}%
\Index%106%Б%базис dcr векторного пространства
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Index%16%Б%базис drc векторного пространства
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Index%24%Б%базис rcd векторного пространства
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%833%В%вектор, линейно зависимый от векторов
   {вектор, линейно зависимый от векторов}%
   {vector linearly dependent on vectors}%
\Index%727%В%векторное пространство над полем
   {векторное пространство над полем}%
   {vector space over field}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%398%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%687%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%33%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%481%В%взаимно простые  A числа
   {взаимно простые  $A$\Hyph числа}%
   {relatively prime A numbers}%
\Index%163%В%внешняя мера
   {внешняя мера}%
   {outer measure}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%231%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%70%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%781%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\SetIndexSpace%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%698%Г%геометрический объект в координатном представлении, определённом в Omega_2- алгебре
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H, representation g}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%700%Г%геометрический объект, определённый в Omega_2- алгбре
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%73%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%686%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%765%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%613%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%655%Д%декартова степень систем подмножеств
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Index%390%Д%декартово произведение групп
   {декартово произведение групп}%
   {Cartesian product of groups}%
\Index%199%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%625%Д%декартово произведение систем подмножеств
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Index%825%Д%декартово произведением Omega алгебр
   {декартово произведением \(\Omega\)\Hyph алгебр}%
   {Cartesian product of Omega algebras}%
\Index%598%Д%деление без остатка
   {деление без остатка}%
   {division without remainder}%
\Index%573%Д%деление с остатком
   {деление с остатком}%
   {division with remainder}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%157%Д%дифференциал Гато отображения
   {дифференциал Гато отображения}%
   {Gateaux differential of map}%
\Index%78%Д%долгота
   {долгота}%
   {longitude}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%44%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\SetIndexSpace%
\Index%662%З%закон ассоциативности
   {закон ассоциативности}%
   {associative law}%
\Index%672%З%закон дистрибутивности
   {закон дистрибутивности}%
   {distributive law}%
\Index%673%З%закон унитарности
   {закон унитарности}%
   {unitarity law}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%80%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\SetIndexSpace%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%164%И%измеримое по Лебегу множество
   {измеримое по Лебегу множество}%
   {Lebesgue measurable}%
\Index%31%И%изоморфизм векторных пространств
   {изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%680%И%интеграл отображения
   {интеграл отображения}%
   {integral of map}%
\Index%693%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%599%К%каноническое представление деления с остатком
   {каноническое представление деления с остатком}%
   {canonical representation of division with remainder}%
\Index%726%К%каноническое частное от деления
   {каноническое частное от деления}%
   {canonical remainder of the division}%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%177%К%категория левосторонних представлений
   {категория левосторонних представлений}%
   {category of left-side representations}%
\Index%176%К%категория левосторонних представлений Omega1 алгебры A
   {категория левосторонних представлений $\Omega$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of maps}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%741%К%кватернионная алгебра
   {кватернионная алгебра}%
   {quaternion algebra}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%577%К%кольцо множеств, порождённое полукольцом множеств
   {кольцо множеств, порождённое полукольцом множеств}%
   {ring of sets generated by semiring}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%170%К%конечное разложение множества
   {конечное разложение множества}%
   {finite expansion of set}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%210%К%координатное Drc векторное расслоение
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%697%К%координатное представление в Omega_2- алгебре
   {координатное представление в $\Omega_2$\Hyph алгебре}%
   {coordinate representation, Omega_2 algebra}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%664%К%координатное представление вектора
   {координатное представление вектора}%
   {coordinate representation of vector}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%25%К%координаты базиса
   {координаты базиса}%
   {coordinates of basis}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%701%К%координаты геометрического объекта в Omega_2- алгбре
   {координаты геометрического объекта в $\Omega_2$\Hyph алгбре $M$}%
   {coordinates of geometric object, representation g}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%699%К%координаты геометрического объекта в координатном пространстве представления
   {координаты геометрического объекта в координатном пространстве представления}%
   {coordinates of geometric object, coordinate representation}%
\Index%723%К%координаты геометрического объекта в кортеже Omega- алгебр
   {координаты геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinates of geometric object, tower of representations g}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%737%К%координаты точки rcd аффинного пространства относительно базиса
   {координаты точки \rcd аффинного пространства относительно базиса}%
   {coordinates in rcd affine space}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%558%К%координаты элемента представления относительно множества
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%166%Л%лебегово продолжение меры
   {лебегово продолжение меры}%
   {Lebesgue extension of measure}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%228%Л%левое D векторное пространство
   {левое $D$\Hyph векторное пространство}%
   {left vector space}%
\Index%585%Л%левое D векторное пространство столбцов
   {левое $D$\hyph векторное пространство столбцов}%
   {left vector space of columns}%
\Index%576%Л%левое D векторное пространство строк
   {левое $D$\hyph векторное пространство строк}%
   {left vector space of rows}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%184%Л%левостороннее представление группы
   {левостороннее представление группы}%
   {left-side representation of group}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%665%Л%левостороннее произведение вектора на скаляр
   {левостороннее произведение вектора на скаляр}%
   {left-side product of vector over scalar}%
\Index%271%Л%левостороннее произведение отображения на скаляр
   {левостороннее произведение отображения на скаляр}%
   {left-side product of map over scalar}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль нaд кольцом
   {левый модуль нaд кольцом $D$}%
   {left module over ring}%
\Index%661%Л%левый модуль над D- алгеброй A
   {левый модуль над $D$\Hyph алгеброй $A$}%
   {left module over algebra}%
\Index%731%Л%левый сдвиг модуля
   {левый сдвиг модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {left shift, fibered group}%
\Index%88%Л%линейная комбинация векторов
   {линейная комбинация векторов}%
   {linear combination of  vectors}%
\Index%832%Л%линейная комбинация векторов
   {линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index%32%Л%линейная оболочка в векторном пространстве
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%688%Л%линейно зависимое множество A- модуля
   {линейно зависимое множество $A$\Hyph модуля}%
   {linear dependent vectors, module}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%21%Л%линейно зависимые векторы
   {линейно зависимые векторы}%
   {linearly dependent vectors}%
\Index%34%Л%линейно независимые векторы
   {линейно независимые векторы}%
   {linearly independent vectors}%
\Index%37%Л%линейное G* представление
   {линейное \Ts{G}представление}%
   {linear G* representation}%
\Index%35%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%740%Л%линейное преобразование rcd аффинного пространства
   {линейное преобразование \rcd аффинного пространства}%
   {linear transformation, rcd affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%769%Л%линейный гомоморфизм
   {линейный гомоморфизм}%
   {linear homomorphism}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear maps}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of maps}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%161%М%мера
   {мера}%
   {measure}%
\Index%165%М%мера Лебега
   {мера Лебега}%
   {Lebesgue measure}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие базисов \rcd аффинного пространства
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%356%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни представлений в башню представлений
   {морфизм из башни представлений в башню представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%828%М%мультипликативная Omega группа
   {мультипликативная $\Omega$\Hyph группа}%
   {multiplicative Omega group}%
\Index%829%М%мультипликативное отображение
   {мультипликативное отображение}%
   {multiplicative map}%
\Index%85%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%207%Н%наибольший общий делитель
   {наибольший общий делитель}%
   {highest common factor}%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%738%Н%начало системы координат star D аффинного пространства
   {начало системы координат $\star D$\Hyph аффинного пространства}%
   {origin of coordinate system of starD affine space}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%29%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%284%Н%норма на теле
   {норма на теле}%
   {absolute value on division ring}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\SetIndexSpace%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%482%О%общий делитель
   {общий делитель}%
   {common factor}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство группы
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен степени
   {однородный многочлен степени $n$}%
   {homogeneous polynomial of power}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear map}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%484%О%остаток от деления
   {остаток от деления}%
   {remainder of the division}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг rcd аффинного пространства
   {параллельный сдвиг \rcd аффинного пространства}%
   {parallel shift, rcd affine space}%
\Index%684%П%парные представления D- алгебры
   {парные представления $D$\Hyph алгебры}%
   {twin representations of D algebra}%
\Index%587%П%парные представления ассоциативной алгебры
   {парные представления ассоциативной алгебры}%
   {twin representations of associative algebra}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное *G представление
   {пассивное \sT{G}представление}%
   {passive *G representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%695%П%пассивное представление группы в многообразии базисов представления
   {пассивное представление группы $G(f)$ в многообразии базисов представления}%
   {passive representation in basis manifold}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%230%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%345%П%полиалинейное косо симметричное отображение
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%764%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%169%П%полукольцо множеств
   {полукольцо множеств}%
   {semiring of sets}%
\Index%186%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%19%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%578%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%353%П%правое D векторное пространство
   {правое $D$\Hyph векторное пространство}%
   {right vector space}%
\Index%671%П%правое D векторное пространство столбцов
   {правое $D$\hyph векторное пространство столбцов}%
   {right vector space of columns}%
\Index%654%П%правое D векторное пространство строк
   {правое $D$\hyph векторное пространство строк}%
   {right vector space of rows}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%355%П%правостороннее представление группы
   {правостороннее представление группы}%
   {right-side representation of group}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%674%П%правостороннее произведение вектора на скаляр
   {правостороннее произведение вектора на скаляр}%
   {right-side product of vector over scalar}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль нaд кольцом
   {правый модуль нaд кольцом $D$}%
   {right module over ring}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%703%П%представитель геометрического объекта в Omega_2- алгбре
   {представитель геометрического объекта в $\Omega_2$\Hyph алгбре}%
   {representative of geometric object, representation g}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%82%П%представление Omega1 алгебры A в Omega2 алгебре *A
   {\sT{A}представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре}%
   {*A representation of algebra}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%90%П%представление в Omega2- алгебре A*
   {\Ts{A}представление в $\Omega_2$\Hyph алгебре}%
   {A* representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%831%П%приведенный морфизм представлений
   {приведенный морфизм представлений}%
   {reduced morphism of representations}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%384%П%принцип инвариантности в представлении универсальной алгебры
   {принцип инвариантности в представлении универсальной алгебры}%
   {invariance principle, representation g}%
\Index%162%П%продолжение меры
   {продолжение меры}%
   {extension of measure}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%663%П%произведение колец множеств
   {произведение колец множеств}%
   {product of rings of sets}%
\Index%172%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%483%П%простое A число
   {простое $A$\Hyph число}%
   {prime A number}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит G* представления
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%412%П%прямое произведение G* представлений
   {прямое произведение \Ts{G}представлений}%
   {direct product of G* representations}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%826%П%прямое произведением Omega алгебр
   {прямое произведением \(\Omega\)\Hyph алгебр}%
   {direct product of Omega algebras}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%782%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%441%С%свободное представление группы
   {свободное представление группы}%
   {free representation of group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль над кольцом
   {свободный модуль над кольцом}%
   {free module over ring}%
\Index%517%С%связное множество
   {связное множество}%
   {connected set}%
\Index%583%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%214%С%симплекс
   {симплекс}%
   {simplex}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%201%С%система линейных уравнений
   {система линейных уравнений}%
   {system of linear equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%683%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%789%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%171%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%351%С%сумма отображений
   {сумма отображений}%
   {sum of maps}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%323%С%суперпозиция координат эндоморфизма представления и элемента
   {суперпозиция координат эндоморфизма представления $f$ и элемента $m$}%
   {superposition of coordinates, representation}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\Index%168%С%сферические координаты
   {сферические координаты}%
   {spherical coordinates}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение
   {тензорное произведение}%
   {tensor product}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\Index%827%Ч%частное от деления
   {частное от деления}%
   {quotient divided by}%
\SetIndexSpace%
\Index%501%Ш%широта
   {широта}%
   {latitude}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%516%Э%эффективное G* представление
   {эффективное \Ts{G}представление}%
   {effective G* representation}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%500%Э%эффективное представление Omega- алгебры
   {эффективное представление $\Omega$\Hyph алгебры}%
   {effective representation of algebra}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности G* представления
   {ядро неэффективности \Ts{G}представления}%
   {kernel of inefficiency of G* representation}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%656%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> Preface.0912.3315.English.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\chapter{Preface}

\section{Preface}

In my papers, I often explore problems relating to the representation of
universal algebra. Initially it was small sketches
which I repeatedly corrected and rewrote.
However gradually there were new observations.
As a result, auxiliary tool became a consistent theory.

I realized this when I was writing book
\citeBib{0906.0135}, and I decided to dedicate a separate book
to the questions related with representation of universal algebra.
Exploring of the theory of representations of universal algebra
shows that this theory has a lot of common with theory of
universal algebra.

The definition of vector space as representation of field
in the Abelian group was the main impetus of deeper exploring
of representations of
universal algebra.
I put attention that this definition changes role 
of linear map.
It was found that linear map is the map
that preserves the structure of the representation.
It is easy to generalize this structure for an arbitrary representation of
universal algebra.
Thus I came to the notion of morphism of representation.

The set of regular automorphisms of vector space
forms a group. This group is single transitive on the set of
basises of vector space. This statement is the foundation of
the theory of invariants of vector space.

The natural question arises. Can we generalize this structure
to arbitrary representation?
The basis is not the only set that forms
the vector space.
If we add an arbitrary vector to the set of vectors of basis,
then a new set also generates the same vector
space, however this set is not basis.
This statement is initial point where I started
exploring of generating set of representation.
Generating set of representation is one more interesting
parallel between theory of representations and
theory of universal algebra.

The set of automorphisms of representations is loop.
Nonassociativity of the product is the source of numerous
questions which require additional research.
All these questions lead to the need to understand the
theory of invariants of a given representation.

If we consider the theory of representations of universal algebra
as an extension of the theory of universal algebra,
then why not consider the representation of one representation
in another representation.
Thus the concept of the tower representations appeared.
The most amazing fact is the statement that all maps in the
tower of representations are coordinated.

\ifx\texFuture\Defined
%Несмотря на обнаруженные в начале XX века проблемы в основаниях
%математики, математика остаётся мощным и надёжным инструментом.
В молодости, изучая теорию множеств по Бурбаки,
я обратил внимание на парадоксальную ситуацию.
В главе I Бурбаки рассматривают основы математической логики.
Это - достаточно стандартный и хорошо известный курс.
Сюрприз ждал меня в приложении
(\citeBib{Bourbaki: Set Theory}, стр. 66 - 70),
где Бурбаки рассматривают логические термы как элементы моноида
(\citeBib{Bourbaki: Set Theory}, гл. I, ).
\fi

\ifx\texFuture\Defined
Морфизм представлений во многом похож на морфизм расслоений.
В обоих случаях я работаю с диаграммой вида
\[
\xymatrix{
A\ar[rr]^f&&B
\\
C\ar[u]^p\ar[rr]^g&&D\ar[u]^q
}
\]
Отображения $f$, $g$ описывают морфизм. При этом каждая
стрелка по отдельности является морфизмом некоторой
universal алгебры.\footnote{Если на множестве
не задана некоторая universal алгебра, то мы можем
полагать, что множество операций, определённых на этом множестве,
пусто.}
Отображения $p$, $q$
согласуют отображения $f$, $g$
таким образом, что диаграмма коммутативна
(определения \ref{definition: morphism of representations of F algebra}
и \xRef{0702.561}{definition: fibered morphism}).

Let us define an additional structure on vector space $\mathcal{V}$
(for instance, a scalar product or a norm of a vector).
Then not every \drc linear map keeps properties of the selected structure.
In this case we need subgroup
$G$ of the group $\RCGL nD$
\drc linear maps from which hold properties of the selected structure.
We usually call group $G$
symmetry group.
Without loss of generality we identify element $g$ of group $G$
with corresponding transformation of representation
and write its action on vector $\Vector V\in\mathcal{V}$ as $v\RCstar g$.

Not every two bases can be mapped by a transformation
from the symmetry group
because not every nonsingular linear transformation belongs to
the representation of group $G$. Therefore, we can represent
the set of bases
as a union of orbits of group $G$.

Properties of basis depend on the symmetry group.
We can select basis $\Basis{e}$ vectors of which are
in a relationship which is invariant relative to symmetry group.
In this case all bases from orbit $\Basis{e}G$
have vectors which satisfy the same relationship. Such a basis we call
\AddIndex{$G$\Hyph basis}{G-basis}.
In each particular case we need to prove the existence of a basis
with certain properties. If such a basis does not exist
we can choose an arbitrary basis.

Basis $\Basis{e}$ creates coordinates in $\mathcal{V}$.
In different types of space it may be done in different ways.
In affine space if node of basis is point $A$ then
point $B$ has the same coordinates as vector $\overset{\longrightarrow}{AB}$
relative basis $\Basis{e}$.
In a general case we introduce coordinates of a vector as coordinates
relative to the selected basis.
Using only bases of type $G$ means using of specific coordinates on $\mathcal{A}_n$.
To distinguish them we call this \AddIndex{$G$\Hyph coordinates}{G-coordinates}.
We also call the space $\mathcal{V}$ with such coordinates
\AddIndex{$G$\Hyph space}{GSpace}.
\fi



==> Preface.0912.3315.Eq.tex <==
%auto-ignore

\DefEq
{
$\Vector u+\Vector v=\Vector v+\Vector u$
}
{vector sum 1}

\DefEq
{
$\Vector u+(-\Vector u)=\Vector 0$
}
{vector sum 4}

\DefEq
{
$\Vector 0+\Vector v=\Vector v$
}
{vector sum 3}

\DefEq
{
$\Vector u+(\Vector v+\Vector w)=(\Vector u+\Vector v)+\Vector w$
}
{vector sum 2}

\DefEq
{
$1\Vector u=\Vector u$
}
{vector am 1}

\DefEq
{
$a(b\Vector u)=(ab)\Vector u$
}
{vector am 2}

\DefEq
{
$(a+b)\Vector u=a\Vector u+b\Vector u$
}
{vector am 3}

\DefEq
{
\begin{align*}
(a+b)\Vector u&=a\Vector u+b\Vector u&
a(\Vector u+\Vector v)&=a\Vector u+a\Vector v&
a,b\in F&&\Vector u,\Vector v\in\Vector V
\end{align*}
}
{vector am 5}

\DefEq
{
$a(\Vector u+\Vector v)=a\Vector u+a\Vector v$
}
{vector am 4}


==> Preface.0912.3315.Russian.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\chapter{Предисловие}

\section{Предисловие}

В статьях я часто рассматриваю вопросы, связанные с представлением
универсальной алгебры. Вначале это были небольшие наброски,
которые я многократно исправлял и переписывал.
Но постепенно появлялись новые наблюдения.
В результате вспомогательный инструмент превратился в стройную теорию.

Я это понял, когда я работал над книгой
\citeBib{0906.0135}, и решил посвятить отдельную книгу
вопросам, связанным с представлением универсальной алгебры.
Изучение теории представлений универсальной алгебры
показывает, что эта теория имеет много общего с теорией
универсальной алгебры.

Основным толчком к более глубокому изучению представлений
универсальной алгебры послужило определение векторного
пространства как представление поля в абелевой группе.
Я обратил внимание, что это определение меняет роль
линейного отображения.
По сути, линейное отображение - это отображение,
которое сохраняет структуру представления.
Эту конструкцию легко обобщить на произвольное представление
универсальной алгебры.
Таким образом появилось понятие морфизма представлений.

Множество невырожденных автоморфизмов векторного пространства
порождает группу. Эта группа действует однотранзитивно на множестве
базисов векторного пространства. Это утверждение является фундаментом
теории инвариантов векторного пространства.

Возникает естественный вопрос. Можно ли обобщить эту конструкцию
на произвольное представление?
Базис - это не единственное множество, которое порождает
векторное пространство.
Если мы к множеству векторов базиса добавим произвольный вектор,
то новое множество по прежнему порождает тоже самое векторное
пространство, но базисом не является.
Это утверждение является исходной точкой, от которой я начал
изучение множества образующих представления.
Множество образующих представления - это ещё одна интересная
параллель теории представлений с теорией универсальной алгебры.

Множество автоморфизмов представления является лупой.
Неассоциативность произведения порождает многочисленные
вопросы, которые требуют дополнительное исследование.
Все эти вопросы ведут к необходимости понимания теории инвариантов
заданного представления.

Если мы рассматриваем теорию представлений универсальной алгебры
как расширение теории универсальной алгебры,
то почему не рассмотреть представление одного представления
в другом представлении. Так появилась концепция башни представлений.
Самый удивительный факт - это то, что все отображения в
башне представлений действуют согласовано.

\ifx\texFuture\Defined
%Несмотря на обнаруженные в начале XX века проблемы в основаниях
%математики, математика остаётся мощным и надёжным инструментом.
В молодости, изучая теорию множеств по Бурбаки,
я обратил внимание на парадоксальную ситуацию.
В главе I Бурбаки рассматривают основы математической логики.
Это - достаточно стандартный и хорошо известный курс.
Сюрприз ждал меня в приложении
(\citeBib{Bourbaki: Set Theory}, стр. 66 - 70),
где Бурбаки рассматривают логические термы как элементы моноида
(\citeBib{Bourbaki: Set Theory}, гл. I, ).
\fi

\ifx\texFuture\Defined
Морфизм представлений во многом похож на морфизм расслоений.
В обоих случаях я работаю с диаграммой вида
\[
\xymatrix{
A\ar[rr]^f&&B
\\
C\ar[u]^p\ar[rr]^g&&D\ar[u]^q
}
\]
Отображения $f$, $g$ описывают морфизм. При этом каждая
стрелка по отдельности является морфизмом некоторой
универсальной алгебры.\footnote{Если на множестве
не задана некоторая универсальная алгебра, то мы можем
полагать, что множество операций, определённых на этом множестве,
пусто.}
Отображения $p$, $q$
согласуют отображения $f$, $g$
таким образом, что диаграмма коммутативна
(определения \ref{definition: morphism of representations of F algebra}
и \xRef{0702.561}{definition: fibered morphism}).

Если на векторном пространстве $\mathcal{V}$ определена дополнительная структура
(например, скалярное произведение или норма вектора),
не всякий \drc линейное отображение сохраняет свойства заданной структуры.
В этом случае нас интересует подгруппа
$G$ группы $\RCGL nD$,
\drc линейное отображения которой сохраняют свойства заданной структуры.
Мы обычно будем называть группу $G$
группой симметрии.
Не нарушая общности, мы будем отождествлять элемент $g$ группы $G$
с соответствующим преобразованием представления
и записывать его действие на вектор $\Vector V\in\mathcal{V}$
в виде $v\RCstar g$.

Не всякие два базиса могут быть связаны
преобразованием группы симметрии
потому, что не всякое невырожденное линейное преобразование принадлежит
представлению группы $G$. Таким образом, множество базисов
можно представить как объединение орбит группы $G$.

Свойства базиса зависят от группы симметрии.
Мы можем выбрать базисы $\Basis{e}$, векторы которых находятся
в отношении, которое инвариантно относительно группы симметрии.
В этом случае все базисы из орбиты $\Basis{e}G$
имеют векторы, которые удовлетворяют одному и тому же отношению.
Такой базис мы будем называть
\AddIndex{$G$\Hyph базисом}{G-basis}.
В каждом конкретном случае мы должны доказать существование
базиса с искомыми свойствами. Если подобного типа базиса
не существует, мы можем выбрать произвольный базис.

Базис $\Basis{e}$ порождает координаты на $\mathcal{V}$.
В различных типах пространства это может быть сделано различным образом.
В аффинном пространстве, если вершина базиса является точкой $A$, то
точка $B$ имеет те же координаты, что и вектор $\overset{\longrightarrow}{AB}$
относительно базиса $\Basis{e}$.
В общем случае мы вводим координаты вектора как координаты
относительно выбранного базиса.
Использование только \Gspaceа означает использование специальных координат на $\mathcal{A}_n$.
Для того, чтобы отличать их, мы будем называть их
\AddIndex{$G$\Hyph координатами}{G-coordinates}.
Мы также будем называть пространство $\mathcal{V}$ с такими координатами
\AddIndex{$G$\Hyph пространством}{GSpace}.
\fi


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {единичный интервал}%
   {unit interval}%

\SetIndexSpace%A%0
\Symb%
   {минорная матрица}%
   {A from b a}%
\Symb%
   {минорная матрица}%
   {A from columns T}%
\Symb%
   {минорная матрица}%
   {A from rows S}%
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
\Symb%
   {минорная матрица}%
   {A without column a}%
\Symb%
   {минорная матрица}%
   {A without columns T}%
\Symb%
   {минорная матрица}%
   {A without row b}%
\Symb%
   {минорная матрица}%
   {A without rows S}%
\Symb%
   {активное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Symb%
   {активное представление группы $G(\Vector  f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {active representation in basis manifold, tower of representations}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
\Symb%
   {аффинное пространство}%
   {An}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb%
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb%
   {\crd вектор}%
   {crd vector}%
\Symb%
   {\dcr вектор}%
   {dcr vector}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb%
   {\drc вектор}%
   {drc vector}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
\Symb%
   {левая дробь}%
   {left fraction}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
\Symb%
   {$A$\Hyph модуль однородных многочленов над $D$\Hyph алгеброй $A$}%
   {module of homogeneous polynomials over algebra}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear map}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
\Symb%
   {главный идеал}%
   {principal ideal}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
\Symb%
   {правый сдвиг}%
   {right shift}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
\Symb%
   {симплекс}%
   {simplex}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \rcd векторного пространства $\Vector V$}%
   {basis manifold of rcd vector space}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Symb%
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
\Symb%
   {каноническое частное от деления}%
   {canonical remainder of the division}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
\Symb%
   {замыкание множества}%
   {closure of set}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
\Symb%
   {открытый шар}%
   {open ball}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb%
   {правая дробь}%
   {right fraction}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
\Symb%
   {структурные константы}%
   {structural constants}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
\Symb%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, scalar}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb%
   {производная Картана}%
   {overbrace D}%
\Symb%
   {производная}%
   {overline D}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%E%0
\Symb%
   {матрица Якоби левого сдвига}%
   {aE, quaternion, Jacobian matrix}%
\Symb%
   {аффинный базис}%
   {Affine Basis}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
\Symb%
   {базис модуля}%
   {basis for module}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
\Symb%
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Symb%
   {базис $D$\Hyph векторного пространства}%
   {basis, D vector space}%
\Symb%
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Symb%
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Symb%
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
\Symb%
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%F%0
\Symb%
   {центро-аффинный}%
   {Central Affine Basis, division ring}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb%
   {норма функционала}%
   {norm of functional}%
\Symb%
   {норма отображения}%
   {norm of map}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
\Symb%
   {норма представления}%
   {norm of representation}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
\Symb%
   {система отсчёта}%
   {reference frame}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Symb%
   {сумма отображений}%
   {sum of maps}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, 1 n}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra of Lie group}%
\Symb%
   {алгебра Ли группы Ли}%
   {Lie algebra of Lie group}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
\Symb%
   {малая группа элемента $x$}%
   {little group}%
\Symb%
   {орбита эффективного \sT{G}представления}%
   {orbit of effective *G representation}%
\Symb%
   {орбита эффективного \Ts{G}представления}%
   {orbit of effective G* representation}%
\Symb%
   {орбита эффективного	\Ts представления группы}%
   {orbit of effective starT representation of fibered group}%
\Symb%
   {орбита эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar representation of fibered group}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Symb%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
\Symb%
   {алгебра кватернионов над полем действительных чисел}%
   {quaternion algebra over real field}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%

\SetIndexSpace%K%0
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%

\SetIndexSpace%L%0
\Symb%
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Symb%
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
\Symb%
   {множество линейных отображений}%
   {set linear maps}%
\Symb%
   {множество левосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of left-side nonsingular transformations}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%

\SetIndexSpace%M%0
\Symb%
   {множество левосторонних преобразований универсальной алгебры $M$}%
   {set of left-side transformations}%
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
\Symb%
   {множество правосторонних преобразований универсальной алгебры $M$}%
   {set of right-side transformations}%
\Symb%
   {множество преобразований универсальной алгебры $M$}%
   {set of transformations}%
\Symb%
   {пространство орбит эффективного \sT{G}представления}%
   {space of orbits of effective *G representation}%
\Symb%
   {пространство орбит эффективного \Ts{G}представления}%
   {space of orbits of effective G* representation}%
\Symb%
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
\Symb%
   {орбита \Ts{G}представления группы}%
   {orbit of representation of group}%
\Symb%
   {тензорное произведение}%
   {tensor product}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb%
   {пассивное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {passive representation in basis manifold}%
\Symb%
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {passive representation in basis manifold, tower of representations}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
\Symb%
   {произведение колец множеств}%
   {product of rings of sets}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
\Symb%
   {множество правосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of right-side nonsingular transformations}%
\Symb%
   {сферические координаты}%
   {spherical coordinates}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb%
   {интеграл отображения \(f\)}%
   {integral of map}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Symb%
   {образ базиса $X$ при пассивном преобразовании $S$}%
   {passive transformation of basis, representation}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%

\SetIndexSpace%T%0
\Symb%
   {категория левосторонних представлений}%
   {category of left-side representations}%
\Symb%
   {касательная плоскость к группе Ли $G$}%
   {tangent plane to Lie group}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Symb%
   {линейная комбинация векторов}%
   {linear composition of  vectors}%
\Symb%
   {векторное пространство}%
   {V}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to generating set, representation}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Symb%
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Symb%
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Symb%
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Symb%
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
\Symb%
   {суперпозиция координат эндоморфизма представления $f$ и точки $m$}%
   {superposition of coordinates, representation}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
\Symb%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%Z%0
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
\Symb%
   {связность}%
   {conection overline}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%M%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Symb%
   {степень меры}%
   {power of measure}%
\Symb%
   {произведение мер}%
   {product of measures}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%

\SetIndexSpace%O%1
\Symb%
   {норма операции}%
   {norm of operation}%
\Symb%
   {множество $n$\Hyph арных операций $\Omega$\Hyph алгебры}%
   {set of n-ary operations}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%

\SetIndexSpace%Fi%2
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi%2
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi%2
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb%
   {декартово произведение групп $G_i$, $i\in I$}%
   {Cartesian product of groups}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, i 1 n}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
\Symb%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S%2
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb%
   {подрасслоение}%
   {subbundle}%

\CloseIndex


==> Tower.Basis.Russian.tex <==
%auto-ignore
\input{Tower.Basis.Eq}

\ePrints{0912.3315,0906.0135}
\ifx\Semafor\ValueOff
\chapter{Базис башни представлений универсальной алгебры}
\label{chapter: Basis of Tower of Representations of Universal Algebra}
\fi

\section{Множество образующих башни представлений}

\begin{definition}
Башня представлений
$(\Vector A,\Vector f)$.
называется \AddIndex{башней эффективных представлений}{tower of effective representations},
если для любого $i$ представление $f_{i,i+1}$ эффективно.
\qed
\end{definition}

\begin{theorem}
\label{theorem: define effective map f13}
Рассмотрим башню представлений
$(\Vector A,\Vector f)$.
Пусть представления $f_{i,i+1}$, ..., $f_{i+k-1,i+k}$ эффективны.
Тогда представление $f_{i,i+k}$ эффективно.
\end{theorem}
\begin{proof}
Мы докажем утверждение теоремы по индукции.

Пусть представления $f_{i,i+1}$, $f_{i+1,i+2}$ эффективны.
Предположим, что преобразование
\ShowEq{effective tower of representations, 1}
не является
тождественным преобразованием. Тогда существует $a_{i+1}\in A_{i+1}$
такой, что
\ShowEq{effective tower of representations, 2}
Так как представление $f_{i+1,i+2}$ эффективно, то преобразования
\ShowEq{f i+1 i+2 a}
и
\ShowEq{effective tower of representations, 3}
не совпадают.
Согласно построению, выполненному в теореме
\ref{theorem: define map f13},
преобразование
\ShowEq{effective tower of representations, 4}
не является тождественным
преобразованием.
Следовательно, представление $f_{i,i+2}$ эффективно.

Предположим утверждение теоремы верно для $k-1$ представлений и
пусть $f_{i,i+1}$, ..., $f_{i+k-1,i+k}$ эффективны.
Согласно предположению индукции, представления
$f_{i,i+k-1}$, $f_{i+k-1,i+k}$ эффективны.
Согласно доказанному выше, представление $f_{i,i+k}$ эффективно.
\end{proof}

\begin{theorem}
\label{theorem: i i+2 prim effective representation}
Рассмотрим башню $(\Vector A,\Vector f)$ представлений
$\Vector{\Omega}$\Hyph алгебр.
Пусть тождественное преобразование
\ShowEq{identity map A i+2}
$\Omega_{i+2}$\hyph алгебры $A_{i+2}$ принадлежит представлению $f_{i+1,i+2}$.
Пусть представления $f_{i,i+1}$, $f_{i+1,i+2}$ эффективны.
Тогда представление $f'_{i,i+2}$, определённое в теореме
\ref{theorem: expand f i i+2 over A i+2}, эффективно.
\end{theorem}
\begin{proof}
Пусть существует $a_{i+1}\in A_{i+1}$ такой, что
\ShowEq{identity map A i+2, 1a}
Допустим, что представление $f'_{i,i+2}$ не является эффективным.
Тогда существуют \ShowEq{i i+2 prim effective representation, 1}
такие, что \ShowEq{i i+2 prim effective representation, 2}
Из равенств
\EqRef{identity map A i+2, 2},
\EqRef{i i+2 prim effective representation, 2},
следует
\ShowEq{i i+2 prim effective representation, 3}
Так как $a_{i+2}$ произвольно, то из \EqRef{i i+2 prim effective representation, 3}
следует
\ShowEq{i i+2 prim effective representation, 4}
Поскольку представление $f_{i,i+1}$ эффективно,
то из условия \EqRef{i i+2 prim effective representation, 1}
следует
\ShowEq{i i+2 prim effective representation, 5}
Из условия \EqRef{i i+2 prim effective representation, 5}
и равенства \EqRef{i i+2 prim effective representation, 4}
следует, что представление $f_{i+1,i+2}$ не является эффективным.
Полученное противоречие доказывает утверждение теоремы.
\end{proof}

Мы строим базис представления башни представлений
по той же схеме, что мы построили базис представления
в секции \ref{section: Basis of representation}.

Мы будем записывать элементы башни представлений
\ShowEq{tower of representations}
в виде кортежа
\ShowEq{elements of tower of representations}
\ePrints{0906.0135}
\ifx\Semafor\ValueOn
Эту запись можно интерпретировать как
\ShowEq{notation for representation in representation f23}
В тоже время эта запись имеет дополнительный смысл. Например,
в аффинном пространстве $a_3$ - это точка пространства, $a_2$
- вектор, определяющий преобразование параллельного переноса.
Таким образом, мы можем интерпретировать кортеж $(a_2,a_3)$
либо как вектор $a_2$ с началом в точке $a_3$, либо как конец
этого вектора.
\fi

\begin{definition}
Пусть $(\Vector A,\Vector f)$ -
башня представлений.
Кортеж множеств
\ShowEq{tuple of sets 2 n}
называется
\AddIndex{кортежем стабильных множеств башни представлений}
{tuple of stable sets of tower of representations}
$\Vector f$,
если
\ShowEq{tuple of sets 2 n, 1}
для любых
\ShowEq{tuple of sets 2 n, 2}
Мы также будем говорить, что кортеж множеств
\ShowEq{tuple of sets 2 n}
стабилен относительно башни представлений
$\Vector f$.
\qed
\end{definition}

\begin{theorem}%
\label{theorem: tower of subrepresentations}
Пусть
$\Vector f$
- башня представлений.
Пусть множество $N_i\subset A_i$ является
подалгеброй $\Omega_i$\Hyph алгебры $A_i$, $i=2$, ..., $n$.
Пусть кортеж множеств
\ShowEq{tuple of sets 2 n}
стабилен относительно башни представлений
$\Vector f$.
Тогда существует башня представлений
\ShowEq{tower of subrepresentations}
такая, что
\ShowEq{representation of algebra A in tuple N 2 n, 1}
Башня представлений
\EqRef{tower of subrepresentations}
называется
\AddIndex{башней подпредставлений}
{tower of subrepresentations}.
\end{theorem}
\begin{proof}
Пусть $\omega_{i-1,1}$ - $m$\Hyph арная операция
$\Omega_{i-1}$\Hyph алгебры $A_{i-1}$, $i=2$, ..., $n$.
Тогда для любых
\ShowEq{tower of subrepresentations, a i-1}\footnote{Положим
$N_1=A_1$.}
и любого $a_i\in N_i$
\ShowEq{tower of subrepresentations, a i-1 omega}
Пусть $\omega_{i,2}$ - $m$\Hyph арная операция
$\Omega_i$\Hyph алгебры $A_i$, $i=2$, ..., $n$.
Тогда для любых
$a_{i,1}$, ..., $a_{i,n}\in N_i$
и любого $a_{i-1}\in N_{i-1}$
\ShowEq{tower of subrepresentations, a i omega}
Утверждение теоремы доказано.
\end{proof}

Из теоремы
\ref{theorem: tower of subrepresentations}
следует, что если отображение
\ShowEq{tower of subrepresentations, N}
- башня подпредставлений башни представлений
$\Vector f$,
то отображение
\ShowEq{tower of subrepresentations, n}
является морфизмом башен представлений.

\begin{theorem}%
Множество\footnote{Это определение
аналогично определению структуры подалгебр
(\citeBib{Cohn: Universal Algebra}, стр. 93, 94)}
\ShowEq{lattice of subrepresentations, tower of representations}
всех башен подпредставлений башни представлений
$\Vector f$
порождает
систему замыканий на башне представлений $\Vector f$
и, следовательно, является полной структурой.
\end{theorem}
\begin{proof}
Пусть для данного $\lambda\in\Lambda$,
$K_{\lambda,i}$, $i=2$, ..., $n$,
- подалгебра
$\Omega_i$\Hyph алгебры $A_i$,
стабильная относительно представления $f_{i-1,i}$.
Операцию пересечения на множестве $\mathcal B_{\Vector f}$
мы определим согласно правилу
\ShowEq{set of subrepresentations, intersection, tower}
$\cap K_{\lambda,i}$ - подалгебра
$\Omega_i$\Hyph алгебры $A_i$.
Пусть $a_i\in \cap K_{\lambda,i}$.
Для любого $\lambda\in\Lambda$ и для любого $a_{i-1}\in K_{i-1}$,
\ShowEq{set of subrepresentations, intersection, i, 1}
Следовательно,
\ShowEq{set of subrepresentations, intersection, i, 2}
Повторяя приведенное построение в порядке возрастания $i$,
$i=2$, ..., $n$, мы видим, что
$(K_1, ..., K_n)$ - кортеж стабильных множеств
башни представления $\Vector f$.
Следовательно, операция пересечения
башен подпредставлений определена корректно.
\end{proof}

Обозначим соответствующий оператор замыкания через
\ShowEq{closure operator, tower of representations}
Если мы обозначим через $\VX X$ кортеж множеств
\ShowEq{tuple of generating sets of tower of representations}
то
\ShowEq{tuple of generating sets of tower of representations, 1}
является пересечением всех кортежей
$(K_1,...,K_n)$,
стабильных относительно представления $\Vector f$
и таких, что для $i=2$, ..., $n$,
$K_i$ - подалгебра $\Omega_i$\Hyph алгебры $A_i$,
содержащая $X_i$.\footnote{При
$n=2$, $J_2(f_{1,2},X_2)=J_{f_{1,2}}(X_2)$.
Было бы проще использовать единные обозначения в разделах
\ref{section: Basis of representation} и
\ref{section: Basis of Tower of Representations}.
Однако использование векторных обозначений в разделе
\ref{section: Basis of representation}
мне кажется несвоевременным.}

\begin{theorem}%
\label{theorem: structure of subrepresentations in tower of representations}
Пусть\footnote{Утверждение теоремы аналогично
утверждению теоремы 5.1, \citeBib{Cohn: Universal Algebra}, стр. 94.}
$\Vector f$ - башня представлений.
Пусть
\ShowEq{structure of subrepresentations in representation, 1}
Положим $Y_1=A_1$.
Последовательно увеличивая значение $i$, $i=2$, ..., $n$,
определим подмножества $X_{i,m}\subset A_i$ индукцией по $m$.
\ShowEq{structure of subrepresentations in representation, 2}
Для каждого значения $i$ положим
\ShowEq{structure of subrepresentations in representation, 3}
Тогда
\ShowEq{structure of subrepresentations in representation, 4}
\end{theorem}
\begin{proof}
Для каждого значения $i$ доказательство теоремы
совпадает с доказательством теоремы
\ref{theorem: structure of subrepresentations}.
Так как для определения устойчивого подмножества
$\Omega_i$\Hyph алгебры $A_i$
нас интересует только некоторое устойчивое подмножество
$\Omega_{i-1}$\Hyph алгебры $A_{i-1}$,
мы должны сперва найти устойчивое  подмножество
$\Omega_{i-1}$\Hyph алгебры $A_{i-1}$.
\end{proof}

\ShowEq{subrepresentation generated by tuple of sets}
называется
\AddIndex{башней подпредставлений башни представлений $\Vector f$,
порождённой кортежем множеств $\VX X$}
{subrepresentation generated by tuple of sets},
а $\VX X$ -
\AddIndex{кортежем множеств образующих башни подпредставлений
$\VJfX$}
{tuple of generating sets of tower subrepresentations}.
В частности,
\AddIndex{кортеж множеств образующих башни представлений $\Vector f$}
{tuple of generating sets of tower of representations}
будет такой кортеж
\ShowEq{tuple of generating sets of tower of representations},
что $\VJfX=\Vector A$.

Нетрудно видеть, что определение кортежа множеств образующих
башни представлений не зависит от того,
эффективны представления башни или нет.
Поэтому в дальнейшем мы будем предполагать, что
представления башни эффективны и будем опираться на соглашение
для эффективного представления в замечании
\ref{remark: notation for effective representation of algebra}.

Мы также будем пользоваться записью
\ShowEq{endomorphism image, tower of effective representations}
для образа кортежа элементов
\ShowEq{tuple of sets 2 n, 3}
при эндоморфизме башни эффективных представлений.
Согласно определению произведения отображений,
для любых эндоморфизмов $\VX r$, $\VX s$ верно равенство
\ShowEq{endomorphism image, 1, tower of effective representations}
Равенство
\EqRef{endomorphism image, 1, tower of effective representations}
является законом ассоциативности для $\circ$ и позволяет
записать выражение
\ShowEq{endomorphism image, 2, tower of effective representations}
без использования скобок.

Из теоремы \ref{theorem: structure of subrepresentations in tower of representations}
следует следующее определение.

\begin{definition}
\label{definition: words of element, tower of representations}
Пусть
\ShowEq{tuple of generating sets of tower of representations}
- кортеж множеств.
Для любого кортежа элементов
\ShowEq{words of element, tower of representations, x in X}
существует
кортеж $\Vector{\Omega}$\Hyph слов,
определённых согласно следующему правилу.
\begin{enumerate}
\item Если $a_1\in A_1$,
то $a_1$ - $\Omega_1$\Hyph слово.
\label{words of element, tower of representations, a1}
\item Если $a_i\in X_i$, $i=2$, ..., $n$,
то $a_i$ - $\Omega_i$\Hyph слово.
\label{words of element, tower of representations, ai}
\item Если $a_{i,1}$, ..., $a_{i,p}$
- $\Omega_i$\Hyph слова, $i=2$, ..., $n$, и
$\omega\in\Omega_i(p)$, то $a_{i,1}...a_{i,p}\omega$
- $\Omega_i$\Hyph слово.
\label{words of element, tower of representations, omega i}
\item Если $a_i$ - $\Omega_i$\Hyph слово, $i=2$, ..., $3$, и
$a_{i-1}$ - $\Omega_{i-1}$\Hyph слово, то $a_{i-1}a_i$
- $\Omega_i$\Hyph слово.
\label{words of element, tower of representations, a i-1 i}
\end{enumerate}
\AddIndex{Кортеж $\Vector{\Omega}$\Hyph слов}
{tuple of words relative to tuple of generating sets, tower of representations}\footnote{Согласно
построению
\ShowEq{words of element, tower of representations, 1}
}
\ShowEq{words of element, tower of representations}
представляет данный элемент $\Vector a\in\VJfX$.\footnote{Эти обозначения
имеют небольшое различие с обозначениями,
предложенными ранее в теории представлении универсальной алгебры.
А именно, в кортеж $\Vector\Omega$\Hyph слов мы добавили слово
$\Omega_1$\Hyph алгебры. Однако очевидно,
что это слово всегда тривиально
\ShowEq{trivial omega1 word}
}
Обозначим
\ShowEq{word set of tower of representations}
\AddIndex{множество кортежей $\Vector\Omega$\Hyph слов
башни представлений $\VJfX$}
{word set of tower of representations}.
\qed
\end{definition}

Представление $a_i\in A_i$ в виде $\Omega_i$\Hyph слова неоднозначно.
Если $a_{i,1}$, ..., $a_{i,p}$ - $\Omega_i$\Hyph слова,
$\omega\in\Omega_i(p)$ и $a_{i-1}\in A_{i-1}$,
то $\Omega_i$\Hyph слова
$a_{i-1}a_{i,1}...a_{i,p}\omega$ и $a_{i-1}a_{i,1}...a_{i-1}a_{i,p}\omega$
описывают один и тот же
элемент $\Omega_i$\Hyph алгебры $A_i$.
Возможны равенства, связанные со спецификой представления.
Например, если $\omega$ является операцией
$\Omega_{i-1}$\Hyph алгебры $A_{i-1}$ и операцией
$\Omega_i$\Hyph алгебры $A_i$, то мы можем потребовать,
что $\Omega_i$\Hyph слова
$a_{i-1,1}...a_{i-1,p}\omega a_i$ и $a_{i-1,1}a_i...a_{i-1,p}a_i\omega$
описывают один и тот же
элемент $\Omega_i$\Hyph алгебры $A_i$.
Перечисленные выше равенства
для каждого значения $i$, $i=2$, ..., $n$,
определяют отношение эквивалентности
$r_i$ на множестве $\Omega_i$\Hyph слов
$W_i(\VfVX)$.% Фактор $\Omega_k$\Hyph алгебра
%$W_k/r_k$
%совпадает с $\Omega_k$\Hyph алгеброй $A_k$.
Согласно построению, отношение эквивалентности
$r_i$ на множестве $\Omega_i$\Hyph слов
$W_i(\VfVX)$ зависит не только от выбора множества
$X_i$, но и от выбора множества $X_{i-1}$.

%Вообще говоря, представление произвольного элемента $a_k\in A_k$
%в множестве $W_k/r_k$ неоднозначно.
%Если кортеж множеств образующих $\VX X$ таков, что представление
%элемента $a_k\in A_k$
%в множестве $W_k/r_k$ однозначно для любого $k$, $k=2$, $3$,
%то кортеж $X_*$ называется
%\AddIndex{базисом представления}
%{basis of representation in representation}
%$\Vector f$.

\begin{theorem}
\label{theorem: map of words of tower of representations}
Эндоморфизм $\VX r$ башни представлений
$\Vector f$
порождает отображение $\VX\Omega$\Hyph слов
\ShowEq{map of words of tower of representations}
такое, что для любого $i$, $i=2$, ..., $n$,
\begin{enumerate}
\item Если
\ShowEq{map of coordinates of tower of representations, a in X, 1}
то
\ShowEq{map of words of tower of representations, a in X}
\item Если
\ShowEq{map of words of tower of representations, omega, 1}
то для операции
$\omega\in\Omega_i(p)$ справедливо
\ShowEq{map of words of tower of representations, omega}
\item Если
\ShowEq{map of words of tower of representations, am, 1}
то
\ShowEq{map of words of tower of representations, am}
\end{enumerate}
\end{theorem}
\begin{proof}
Утверждения
\eqref{theorem: map of words of tower of representations, a in X},
\eqref{theorem: map of words of tower of representations, omega}
теоремы справедливы в силу определения эндоморфизма $r_i$.
Утверждение
\eqref{theorem: map of words of tower of representations, am}
теоремы следует из равенства
\EqRef{morphism of tower of representations, levels k k+1}.
\end{proof}

\begin{remark}
\label{remark: coordinates of tower of representations}
Пусть $\VX r$ - эндоморфизм башни представлений $\Vector f$.
Пусть
\ShowEq{map of words of tower of representations 1}
Теорема
\ref{theorem: map of words of tower of representations}
утверждает, что
\ShowEq{map of words of tower of representations 2}.
Теорема
\ref{theorem: map of words of tower of representations}
также утверждает, что
$\VX\Omega$\Hyph слово, представляющее $\VX a$, относительно $\VX X$ и
$\VX\Omega$\Hyph слово, представляющее $\VX a'$, относительно $\VX X'$
формируются согласно одному и тому же алгоритму.
Это позволяет рассматривать множество $\VX\Omega$\Hyph слов $\VX w(\VfVX',\VX a')$
как отображение
\ShowEq{coordinates of tower of representations 3}
такое, что, если для некоторого эндоморфизма $\VX r$
\ShowEq{coordinates of tower of representations 4}
то
\ShowEq{coordinates of tower of representations 5}
Кортеж отображений\footnote{Согласно
построению
\ShowEq{coordinates of element, tower of representations, 1}
Нас не интересует отображение $W_1(\Vector f,\Vector X,a_1)$
поскольку оно тривиально
\ShowEq{W1(a1)=a1}
}
\ShowEq{coordinates of element, tower of representations}
представляющий данный элемент $\Vector a\in\VJfX$, называется
\AddIndex{кортежем координат элемента $\Vector a$ относительно кортежа
множеств $\VX X$}
{coordinates of element, tower of representations}.
Обозначим
\ShowEq{coordinate set of tower of representations}
\AddIndex{множество кортежей координат
башни представлений $\VJfX$}
{coordinate set of tower of representations}.
Аналогично, мы можем рассмотреть координаты кортежа множеств
\ShowEq{subset of tower of representations}
относительно кортежа множеств $\VX X$
\ShowEq{subset of coordinates of tower of representations}
\qed
\end{remark}

\begin{theorem}
\label{theorem: set of coordinates, tower of representations, omega}
На множестве координат $W_k(\VfVX)$ определена структура $\Omega_k$\Hyph алгебры.
\end{theorem}
\begin{proof}
Пусть $\omega\in\Omega_k(n)$. Тогда для любых
\ShowEq{set of coordinates, 1k, omega}
положим
\ShowEq{set of coordinates, k, omega}
Согласно замечанию
\ref{remark: coordinates of tower of representations},
из равенства
\EqRef{set of coordinates, k, omega}
следует
\ShowEq{set of coordinates, 2k, omega}
Согласно правилу
\eqref{words of element, tower of representations, omega i}
определения
\ref{definition: words of element, tower of representations},
из равенства
\EqRef{set of coordinates, 2k, omega}
следует
\ShowEq{set of coordinates, 3k, omega}
Из равенства
\EqRef{set of coordinates, 3k, omega}
следует корректность определения
\EqRef{set of coordinates, k, omega}
операции $\omega$ на множестве координат $W_k(\VfVX)$.
\end{proof}

\begin{theorem}
\label{theorem: set of coordinates, tower of representations, am}
Для $k=2$, ..., $n$,
определено представление $\Omega_{k-1}$\Hyph алгебры $W_{k-1}(\VfVX)$
в $\Omega_k$\Hyph алгебре $W_k(\VfVX)$.\footnote{Согласно равенству
\EqRef{W1(a1)=a1},
мы можем отождествить $\Omega_1$\Hyph алгебры $W_1(\VfVX)$ и $A_1$.}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{set of coordinates, 1 k-1, am}
Тогда для любого
\ShowEq{set of coordinates, 1 k, am}
положим
\ShowEq{set of coordinates, am k}
Согласно замечанию
\ref{remark: coordinates of tower of representations},
из равенства
\EqRef{set of coordinates, am k}
следует
\ShowEq{set of coordinates, 2, am k}
Согласно правилу
\eqref{words of element, tower of representations, a i-1 i}
определения
\ref{definition: words of element, tower of representations},
из равенства
\EqRef{set of coordinates, 2, am k}
следует
\ShowEq{set of coordinates, 3, am k}
Из равенства
\EqRef{set of coordinates, 3, am k}
следует корректность определения
\EqRef{set of coordinates, am k}
представления $\Omega_{k-1}$\Hyph алгебры $W_{k-1}(\VfVX)$
в $\Omega_k$\Hyph алгебре $W_k(\VfVX)$.
\end{proof}

\begin{corollary}
\label{corollary: set of coordinates, tower of representations, am}
Кортеж $\Vector\Omega$\Hyph алгебр $\Vector W(\VfVX)$
порождает башню представлений.
\qed
\end{corollary}

\ePrints{0906.0135}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: map of words of tower of representations, 1}
Пусть
$\Vector f$
- башня представлений.
Для заданных множеств
\ShowEq{map of coordinates of tower of representations, Xk}
рассмотрим кортеж отображений
\ShowEq{map of coordinates of tower of representations, R}
таких, что для любого $k=2$, ..., $n$, отображение
\ShowEq{map of coordinates of tower of representations, Rk}
согласовано со структурой представления $f_{k-1,k}$,
т. е.\footnote{Мы полагаем $X_1=A_1$, $R_1(a_1)=a_1$.}
\ShowEq{map of words of tower of representations, 1k}
Рассмотрим отображение $\VX\Omega$\Hyph слов
\ShowEq{map of words of tower of representations, W}
удовлетворяющее условиям
\eqref{theorem: map of words of tower of representations, a in X},
\eqref{theorem: map of words of tower of representations, omega},
\eqref{theorem: map of words of tower of representations, am}
теоремы
\ref{theorem: map of words of tower of representations},
и такое, что
\ShowEq{map of words of tower of representations, W in X}
Для каждого $k$, $k=2$, ..., $n$, существует эндоморфизм $\Omega_k$\Hyph алгебры $A_k$
\ShowEq{map of coordinates of tower of representations, r}
определённый правилом
\ShowEq{endomorphism based on map of words of tower of representations}
Кортеж эндоморфизмов $\VX r$ является морфизмом башен представлнений
$\VJfX$ и $\Vector J(\VfVX')$.
\end{theorem}
\begin{proof}
При $n=2$ башня представлений $\Vector f$ является представлением
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Утверждение теоремы является следствием теоремы
\ref{theorem: map of words of representation, 1}.

Пусть утверждение теоремы верно для $n-1$.
Обозначения в теореме не меняются при переходе от
одного уровня к другому, так как слово в
$\Omega_{n-1}$\Hyph алгебре $A_{n-1}$
не зависит от слова в
$\Omega_n$\Hyph алгебре $A_n$.
Мы будем доказывать теорему индукцией по сложности
$\Omega_n$\Hyph слова.

Если
\ShowEq{map of words of tower of representations, w(a)=a}
то $a_n\in X_n$.
Согласно условию
\eqref{theorem: map of words of tower of representations, a in X}
теоремы
\ref{theorem: map of words of tower of representations},
\ShowEq{map of words of tower of representations, r(a)=R(a)}
Следовательно, на множестве $X_n$ отображения $r_n$ и $R_n$ совпадают,
и отображение $r_n$ согласовано со структурой $\Omega_n$\Hyph
алгебры.

Пусть $\omega\in\Omega_n(p)$.
Пусть предположение индукции верно для
\ShowEq{map of words of tower of representations, r(a), omega, 1}
Пусть
\ShowEq{map of words of tower of representations, r(a), omega, 2}
Если
\ShowEq{map of words of tower of representations, r(a), omega, 3}
то согласно условию
\eqref{words of element, tower of representations, omega i}
определения
\ref{definition: words of element, tower of representations},
\ShowEq{map of words of tower of representations, r(a), omega, 4}
Согласно условию
\eqref{theorem: map of words of tower of representations, omega}
теоремы
\ref{theorem: map of words of tower of representations},
\ShowEq{map of words of tower of representations, r(a), omega, 5}
Следовательно, отображение $r_n$ является эндоморфизмом
$\Omega_n$\Hyph алгебры $A_n$.

Пусть предположение индукции верно для
\ShowEq{map of words of tower of representations, r(a), a i-1 i, 1}
Согласно условию
\eqref{words of element, tower of representations, a i-1 i}
определения
\ref{definition: words of element, tower of representations},
\ShowEq{map of words of tower of representations, r(a), a i-1 i, 2}
Согласно условию
\eqref{theorem: map of words of tower of representations, am}
теоремы
\ref{theorem: map of words of tower of representations},
\ShowEq{map of words of tower of representations, r(a), a i-1 i, 3}
Из равенства
\EqRef{morphism of tower of representations, levels k k+1}
следует, что отображение $\Vector r$ является морфизмом
башни представлений $\Vector f$.
\end{proof}

\begin{remark}
Теорема \ref{theorem: map of words of tower of representations, 1}
- это теорема о продолжении отображения.
Единственное, что нам известно о кортеже множеств $\VX X$ - это то, что
$\VX X$ - кортеж множеств образующих башни представлений $\Vector f$.
Однако, между элементами множества $X_k$, $k=2$, ..., $n$, могут существовать соотношения,
порождённые либо операциями $\Omega_k$\Hyph алгебры $A_k$, либо
преобразованиями представления $f_{k-1,k}$.
Поэтому произвольное отображение кортежа множеств $\VX X$, вообще говоря,
не может быть продолжено до эндоморфизма башни представлений $\Vector f$.\footnote{В
теореме
\ref{theorem: automorphism uniquely defined by image of basis, tower of representations},
требования к кортежу множеств образующих более жёсткие. Поэтому теорема
\ref{theorem: automorphism uniquely defined by image of basis, tower of representations}
говорит о продолжении произвольного отображения.
Более подробный анализ дан в замечании
\ref{remark: automorphism uniquely defined by image of basis, tower of representations}.}
Однако, если
для каждого $k$, $k=2$, ..., $n$,
отображение $R_k$ согласованно со структурой представления
$f_{k-1,k}$, то мы можем построить продолжение этого отображения,
которое является эндоморфизмом башни представлений $\Vector f$.
\qed
\end{remark}
\fi

\begin{definition}
Пусть $\VX X$ - кортеж множеств образующих башни представлений $\Vector f$.
Пусть $\VX r$ - эндоморфизм башни представлений $\Vector f$.
Множество координат
\ShowEq{coordinates of endomorphism, 2, tower of representations}
называется
\AddIndex{координатами эндоморфизма башни представлений}
{coordinates of endomorphism, tower of representations}.
\qed
\end{definition}

\begin{definition}
\label{definition: superposition of coordinates, tower of representations}
Пусть $\VX X$ - кортеж множеств образующих башни представлений $\Vector f$.
Пусть $\VX r$ - эндоморфизм башни представлений $\Vector f$.
Пусть $\VX a\in\VX A$.
Мы определим
\AddIndex{суперпозицию координат}
{superposition of coordinates, tower of representations}
эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$
как координаты, определённые согласно правилу
\ShowEq{superposition of coordinates, tower of representations}
Пусть $\VX Y\subset\VX A$.
Мы определим
суперпозицию координат
эндоморфизма башни представлений $\Vector f$ и кортежа множеств $\VX Y$
согласно правилу
\ShowEq{superposition of coordinates, 1, tower of representations}
\qed
\end{definition}

\begin{theorem}
\label{theorem: map of coordinates of tower of representations}
Эндоморфизм $\VX r$ представления
$\Vector f$
порождает отображение координат башни представлений
\ShowEq{map of coordinates of tower of representations}
такое, что
\ShowEq{map of coordinates of tower of representations, 1}
\end{theorem}
\begin{proof}
Согласно замечанию
\ref{remark: coordinates of tower of representations},
мы можем рассматривать равенства
\EqRef{superposition of coordinates, tower of representations},
\EqRef{map of coordinates of tower of representations}
относительно заданного кортежа множеств образующих $\VX X$.
При этом координатам $\VX W(\VfVX,\VX a)$ соответствует кортеж слов
\ShowEq{map of coordinates of tower of representations, 2}
а координатам $\VX W(\VfVX,\VX r\circ\VX a)$ соответствует кортеж слов
\ShowEq{map of coordinates of tower of representations, 3}
Поэтому для того, чтобы доказать теорему,
нам достаточно показать, что отображению $\WVXR$
соответствует отображение $\wVXR$.
Мы докажем утверждение индукцией по числу $n$ универсальных алгебр в башне представлений.

При $n=2$ башня представлений $\Vector f$ является представлением
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Утверждение теоремы является следствием теоремы
\ref{theorem: map of coordinates of representation}.
Пусть утверждение теоремы верно для $n-1$.
Мы будем доказывать теорему индукцией по сложности
$\Omega_n$\Hyph слова.

Если
\ShowEq{map of words of tower of representations, a in X, 1}
то, согласно равенствам
\EqRef{map of coordinates of tower of representations, 2},
\EqRef{map of coordinates of tower of representations, 3},
отображения $W_n[\VfVX,\VX r]$ и $w_n[\VfVX,\VX r]$ согласованы.

Пусть для
\ShowEq{superposition of coordinates, tower of representations, omega, 1}
отображения $W_n[\VfVX,\VX r]$ и $w_n[\VfVX,\VX r]$ согласованы.
Пусть $\omega\in\Omega_n(p)$.
Согласно теореме
\ref{theorem: set of coordinates, representation, omega}
\ShowEq{superposition of coordinates, tower of representations, omega, 2}
Так как $r_n$ - эндоморфизм $\Omega_n$\Hyph алгебры $A_n$,
то из равенства
\EqRef{superposition of coordinates, tower of representations, omega, 2}
следует
\ShowEq{superposition of coordinates, tower of representations, omega, 3}
Из равенств
\EqRef{superposition of coordinates, tower of representations, omega, 2},
\EqRef{superposition of coordinates, tower of representations, omega, 3}
и предположения индукции следует, что
отображения $W_n[\VfVX,\VX r]$ и $w_n[\VfVX,\VX r]$ согласованы для $a_n=a_{n,1}...a_{n,p}\omega$.

Пусть для
$a_{n,1}\in A_n$
отображения $W_n[\VfVX,\VX r]$ и $w_n[\VfVX,\VX r]$ согласованы.
Пусть $a_{n-1}\in A_{n-1}$.
Согласно теореме
\ref{theorem: set of coordinates, tower of representations, am}
\ShowEq{superposition of coordinates, tower of representations, a n n-1, 1}
Так как $\VX r$ - эндоморфизм башни представлений $\Vector f$,
то из равенства
\EqRef{superposition of coordinates, tower of representations, a n n-1, 1}
следует
\ShowEq{superposition of coordinates, tower of representations, a n n-1, 2}
Из равенств
\EqRef{superposition of coordinates, tower of representations, a n n-1, 1},
\EqRef{superposition of coordinates, tower of representations, a n n-1, 2}
и предположения индукции следует, что
отображения $W_n[\VfVX,\VX r]$ и $w_n[\VfVX,\VX r]$ согласованы для
$a_{n,2}=a_{n-1}a_{n,1}$.
\end{proof}

\begin{corollary}
\label{corollary: map of coordinates of tower of representations}
Пусть $\VX X$ - кортеж множеств образующих башни представлений $\Vector f$.
Пусть $\VX r$ - эндоморфизм башни представлений $\Vector f$.
Отображение $\WVXR$ является эндоморфизмом башни представлений $\Vector W(\VfVX)$.
\qed
\end{corollary}

В дальнейшем мы будем отождествлять отображение $\WVXR$
и множество координат $\VX W(\VfVX,\VX r\circ\VX X)$.

\begin{theorem}
Пусть $\VX X$ - кортеж множеств образующих башни представлений $\Vector f$.
Пусть $\VX r$ - эндоморфизм башни представлений $\Vector f$.
Пусть $\VX Y\subset\VX M$.
Тогда
\ShowEq{superposition of coordinates, 2, tower of representations}
\end{theorem}
\begin{proof}
Равенство
\EqRef{superposition of coordinates, 2, tower of representations}
является следствием равенства
\ShowEq{superposition of coordinates, 3, tower of representations}
а также равенств
\EqRef{superposition of coordinates, tower of representations},
\EqRef{superposition of coordinates, 1, tower of representations}.
Равенство
\EqRef{superposition of coordinates, 2a, tower of representations}
является следствием равенств
\EqRef{superposition of coordinates, 2, tower of representations},
\EqRef{map of coordinates of tower of representations, 1}.
\end{proof}

\begin{theorem}
Пусть $\VX X$ - кортеж множеств образующих башни представлений $\Vector f$.
Пусть $\VX r$, $\VX s$ - эндоморфизмы башни представлений $\Vector f$.
Тогда
\ShowEq{superposition of coordinates, 4, tower of representations}
\end{theorem}
\begin{proof}
Равенство
\EqRef{superposition of coordinates, 4, tower of representations}
следует из равенства
\EqRef{superposition of coordinates, 2, tower of representations},
если положить $\VX Y=\VX s\circ\VX X$.
Равенство
\EqRef{superposition of coordinates, 4a, tower of representations}
следует из равенства
\EqRef{superposition of coordinates, 4, tower of representations}
и цепочки равенств
\ShowEq{superposition of coordinates, 4b, tower of representations}
\end{proof}

Мы можем обобщить определение суперпозиции координат и предположить,
что один из множителей является кортежем множеств $\VX\Omega$\Hyph слов.
Соответственно, определение суперпозиции координат имеет вид
\ShowEq{superposition of coordinates, 5, tower of representations}

Следующие формы записи образа кортежа множеств $\VX Y$
при эндоморфизме $\VX r$ эквивалентны.
\ShowEq{superposition of coordinates, 6, tower of representations}
Из равенств
\EqRef{superposition of coordinates, 2, tower of representations},
\EqRef{superposition of coordinates, 6, tower of representations}
следует, что
\ShowEq{superposition of coordinates, 7, tower of representations}
Равенство
\EqRef{superposition of coordinates, 7, tower of representations}
является законом ассоциативности для операции композиции и позволяет
записать выражение
\ShowEq{superposition of coordinates, 8, tower of representations}
без использования скобок.

\begin{definition}
\label{definition: endomorphism of representation, regular on tuple}
Пусть
\ShowEq{tuple of generating sets of tower of representations}
- кортеж множеств образующих башни представлений
$\Vector f$.
Пусть отображение
$\VX r$
является эндоморфизмом башни представления $\Vector f$.
Пусть кортеж множеств
\ShowEq{endomorphism of representation, regular on tuple}
является образом кортежа множеств $\VX X$
при отображении $\VX r$.
Эндоморфизм $\VX r$ башни представлений $\Vector f$ называется
\AddIndex{невырожденным на кортеже множеств образующих}
{endomorphism of representation, regular on tuple} $\VX X$,
если кортеж множеств $\VX X'$ является кортежем множеств образующих
башни представлений $\Vector f$.
В противном случае, эндоморфизм $\VX r$ называется
\AddIndex{вырожденным на кортеже множеств образующих}
{endomorphism of representation, singular on tuple} $\VX X$,
\qed
\end{definition}

\begin{definition}
\label{definition: regular endomorphism of tower of representations}
Эндоморфизм башни представлений $\Vector f$ называется
\AddIndex{невырожденным}
{regular endomorphism of tower of representations},
если он невырожден на любом кортеже множеств образующих.
\qed
\end{definition}

\begin{theorem}
\label{theorem: Automorphism of tower of representations is regular endomorphism}
Автоморфизм $\Vector r$ башни представлений
$\Vector f$
является невырожденным эндоморфизмом.
\end{theorem}
\begin{proof}
Пусть $\VX X$ - кортеж множеств образующих
башни представлений $\Vector f$.
Пусть $\VX X'=\VX r\circ\VX X$.

Согласно теореме
\ref{theorem: map of coordinates of tower of representations}
эндоморфизм $\VX r$
порождает отображение  $\VX\Omega$\Hyph слов
$\VX w[\VfVX,\VX r]$.

Пусть $\VX a'\in\VX A$. Так как $\VX r$
- автоморфизм, то существует
\ShowEq{Automorphism of tower of representations is regular endomorphism, 0}
Согласно определению
\ref{definition: words of element, tower of representations},
$\VX w(\VfVX,\VX a)$ - кортеж $\VX\Omega$\Hyph слов, представляющих
$\VX a$ относительно кортежа множеств образующих $\VX X$.
Согласно теореме
\ref{theorem: map of coordinates of tower of representations},
$\VX w(\VfVX',\VX a')$ - кортеж $\VX\Omega$\Hyph слов, представляющих
$\VX a'$ относительно кортежа множеств $\VX X'$
\ShowEq{Automorphism of tower of representations is regular endomorphism, 1}
Следовательно, $\VX X'$ - множество образующих представления $\Vector f$.
Согласно определению
\ref{definition: regular endomorphism of tower of representations},
автоморфизм $\VX r$ - невырожден.
\end{proof}

\section{Базис башни представлений}
\label{section: Basis of Tower of Representations}

\begin{definition}
Если кортеж множеств $\VX X$ является
кортежем множеств образующих башни представлений
$\Vector f$, то любой кортеж множеств $\VX Y$,
$X_i\subset Y_i\subset A_i$, $i=2$, ..., $n$,
также является кортежем множеств образующих башни представлений $\Vector f$.
Если существует кортеж минимальных множеств $\VX X$, порождающих
башню представлений $\Vector f$,
то такой кортеж множеств $\VX X$ называется
\AddIndex{базисом башни представлений}
{basis of tower of representations}
$\Vector f$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: X is basis of tower of representations}
Базис башни представлений определён индукцией по $n$.
При $n=2$ базис башни представлений является базисом
представления $f_{1,2}$.
Если кортеж множеств $\Vector X_{[1,n]}$
является базисом башни представлений $\VX f$,
то кортеж множеств образующих $\VX X$ башни представлений
$\Vector f$ является базисом
тогда и только тогда, когда для любого $a_n\in X_n$
кортеж множеств $(X_2,...,X_{n-1},X_n\setminus\{a_n\})$ не является
кортежем множеств образующих башни представлений $\Vector f$.
\end{theorem}
\begin{proof}
При $n=2$ утверждение теоремы является следствием теоремы
\ref{theorem: X is basis of representation}.

Пусть $n>2$.
Пусть $\VX X$ - кортеж множеств образующих
башни расслоений $\Vector f$.
Пусть кортеж множеств $\Vector X_{[1,n]}$
является базисом башни расслоений $\Vector f_{[n]}$.
Допустим для некоторого $a_n\in X_n$ существует слово
\ShowEq{X is basis of tower of representations, 1}
Рассмотрим $a'_n\in A_n$, для
которого слово
\ShowEq{X is basis of tower of representations, 2}
зависит от $a_n$.
Согласно определению
\ref{definition: word of element relative to set, representation},
любое вхождение $a_n$ в слово $w'_n$ может быть заменено словом
$w_n$. Следовательно, слово $w'_n$ не зависит от $a_n$,
а кортеж множеств $(X_2,...,X_{n-1},X_n\setminus\{a_n\})$ является
кортежем множеств образующих башни представлений $\Vector f$.
Следовательно, $\VX X$ не является базисом башни представлений $\Vector f$.
\end{proof}

\begin{remark}
\label{remark: X is basis of tower of representations}
Доказательство теоремы
\ref{theorem: X is basis of tower of representations}
даёт нам эффективный метод построения базиса
башни представлений $\Vector f$.
Мы начинаем строить базис в самом нижнем слое.
Когда базис построен в слое $i$, $i=2$, ..., $n-1$,
мы можем перейти к построению базиса в слое $i+1$.
\qed
\end{remark}

\begin{remark}
Мы будем записывать базис также в виде 
\ShowEq{notation for basis of tower of representations 1}
Если базис - конечный, то мы будем также пользоваться записью
\ShowEq{notation for basis of tower of representations 2}
\qed
\end{remark}

\begin{remark}
Координаты $a_k\in A_k$ относительно базиса $\VX X$ башни представлений $\Vector f$
определены неоднозначно.
Так же как в замечании
\ref{remark: equivalence of representation},
мы рассмотрим 
\AddIndex{кортеж отношений эквивалентности $\VX\rho(\Vector f)$,
порождённых башней представлений $\Vector f$}
{tuple of equivalence of tower of representations}.
Если в процессе построений мы получим равенство двух $\Omega_k$\Hyph слов
относительно заданного базиса, мы можем утверждать, что эти $\Omega_k$\Hyph слова равны,
не заботясь об отношении эквивалентности
$\rho_k(\Vector f)$.
\qed
\end{remark}

\begin{theorem}
\label{theorem: Automorphism of tower of representations maps a basis into basis}
Автоморфизм башни представлений $\Vector f$ отображает базис
башни представлений $\Vector f$ в базис.
\end{theorem}
\begin{proof}
При $n=2$ утверждение теоремы является следствием теоремы
\ref{theorem: Automorphism of tower of representations maps a basis into basis}.

Пусть отображение $\Vector r$ - автоморфизм
башни представлений $\Vector f$.
Пусть кортеж множеств $\VX X$
- базис башни представлений $\Vector f$.
Пусть $\VX X'=\VX r(\VX X)$.

Допустим кортеж множеств $\VX X'$ не является базисом.
Согласно теореме
\ref{theorem: X is basis of tower of representations}
существуют $i$, $i=2$, ..., $n$,
и $a_i'\in X'_i$ такие, что кортеж множеств
\ShowEq{map of basis of tower of representations, 1}
является кортежем множеств образующих
башни представлений $\Vector f$.
Согласно теореме
\ref{theorem: group of automorphisms of tower of representations}
отображение $\Vector r^{-1}$ является автоморфизмом
башни представлений $\Vector f$.
Согласно теореме
\ref{theorem: Automorphism of tower of representations is regular endomorphism}
и определению
\ref{definition: regular endomorphism of tower of representations},
кортеж множеств
\ShowEq{map of basis of tower of representations, 2}
является кортежем множеств образующих
представления $\Vector f$.
Полученное противоречие доказывает теорему.
\end{proof}

\begin{theorem}
\label{theorem: automorphism uniquely defined by image of basis, tower of representations}
Пусть $\VX X$ - базис представления $\Vector f$.
Пусть
\ShowEq{VXR X->}
произвольное отображение кортежа множеств $\VX X$.
Рассмотрим отображение $\VX\Omega$\Hyph слов
\ShowEq{map of words of tower of representations, W}
удовлетворяющее условиям
\eqref{theorem: map of words of tower of representations, a in X},
\eqref{theorem: map of words of tower of representations, omega},
\eqref{theorem: map of words of tower of representations, am}
теоремы
\ref{theorem: map of words of tower of representations},
и такое, что
\ShowEq{map of words of tower of representations, W in X}
Существует единственный эндоморфизм представлнения $\Vector f$\footnote{Это утверждение
похоже на теорему \citeBib{Serge Lang}-1, с. 104.}
\ShowEq{VXr:A->A}
определённый правилом
\ShowEq{endomorphism VXr based on map of words of tower of representations}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\ref{theorem: map of words of representation},
\ref{theorem: map of words of representation, 1}.
\end{proof}

\begin{corollary}
\label{corollary: automorphism uniquely defined by image of basis, tower of representations}
Пусть $\VX X$, $\VX X'$ - базисы представления $\Vector f$.
Пусть $\VX r$ - автоморфизм представления $\Vector f$
такой, что
\ShowEq{endomorphism of representation, regular on tuple}.
Автоморфизм $\VX r$ определён однозначно.
\qed
\end{corollary}

\begin{remark}
\label{remark: automorphism uniquely defined by image of basis, tower of representations}
Теорема \ref{theorem: automorphism uniquely defined by image of basis, tower of representations},
так же как и
теорема \ref{theorem: map of words of tower of representations, 1},
является теоремой о продолжении отображения.
Одако здесь $\VX X$ - не произвольный кортеж множеств образующих башни представлений,
а базис.
Согласно замечаниям
\ref{remark: X is basis of tower of representations},
\ref{remark: X is basis of representation},
мы не можем определить координаты любого элемента базиса
через остальные элементы этого же базиса.
Поэтому отпадает необходимость в согласованности отображения базиса с представлением.
\qed
\end{remark}

\begin{theorem}
\label{theorem: coordinates of identity transformation, tower of representations}
Набор координат $\VX W(\VfVX,\VX X)$
соответствует тождественному преобразованию
\ShowEq{identity transformation, tower of representations}
\end{theorem}
\begin{proof}
Утверждение теоремы следует из равенства
\ShowEq{coordinates of identity transformation, tower of representations}
\end{proof}

\begin{theorem}
\label{theorem: coordinates of inverse transformation, tower of representations}
Пусть
\ShowEq{coordinates of endomorphism, 2, tower of representations}
- множество координат автоморфизма $\VX r$.
Определено множество координат
\ShowEq{coordinates of endomorphism, 3, tower of representations},
соответствующее
автоморфизму $\VX r^{-1}$. Множество координат
\ShowEq{coordinates of endomorphism, 3, tower of representations}
удовлетворяет равенству\footnote{Смотри
также замечание \ref{remark: coordinates of inverse transformation, representation}.}
\ShowEq{coordinates of inverse transformation, tower of representations}
\ShowEq{coordinates of inverse transformation, a, tower of representations}
\end{theorem}
\begin{proof}
Поскольку $\VX r$ - автоморфизм башни представлений $\Vector f$, то, согласно теореме
\ref{theorem: Automorphism of tower of representations maps a basis into basis},
множество
\ShowEq{coordinates of endomorphism, 4, tower of representations}
- базис башни представлений $\Vector f$. Следовательно, определено
множество координат
\ShowEq{coordinates of endomorphism, 3, tower of representations}.
Равенство
\EqRef{coordinates of inverse transformation, tower of representations}
следует из цепочки равенств
\ShowEq{coordinates of inverse transformation, 1, tower of representations}
\end{proof}

\begin{theorem}
Группа автоморфизмов $G(\Vector f)$
башни эффективных представлений $\Vector f$
порождает эффективное представление
в башне представлений $\Vector f$.
\end{theorem}
\begin{proof}
Из следствия
\ref{corollary: automorphism uniquely defined by image of basis, tower of representations}
следует, что если автоморфизм $\VX r$ отображает базис $\VX X$ в базис $\VX X'$,
то множество координат $\VX W(\VfVX,\VX X')$ однозначно определяет автоморфизм $\VX r$.
Из теоремы
\ref{theorem: map of coordinates of tower of representations}
следует, что
множество координат $\VX W(\VfVX,\VX X')$ определяет правило
отображения координат относительно
базиса $\VX X$ при автоморфизме башни представлений $\Vector f$.
Из равенства
\EqRef{superposition of coordinates, 6, tower of representations}
следует, что автоморфизм $\VX r$ действует справа на элементы
$\Omega_k$\Hyph алгебры $A_k$, $k=2$, ..., $n$.
Из равенства
\EqRef{superposition of coordinates, 4, tower of representations}
следует, что представление группы является \sT{T}представлением.
Согласно теореме
\ref{theorem: coordinates of identity transformation, tower of representations}
набор координат $\VX W(\VfVX,\VX X)$
соответствует тождественному преобразованию.
Из теоремы
\ref{theorem: coordinates of inverse transformation, tower of representations}
следует, что набор координат
\ShowEq{coordinates of endomorphism, 3, tower of representations}
соответствует преобразованию, обратному преобразованию $\VX W(\VfVX,\VX r\circ\VX X)$.
\end{proof}

\ePrints{0912.3315,0906.0135}
\ifx\Semafor\ValueOff
\section{Многообразие базисов башни представлений}

Множество
\ShowEq{basis manifold tower of representations}
базисов башни представлений $\Vector f$ называется
\AddIndex{многообразием базисов башни представлений $\Vector f$}
{basis manifold tower of representations}.

Согласно теореме
\ref{theorem: Automorphism of tower of representations maps a basis into basis},
автоморфизм $\VX R$ башни представлений $\Vector f$
порождает преобразование
\ShowEq{active transformation, tower of representations}
многообразия базисов башни представлений.
Это преобразование называется
\AddIndex{активным}{active transformation of basis, tower of representations}.
Согласно теореме
\ref{theorem: group of automorphisms of tower of representations},
определено
\AddIndex{активное представление}{active representation in basis manifold, tower of representations}
\ShowEq{active representation in basis manifold, tower of representations}
группы $G(\Vector f)$
в многообразии базисов $\mathcal B(\Vector f)$.
Согласно следствию
\ref{corollary: automorphism uniquely defined by image of basis, tower of representations},
это представление однотранзитивно.

\begin{remark}
Согласно замечанию
\ref{remark: X is basis of representation},
могут существовать базисы представления $f$, не связанные активным преобразованием.
В этом случае мы в качестве многообразия базисов будем рассматривать
орбиту выбранного базиса.
Следовательно, представление $f$ может иметь различные многообразия базисов.
Мы будем предполагать, что мы выбрали многообразие базисов.
\qed
\end{remark}

\begin{definition}
\label{definition: passive transformation of basis, tower of representations}
Автоморфизм $\VX s$ представления $A(\Vector f))$ называется
\AddIndex{пассивным преобразованием многообразия базисов башни представлений}
{passive transformation of basis, tower of representations}.
Мы будем пользоваться записью
\ShowEq{passive transformation of basis, tower of representations}
для обозначения образа базиса $\VX X$ при пассивном преобразовании $\VX s$.
\qed
\end{definition}

\begin{theorem}
Пассивное преобразование базиса имеет вид
\ShowEq{passive transformation, tower of representations}
\end{theorem}
\begin{proof}
Согласно равенству
\EqRef{active transformation, tower of representations},
активное преобразование действует на координаты
базиса справа.
Равенство
\EqRef{passive transformation, tower of representations}
следует из теорем
\ref{theorem: shift is automorphism of representation},
\ref{theorem: two representations of group},
\ref{theorem: twin representations of group, automorphism};
согласно которым
пассивное преобразование действует на координаты
базиса слева.
\end{proof}

\begin{theorem}
\label{theorem: select second basis of tower of representations}
Пусть $\VX s$ - пассивное преобразование
многообразия базисов представления $\Vector f$.
Пусть $\VX X$ - базис представления $\Vector f$,
\ShowEq{select second basis of tower of representations, 3}
Пусть для базиса $Y$ существует активное преобразование $\VX r$ такое,
что
\ShowEq{select second basis of tower of representations, 2}
Положим
\ShowEq{select second basis of tower of representations, 1}
Тогда
\ShowEq{select second basis of tower of representations, 4}
\end{theorem}
\begin{proof}
Согласно равенству
\EqRef{active transformation, tower of representations},
активное преобразование координат базиса $\VX Y$ имеет вид
\ShowEq{active transformation, tower of representations, 1}
Пусть
\ShowEq{select second basis of tower of representations, 5}
Из равенства
\EqRef{passive transformation, tower of representations}
следует, что
\ShowEq{passive transformation, tower of representations, 1}
Из совпадения выражений в равенствах
\EqRef{active transformation, tower of representations, 1},
\EqRef{passive transformation, tower of representations, 1}
следует, что
\ShowEq{passive and active maps, tower of representations, 1}
Следовательно, коммутативна диаграмма
\ShowEq{passive and active maps, tower of representations}
\end{proof}

\begin{theorem}
\label{theorem: passive representation in basis manifold, tower of representations}
Существует однотранзитивное
\AddIndex{пассивное представление}
{passive representation in basis manifold, tower of representations}
\ShowEq{passive representation in basis manifold, tower of representations}
\end{theorem}
\begin{proof}
Поскольку $A(\Vector f)$ - однотранзитивное представление группы $G(\Vector f)$,
то согласно определению
\ref{definition: passive transformation of basis, tower of representations}
и теореме
\ref{theorem: group of automorphisms of tower of representations},
множество пассивных преобразований порождает группу.
\end{proof}

Пусть пассивное преобразование $\VX s$ отображает базис $\VX Y$ в базис
\ShowEq{passive transformation s, tower of representations}
Пусть пассивное преобразование $\VX t$ отображает базис $\VX Y'$ в базис
\ShowEq{passive transformation t, tower of representations}
Обозначим
\ShowEq{passive transformation t s 0, tower of representations}
произведение пассивных преобразований $\VX t$ и $\VX s$
\ShowEq{passive transformation t s 1, tower of representations}
Из равенств
\EqRef{passive transformation s, tower of representations},
\EqRef{passive transformation t, tower of representations}
следует, что
\ShowEq{passive transformation t s 2, tower of representations}
Из равенств
\EqRef{passive transformation t s 1, tower of representations},
\EqRef{passive transformation t s 2, tower of representations}
и теоремы
\ref{theorem: passive representation in basis manifold, tower of representations}
следует, что
\ShowEq{passive transformation t s 3, tower of representations}

\section{Геометрический объект башни представлений}

Активное преобразование изменяет базисы и
элементы $\Vector\Omega$\Hyph алгебр согласовано
и координаты элемента относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к изменению
координат элемента относительно базиса.

Допустим пассивное преобразование $\VX s\in G(\Vector f)$ отображает
базис $\VX Y\in\mathcal B(\Vector f)$
в базис $\VX Y'\in\mathcal B(\Vector f)$
\ShowEq{passive transformation of tower of representations}
Допустим элемент $\VX a\in\VX A$ имеет $\VX\Omega$\Hyph слово
\ShowEq{Omega word in tower of representations, basis Y}
относительно базиса $\VX Y$ и имеет $\VX\Omega$\Hyph слово
\ShowEq{Omega word in tower of representations, basis Y prim}
относительно базиса $Y'$.
Из \EqRef{passive transformation of tower of representations}
и \EqRef{Omega word in tower of representations, basis Y prim} следует, что
\ShowEq{Omega word in tower of representations, basis Y, 1}
Сравнивая \EqRef{Omega word in tower of representations, basis Y}
и \EqRef{Omega word in tower of representations, basis Y, 1} получаем, что
\ShowEq{coordinate transformation in tower of representations, 1}
Так как $\VX s$ - автоморфизм башни представлений, то
из \EqRef{coordinate transformation in tower of representations, 1}
и теоремы
\ref{theorem: coordinates of inverse transformation, tower of representations}
следует
\ShowEq{coordinate transformation in tower of representations}
Преобразование координат \EqRef{coordinate transformation in tower of representations}
не зависит от элемента $\VX a$ или базиса $\VX Y$, а
определенно исключительно координатами элемента $\VX a$
относительно базиса $\VX Y$.

\begin{theorem}
Преобразования координат \EqRef{coordinate transformation in tower of representations}
порождают эффективное
\sT{T}представление группы $G(\Vector f)$, называемое
\AddIndex{координатным представлением в кортеже $\VX\Omega$\Hyph алгебр}
{coordinate tower of representations, Omega algebra}.
\end{theorem}
\begin{proof}
Согласно следствию
\ref{corollary: map of coordinates of tower of representations},
преобразование
\EqRef{coordinate transformation in tower of representations}
является эндоморфизмом башни представлений
$\Vector f$.\footnote{Это преобразование
не порождает эндоморфизма башни представлений $\Vector f$.
Координаты меняются, поскольку меняется
базис, относительно которого мы определяем координаты. Однако элемент
$\VX\Omega$\Hyph алгебры $\VX A$, координаты которого мы рассматриваем, не меняется.}

Допустим мы имеем два последовательных пассивных преобразования
$\VX s$ и $\VX t$. Преобразование координат
\EqRef{coordinate transformation in tower of representations}
соответствует пассивному преобразованию $\VX s$.
Преобразование координат
\ShowEq{coordinate transformation in tower of representations, t}
соответствует пассивному преобразованию $\VX t$.
Согласно теореме
\ref{theorem: W f,(SR)X,X},
произведение
преобразований координат \EqRef{coordinate transformation in tower of representations}
и \EqRef{coordinate transformation in tower of representations, t} имеет вид
\ShowEq{coordinate transformation in tower of representations, ts}
и является координатным преобразованием,
соответствующим пассивному преобразованию
\ShowEq{coordinate transformation in tower of representations, ts 1}
Это доказывает, что преобразования координат
порождают \sT{T}представление группы $G(\Vector f)$.

Если координатное преобразование не изменяет координаты выбранного базиса,
то ему соответствует единица группы $G(\Vector f)$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
\end{proof}

Пусть $(\Vector A,\Vector f)$ - башня представлений.
Пусть $(\Vector B,\Vector g)$ - башня представлений такая, что $A_1=B_1$.
Пассивное представление $P(\Vector g)$ согласовано
с пассивным представлением $P(\Vector f)$,
если существует гомоморфизм $h$ группы $G(\Vector f)$ в группу $G(\Vector g)$.
Рассмотрим диаграмму
\ShowEq{passive representation coordinated with passive representation, tower of representations}
Так как отображения $P(\Vector f)$, $P(\Vector g)$ являются изоморфизмами группы,
то отображение $H$ является гомоморфизмом групп.
Следовательно, отображение $f'$ является представлением группы $G(\Vector f)$
в многообразии базисов $\mathcal B(\Vector g)$.
Согласно построению, пассивному преобразованию $\VX s$
башни представлений $\Vector f$
соответствует пассивное преобразование $H(\VX s)$
башни представлений $\Vector g$.
\ShowEq{passive transformation of tower of representations g}
Тогда координатное преобразование в башне представлений $\Vector g$ принимает вид
\ShowEq{coordinate transformation, tower of representations g}

\begin{definition}
\label{definition: geometric object, coordinate representation, tower of representations g}
Мы будем называть орбиту
\ShowEq{geometric object, coordinate tower of representations g}%
\AddIndex{геометрическим объектом в координатном представлении,
определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}
{geometric object, coordinate tower of representations g}.
Для любого базиса
\ShowEq{geometric object 1, coordinate tower of representations}
соответствующая точка \EqRef{coordinate transformation, tower of representations g}
орбиты  определяет
\AddIndex{координаты геометрического объекта в координатном пространстве башни представлений}
{coordinates of geometric object, coordinate tower of representations}
относительно базиса
\ShowEq{geometric object 2, coordinate tower of representations}
\qed
\end{definition}

\begin{definition}
\label{definition: geometric object, tower of representations g}
Мы будем называть орбиту
\ShowEq{geometric object, tower of representations g}%
\AddIndex{геометрическим объектом, определённым в кортеже $\VX\Omega$\Hyph алгебр}
{geometric object, tower of representations g}
$\VX A$.
Для любого базиса
\ShowEq{geometric object 1, tower of representations}
соответствующая точка \EqRef{coordinate transformation, tower of representations g}
орбиты  определяет
\AddIndex{координаты геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}
{coordinates of geometric object, tower of representations g} $\VX A$
относительно базиса $Y'_M$
и соответствующий вектор
\ShowEq{geometric object 2, tower of representations g}%
называется
\AddIndex{представителем геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}
{representative of geometric object, tower of representations g}
$\VX A$.
\qed
\end{definition}

Так как геометрический объект - это орбита представления,
то согласно теореме
\ref{theorem: proper definition of orbit}
определение геометрического объекта корректно.

%Мы будем также говорить, что $\VX b$ - это
%\AddIndex{геометрический объект типа $H$}{geometric object of type H, representation g}

Определение
\ref{definition: geometric object, coordinate representation, tower of representations g}
строит геометрический объект в координатном пространстве.
Определение \ref{definition: geometric object, tower of representations g} предполагает,
что мы выбрали базис башни представлений $\Vector g$.
Это позволяет использовать представитель геометрического объекта
вместо его координат.

\begin{theorem}[\AddIndex{принцип инвариантности}{invariance principle, tower of representations g}]
\label{theorem: invariance principle, tower of representations g}
Представитель геометрического объекта не зависит от выбора
базиса $\Vector Y'_{\Vector g\cdot[1]}$.
\end{theorem}
\begin{proof}
Чтобы определить представителя геометрического объекта,
мы должны выбрать базис $\Vector Y_{\Vector f\cdot[1]}$,
базис
$\Vector Y_{\Vector g\cdot[1]}$
и координаты геометрического объекта
\ShowEq{invariance principle 4, tower of representations}
Соответствующий представитель геометрического
объекта имеет вид
\ShowEq{invariance principle 1, tower of representations}
Базис
\ShowEq{basis Y prim f, tower of representations}
связан с базисом
\ShowEq{basis Y f, tower of representations}
пассивным преобразованием
\ShowEq{invariance principle 2, tower of representations}
Согласно построению это порождает пассивное преобразование
\EqRef{passive transformation of tower of representations g}
и координатное преобразование
\EqRef{coordinate transformation, tower of representations g}. Соответствующий
представитель геометрического объекта имеет вид
\ShowEq{invariance principle 3, tower of representations}
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
\end{proof}
\fi

\ePrints{0906.0135}
\ifx\Semafor\ValueOff
\section{Примеры базиса башни представлений}

\subsection{Аффинное пространство}
\label{subsection: Affine Space, basis}
Рассмотрим аффинное пространство $\overset{\circ}{A}$ (раздел
\ref{subsection: Affine space is single transitive representation}).

Абелевая группа $\Vector A$ действует однотранзитивно на множестве $\overset{\circ}{A}$.
Из построений в подразделе
\ref{subsection: representation of group on the set, basis}
следует, что базис множества $\overset{\circ}{A}$ относительно представления
абелевой группы $\Vector A$ состоит из одной точки. Эту точку обычно обозначают
буквой $O$ и называют
\AddIndex{началом системы координат аффинного пространства}
{origin of coordinate system of affine space}.
Следовательно, произвольную точку $A\in\overset{\circ}{A}$
можно представить с помощью вектора
\ShowEq{affine space coordinates, 1}

Пусть $\Basis e$ - базис векторного пространства $\Vector A$.
Тогда вектор $\overset{\longrightarrow}{OA}$ имеет вид
\ShowEq{affine space coordinates, 2}

Множество
\ShowEq{affine space coordinates, 3}
называется
\AddIndex{координатами точки $A$ аффинного пространства $\overset{\circ}{A}$
относительно базиса $(O,\Basis e)$}
{coordinates in affine space}.

\subsection{Координаты вектора в \texorpdfstring{$R$}{R}\Hyph модуле}
\label{subsection: coordinates of vector in module}

Пусть левый модуль $\Vector M$
над кольцом $R$ (\citeBib{Serge Lang}, с. 93)
имеет конечный базис
\ShowEq{left module, basis 1}
Согласно определению
\ref{definition: basis of representation}
любой вектор $\Vector v\in\Vector M$ можно представить в виде
\ShowEq{left module, basis 2}
Согласно теореме
\ref{theorem: X is basis of representation}
$\Vector e_i\in\Basis e$ не может быть представлен подобным образом
через остальные векторы базиса.
Однако это не означает, что мы не можем записать равенство
\ShowEq{left module, basis 3}
где не все $c^i$ равны $0$.
Для того, чтобы равенство
\EqRef{left module, basis 3}
было возможным,
необходимо потребовать, чтобы числа $c^1$, ..., $c^n$ были необратимы
в кольце $R$.
Из равенств
\EqRef{left module, basis 2},
\EqRef{left module, basis 3}
следует, что
вектор $\Vector v$ кроме разложения
\EqRef{left module, basis 2}
относительно базиса $\Basis e$,
имеет также разложение
\ShowEq{left module, basis 4}
Нетрудно заметить, что множество кортежей
\ShowEq{left module, basis 5}
порождает левый $R$\hyph модуль.
Следовательно, множество координат в $R$\Hyph модуле $\Vector M$
является аффинным пространством, а координаты
вектора $\Vector v$ являются аффинной плоскостью в этом пространстве.

Не исключено, что множество координат произвольного представления
универсальной алгебры также можно рассматривать как некоторую башню
представлений.

\subsection{Базис \texorpdfstring{$R$}{R}\Hyph алгебры}
\label{subsection: Basis of R algebra}

Обычно, когда мы рассматриваем $R$\Hyph алгебру $A$, мы
выбираем базис $\Basis e$ соответствующего $R$\Hyph модуля $A$.
Этот выбор удобен, так как
если $R$ - коммутативная алгебра с делением, то разложение вектора однозначно
относительно базиса $R$\Hyph векторного пространства.
Это, в частности, позволяет описать операции произведения, указав структурные константы
алгебры относительно заданого базиса.

В общем случае, базис $R$\Hyph модуля $A$ может оказаться множеством образующих.
Например, если в векторном пространстве $H$, в котором задана алгебра
кватернионов над полем действительных чисел, рассмотреть базис
\ShowEq{quaternion basis over R}
то в алгебре $H$ верно равенство
\ShowEq{quaternion basis over R 1}
Следовательно, множество
\ShowEq{quaternion basis over R 2}
является базисом алгебры $H$.
Следствием равенства
\EqRef{quaternion basis over R 1}
является неоднозначность представления кватерниона относительно
заданного базиса.
А именно, кватернион $a\in H$ можно записать в виде
\ShowEq{quaternion basis over R 3}
где $a^{\gi 4}$ - произвольно.

\subsection{Модуль над алгеброй}
Пусть $A_3$ - свободный модуль над $A_1$\Hyph алгеброй $A_2$ (раздел
\ref{subsection: Module over Algebra}).
Пусть $\Basis e_{32}$ - базис алгебры $A_3$ над алгеброй $A_2$.
Вектор $a_3\in A_3$ имеет представление
\ShowEq{vector space over algebra, 1}
Пусть $\Basis e_{21}$ - базис алгебры $A_2$ над полем $A_1$.
Так как $a_3^j\in A_2$, то мы можем записать их координаты
относительно базиса $\Basis e_{21}$
\ShowEq{vector space over algebra, 2}
Из равенств
\EqRef{vector space over algebra, 1},
\EqRef{vector space over algebra, 2}
следует
\ShowEq{vector space over algebra, 3}
Равенство
\EqRef{vector space over algebra, 3}
показывает структуру координат в векторном пространстве $A_3$
над полем $A_1$.
Нетрудно убедиться, что векторы
\ShowEq{vector space over algebra, 3set}
линейно независимы над полем $A_1$.
Следовательно, мы построили базис $\Basis e_{31}$
векторного пространстве $A_3$
над полем $A_1$.
Следовательно, мы можем переписать равенство
\EqRef{vector space over algebra, 3}
в виде
\ShowEq{vector space over algebra, 4}
Нетрудно убедиться, что вектор $\Vector e_{31\cdot ij}$
можно отожлествить с тензорным произведением
$\Vector e_{21\cdot i}\otimes\Vector e_{32\cdot j}$.
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\section{Представление в категории}
\label{section: Representations in Category}

\ifx\texFuture\Defined
Когда мы рассматриваем представление $\Omega$\Hyph алгебры $A$
в множестве $M$,
вопрос о произведении преобразований множества $M$ остаётся открытым
до тех пор пока мы не рассматриваем произведение групп.
Однако и здесь возникает проблема при определении контравариантного
представления.
Эта задача имеет естественное решение, если вместо множества преобразований
мы рассматриваем множество морфизмов некоторой категории.
\fi

\begin{definition}
Пусть для любых объектов $B$ и $C$ категории $\mathcal B$
на множестве морфизмов $Mor(B,C)$
определена структура $\Omega$\Hyph алгебры.
Множество гомоморфизмов $\Omega$\Hyph алгебры
\[
f_{B,C}:A\rightarrow Mor(B,C)
\]
называется
\AddIndex{представлением $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}
{representation of Omega algebra in category}.
\qed
\end{definition}

Если предположить, что множество $Mor(B,C)$ определенно
только, когда $B=C$, то мы получим определение представления.
Различие в определениях состоит в том, что мы не ограничиваем
себя преобразованиями множества $B$, а рассматриваем $\Omega$\Hyph алгебру
отображений из множества $B$ в множество $C$.
На первый взгляд нет принципиальных различий между рассматриваемыми
теориями. Однако нетрудно заметить, что представление векторного
пространства в категории расслоений приводит к теории связностей.

%Интересную точку зрения представляет случай, когда $\Omega$\Hyph алгебра
%является множеством морфизмов категории $\mathcal A$.
\fi


==> Tower.Representation.Russian.tex <==
%auto-ignore
\input{Tower.Representation.Eq}
\chapter{Башня представлений
универсальных алгебр}
\label{chapter: Tower of Representations of Algebras}

\section{Башня представлений
универсальных алгебр}
\label{section: Tower of Representations of Algebras}

\begin{definition}
\label{definition: tower of representations}
\ePrints{0906.0135}
\ifx\Semafor\ValueOn
Рассмотрим\footnote{Определения и теоремы из этой главы
включены также в главы
\xRef{8443-0072}{chapter: Tower of Representations of Algebras},
\xRef{8443-0072}{chapter: Basis of Tower of Representations of Universal Algebra}.
}
\else
Рассмотрим
\fi
множество $\Omega_k$\Hyph алгебр $A_k$, \Kn1.
Положим $\Vector A=(A_1,...,A_n)$.
Положим $\Vector f=(f_{1,2},...,f_{n-1,n})$.
Множество представлений $f_{k,k+1}$,
\Kn1, 
$\Omega_k$\Hyph алгебры $A_k$ в
$\Omega_{k+1}$\Hyph алгебре $A_{k+1}$
называется
\AddIndex{башней $(\Vector A,\Vector f)$ представлений
$\Vector{\Omega}$\Hyph алгебр}
{tower of representations of algebras}.
\qed
\end{definition}

Мы можем проиллюстрировать определение \ref{definition: tower of representations}
с помощью диаграммы
\ShowEq{Tower of Representations}
$f_{i,i+1}$ - представление $\Omega_i$\Hyph алгебры $A_i$
в $\Omega_{i+1}$\Hyph алгебре $A_{i+1}$.
$f_{i+1,i+2}$ - представление $\Omega_{i+1}$\Hyph алгебры $A_{i+1}$
в $\Omega_{i+2}$\Hyph алгебре $A_{i+2}$.

\begin{theorem}
\label{theorem: define map f13}
Отображение
\[
f_{i,i+2}:A_i\rightarrow {}^{**}A_{i+2}
\]
является представлением $\Omega_i$\Hyph алгебры $A_i$
в $\Omega_{i+1}$\Hyph алгебре ${}^*A_{i+2}$.
\end{theorem}
\begin{proof}
Произвольному $a_{i+1}\in A_{i+1}$ соответствует автоморфизм $f_{i+1,i+2}(a_{i+1})\in {}^*A_{i+2}$.
Произвольному $a_i\in A_i$ соответствует автоморфизм $f_{i,i+1}(a_i)\in {}^*A_{i+1}$.
Так как образом элемента $a_{i+1}\in A_{i+1}$ является элемент
$f_{i,i+1}(a_i)(a_{i+1})\in A_{i+1}$, то тем самым элемент $a_i\in A_i$
порождает преобразование $\Omega_{i+1}$\Hyph алгебры ${}^*A_{i+2}$,
определённое равенством
\ShowEq{define map f13}

Пусть $\omega$ - $n$\Hyph арная операция $\Omega_i$\Hyph алгебры.
Так как $f_{i,i+1}$ - гомоморфизм $\Omega_i$\Hyph алгебры, то
\ShowEq{f12 morphism f1 algebra}
Для $a_1$, ..., $a_n\in A_i$ мы определим операцию $\omega$ на множестве ${}^{**}A_{i+2}$
с помощью равенства
\ShowEq{omega f1 on level 3}
Первое равенство следует из равенства \EqRef{define map f13}.
Второе равенство постулировано на основе требования, что отображение $f_{i+1,i+2}$
является гомоморфизмом $\Omega_i$\Hyph алгебры.
Следовательно, мы определили
структуру $\Omega_i$\Hyph алгебры на множестве ${}^{**}A_{i+2}$.

Из \EqRef{omega f1 on level 3} и \EqRef{f12 morphism f1 algebra} следует
\ShowEq{omega f1 on level 3, 2}
Из равенства \EqRef{omega f1 on level 3, 2} следует
\ShowEq{omega f1 on level 3, 3}
Следовательно, отображение $f_{i,i+2}$ является гомоморфизмом $\Omega_i$\Hyph алгебры.
Следовательно, отображение $f_{i,i+2}$ является представлением
$\Omega_i$\Hyph алгебры $A_i$
в $\Omega_{i+1}$\Hyph алгебре ${}^*A_{i+2}$.
\end{proof}

\begin{theorem}
\label{theorem: morphism representations f23}
$(id,f_{i+1,i+2})$ является морфизмом представлений
$\Omega_i$\Hyph алгебры
из $f_{i,i+1}$ в $f_{i,i+2}$.
\end{theorem}
\begin{proof}
Рассмотрим более детально диаграмму \EqRef{Tower of Representations}.
\ShowEq{morphism representations f23}
Утверждение теоремы следует
из равенства \EqRef{define map f13} и
определения \ref{definition: morphism of representations of F algebra}.
\end{proof}

\begin{theorem}
\label{theorem: expand f i i+2 over A i+2}
Рассмотрим башню $(\Vector A,\Vector f)$ представлений
$\Vector{\Omega}$\Hyph алгебр.
Если тождественное преобразование
\ShowEq{identity map A i+2}
$\Omega_{i+2}$\hyph алгебры $A_{i+2}$ принадлежит представлению $f_{i+1,i+2}$,
то представление $f_{i,i+2}$ $\Omega_i$\hyph алгебры $A_i$
в $\Omega_{i+1}$\hyph алгебре ${}^*A_{i+2}$ может быть продолжено до представления
\ShowEq{extend representation i i+2}
$\Omega_i$\hyph алгебры $A_i$
в $\Omega_{i+2}$\hyph алгебре $A_{i+2}$.
\end{theorem}
\begin{proof}
Согласно равенству
\EqRef{define map f13},
для заданного $a_{i+1}\in A_{i+1}$ мы можем определить отображение
\ShowEq{define map f13, v}
Пусть существует $a_{i+1}\in A_{i+1}$ такой, что
\ShowEq{identity map A i+2, 1}
Тогда из \EqRef{define map f13, v},\EqRef{identity map A i+2, 1}
следует
\ShowEq{identity map A i+2, 2}
Пусть $\omega$ - $n$\hyph арная операция $\Omega_i$\hyph алгебры $A_i$.
Поскольку $f_{i,i+2}$ - гомоморфизм $\Omega_i$\hyph алгебры, то из равенства
\EqRef{define map f13} следует
\ShowEq{identity map A i+2, 4}
Из равенства \EqRef{identity map A i+2, 4} следует
\ShowEq{identity map A i+2, 5}
Из равенств
\EqRef{identity map A i+2, 1}, \EqRef{identity map A i+2, 2},
\EqRef{identity map A i+2, 5} следует
\ShowEq{identity map A i+2, 6}
Равенство \EqRef{identity map A i+2, 6} определяет операцию $\omega$
на множестве ${}^*A_{i+2}$
\ShowEq{identity map A i+2, 7}
При этом отображение $f'_{i,i+2}$
является гомоморфизмом $\Omega_i$\hyph алгебры. Следовательно, мы построили
представление $\Omega_i$\hyph алгебры $A_i$ в $\Omega_{i+2}$\hyph алгебре $A_{i+2}$.
\end{proof}

\begin{definition}
Рассмотрим башню представлений
\ShowEq{tower of representations, 1 2 3}
Отображение
\ShowEq{representation of algebra in representation}
называется \AddIndex{представлением $\Omega_1$\Hyph
алгебры $A_1$ в представлении $f_{2,3}$}
{representation of Omega algebra in representation}.
\qed
\end{definition}

\begin{definition}
Рассмотрим башню представлений $(\Vector A,\Vector f)$.
Отображение
\ShowEq{representation of algebra in tower of representations}
называется \AddIndex{представлением $\Omega_1$\Hyph
алгебры $A_1$ в башне представлений}
{representation of Omega algebra in tower of representations}
\ShowEq{tower of representations, 2 ... n}
\qed
\end{definition}

\ifx\texFuture\Defined
\section{Башня \texorpdfstring{$T*$\Hyph }{Ts-}представлений
групп}
\label{section: Tower of Representations of Groups}

Башня представлений $(\Vector G,\Vector f)$
называется башней представлений групп, если все рассматриваемые
$\Omega_i$\Hyph алгебры являются группами.
Так как мы рассматриваем одновременно несколько групп,
нам необходимо отличать групповую операцию на разных уровнях.
Когда групповых структур немного, мы можем воспользоваться символами
$.$, $*$, $+$. В общем случае мы будем обозначать групповую
операцию на уровне $i$ символом $*_i$.

Произведение в группе согласованно с произведением
преобразований представления. Это позволяет определить
категорию, объектами которой являются элементы множеств и морфизмами
которой являются преобразования преобразования представления. 

\begin{definition}
Пусть $(\Vector G,\Vector f)$ - башня представлений групп.
Единственным объектом категории $\mathcal G$
является последовательность $(G_i)$, $i>1$.
Морфизмами является последовательность
преобразований $(f_{i-1,i}(c_{i-1}))$.
\qed
\end{definition}

Согласно теореме
\ref{theorem: define map f13}
определён $2$\Hyph морфизм $(f_{i-2,i}(d_{i-2}))$, отображающий
морфизм $(f_{i-1,i}(c_{i-1}))$ в морфизм
$(f_{i-1,i}(f_{i-2,i}(d_{i-2})(c_{i-1})))$.
Таким образом, категория $\mathcal G$ является $2$\Hyph категорией
(\citeBib{9705.009}).

Согласно \citeBib{9705.009} определено два вида произведений
$2$\Hyph морфизмов.

Вертикальное произведение $2$\Hyph морфизмов определенно согласно
следующей диаграмме
\[
\xymatrix{
\\
A_{i+2}
\ar@/^4pc/[rrrrrr]^{f_{i+1,i+2}(a_{i+1})}^(.6){\ }="f1"
\ar[rrrrrr]^(.4){f_{i+1,i+2}(b_{i+1})}^(.1){\ }="f2"
\ar@/_4pc/[rrrrrr]_{f_{i+1,i+2}(c_{i+1})}_(.6){\ }="f3"
&&&&&&A_{i+2}
\\
&
\ar @{=>}^{f_{i,i+2}(a_i)} "f1";"f2"
\ar @{=>}^{f_{i,i+2}(b_i)} "f2";"f3"
\ar @{=>}^(.3){f_{i,i+2}(c_i)} "f1";"f3"
}
\]

Горизонтальное произведение $2$\Hyph морфизмов определенно согласно
следующей диаграмме
\[
\xymatrix{
\\
A_i
\ar@/^2pc/[rrrrr]^(.6){f_{i-1,i}(a_{i-1})}^(.3){\ }="f1"
\ar@/_2pc/[rrrrr]_(.6){f_{i-1,i}(b_{i-1})}_(.3){\ }="f2"
\ar@/^4pc/[rrrrrrrrrr]^{f_{i-1,i}(e_{i-1})}^{\ }="f1a"
\ar@/_4pc/[rrrrrrrrrr]_{f_{i-1,i}(g_{i-1})}_{\ }="f2a"
&&&&&A_i
\ar@/^2pc/[rrrrr]^(.4){f_{i-1,i}(c_{i-1})}^{\ }="f3"
\ar@/_2pc/[rrrrr]_(.4){f_{i-1,i}(d_{i-1})}_{\ }="f4"
&&&&&A_i
\\
&
\ar @{=>}^{f_{i-2,i}(a_{i-2})} "f1";"f2"
\ar @{=>}^{f_{i-2,i}(b_{i-2})} "f3";"f4"
\ar @/^2pc/@{=>}^{f_{i-2,i}(c_{i-2})} "f1a";"f2a"
}
\]
\begin{align}
b_{i-1}&=f_{i-2,i-1}(a_{i-2})(a_{i-1})
\label{horizontal product 2-morphism, b i-1 a i-2}
\\
d_{i-1}&=f_{i-2,i-1}(b_{i-2})(c_{i-1})
\label{horizontal product 2-morphism, d i-1 b i-2}
\\
g_{i-1}&=f_{i-2,i-1}(c_{i-2})(e_{i-1})
\label{horizontal product 2-morphism, d i-1}
\\
e_{i-1}&=c_{i-1}a_{i-1}
\label{horizontal product 2-morphism, e i-1}
\\
g_{i-1}&=d_{i-1}b_{i-1}
\label{horizontal product 2-morphism, g i-1}
\end{align}
Из равенств
\eqref{horizontal product 2-morphism, g i-1},
\eqref{horizontal product 2-morphism, b i-1 a i-2},
\eqref{horizontal product 2-morphism, d i-1 b i-2}
следует
\[
g_{i-1}=f_{i-2,i-1}(b_{i-2})(c_{i-1})f_{i-2,i-1}(a_{i-2})(a_{i-1})
\]
\fi

\section{Морфизм башни \texorpdfstring{$T*$\Hyph }{Ts-}представлений}
\label{section: Morphism of Tower of Representations}

\begin{definition}
Рассмотрим множество $\Omega_k$\Hyph алгебр $A_k$, $B_k$, \Kn1.
Множество отображений
$(h_1,...,h_n)$ называется \AddIndex{морфизмом из башни представлений
$(\Vector A,\Vector f)$ в башню представлений $(\Vector B,\Vector g)$}
{morphism from tower of representations into tower of representations},
если для каждого $k$, $k=1$, ..., $n-1$,
пара отображений $(h_k,h_{k+1})$ является
морфизмом представлений из $f_{k,k+1}$ в $g_{k,k+1}$.
\qed
\end{definition}

Для любого $k$, $k=1$, ..., $n-1$, мы имеем диаграмму
\ShowEq{morphism of tower of representations of F algebra, level k, diagram}
Равенства
\ShowEq{morphism of tower of representations}
выражают коммутативность диаграммы (1).
Однако уже для морфизма $(h_k,h_{k+1})$, $k>1$, диаграмма
\EqRef{morphism of tower of representations of F algebra, level k, diagram}
неполна.
Учитывая аналогичную диаграмму для морфизма $(h_k,h_{k+1})$ эта
диаграмма на верхнем уровне приобретает вид
\ShowEq{morphism h3}
К сожалению, диаграмма \EqRef{morphism h3} малоинформативна. Очевидно,
что существует морфизм из ${}^*A_{k+2}$ в ${}^*B_{k+2}$,
отображающий $f_{k,k+2}(a_k)$ в $g_{k,k+2}(h_k(a_k))$.
Однако структура этого морфизма из диаграммы неясна.
Мы должны рассмотреть отображение из ${}^*A_{k+2}$ в ${}^*B_{k+2}$,
так же мы это сделали в теореме
\ref{theorem: morphism representations f23}.

\begin{theorem}
\label{theorem: morphism representations h3 h1}
Если представления $f_{i+1,i+2}$ эффективно, то
$(h_i,{}^*h_{i+2})$ является морфизмом представлений
из представления $f_{i,i+2}$ в представление $g_{i,i+2}$
$\Omega_i$\Hyph алгебры.
\end{theorem}
\begin{proof}
Рассмотрим диаграмму
\ShowEq{morphism representations h3 h1}
Существование отображения ${}^*h_{i+2}$ и
коммутативность диаграмм $(2)$ и $(3)$ следует
из эффективности отображения $f_{i+1,i+2}$ и
теоремы \ref{theorem: morphism of representations and homomorphism of algebra}.
Коммутативность диаграмм $(4)$ и $(5)$ следует
из теоремы \ref{theorem: morphism representations f23}.

Из коммутативности диаграммы $(4)$ следует
\begin{equation}
f_{i+1,i+2}\circ f_{i,i+1}(a_i)=f_{i,i+2}(a_i)\circ f_{i+1,i+2}
\EqLabel{Morphism of Tower of Representations, diagram 4}
\end{equation}
Из равенства \EqRef{Morphism of Tower of Representations, diagram 4} следует
\begin{equation}
{}^*h_{i+2}\circ f_{i+1,i+2}\circ f_{i,i+1}(a_i)={}^*h_{i+2}\circ f_{i,i+2}(a_i)\circ f_{i+1,i+2}
\EqLabel{Morphism of Tower of Representations, diagram 4a}
\end{equation}
Из коммутативности диаграммы $(3)$ следует
\begin{equation}
{}^*h_{i+2}\circ f_{i+1,i+2}=g_{i+1,i+2}\circ h_{i+1}
\EqLabel{Morphism of Tower of Representations, diagram 3}
\end{equation}
Из равенства \EqRef{Morphism of Tower of Representations, diagram 3} следует
\begin{equation}
{}^*h_{i+2}\circ f_{i+1,i+2}\circ f_{i,i+1}(a_i)=g_{i+1,i+2}\circ h_{i+1}\circ f_{i,i+1}(a_i)
\EqLabel{Morphism of Tower of Representations, diagram 3a}
\end{equation}
Из равенств \EqRef{Morphism of Tower of Representations, diagram 4a}
и \EqRef{Morphism of Tower of Representations, diagram 3a} следует
\begin{equation}
{}^*h_{i+2}\circ f_{i,i+2}(a_i)\circ f_{i+1,i+2}=g_{i+1,i+2}\circ h_{i+1}\circ f_{i,i+1}(a_i)
\EqLabel{Morphism of Tower of Representations, diagrams 4, 3}
\end{equation}

Из коммутативности диаграммы $(5)$ следует
\ShowEq{Morphism of Tower of Representations, diagram 5}
Из равенства \EqRef{Morphism of Tower of Representations, diagram 5} следует
\ShowEq{Morphism of Tower of Representations, diagram 5a}
Из коммутативности диаграммы $(2)$ следует
\ShowEq{Morphism of Tower of Representations, diagram 2}
Из равенства \EqRef{Morphism of Tower of Representations, diagram 2} следует
\ShowEq{Morphism of Tower of Representations, diagram 2a}
Из равенств \EqRef{Morphism of Tower of Representations, diagram 5a}
и \EqRef{Morphism of Tower of Representations, diagram 2a} следует
\ShowEq{Morphism of Tower of Representations, diagrams 5, 2}

Внешняя диаграмма является диаграммой
\EqRef{morphism of tower of representations of F algebra, level k, diagram}
при $i=1$. Следовательно, внешняя диаграмма коммутативна
\ShowEq{morphism of tower of representations of F algebra, level 1}
Из равенства \EqRef{morphism of tower of representations of F algebra, level 1} следует
\ShowEq{morphism of tower of representations of F algebra, level 1, a}
Из равенств \EqRef{Morphism of Tower of Representations, diagrams 4, 3},
\EqRef{Morphism of Tower of Representations, diagrams 5, 2}
и \EqRef{morphism of tower of representations of F algebra, level 1, a} следует
\ShowEq{morphism of tower of representations of F algebra, level 2}
Так как отображение $f_{i+1,i+2}$ - инъекция, то из равенства
\EqRef{morphism of tower of representations of F algebra, level 2} следует
\ShowEq{morphism of tower of representations of F algebra, level 2, a}
Из равенства \EqRef{morphism of tower of representations of F algebra, level 2, a}
следует коммутативность диаграммы $(1)$, откуда следует утверждение теоремы.
\end{proof}

Теоремы \ref{theorem: morphism representations f23}
и \ref{theorem: morphism representations h3 h1}
справедливы для любых уровней башни представлений.
В каждом конкретном случае надо правильно указывать множества,
откуда и куда направленно отображение.
Смысл приведенных теорем состоит в том,
что все отображения в башне представлений действуют согласовано.

Теорема \ref{theorem: morphism representations h3 h1} утверждает,
что неизвестное отображение на диаграмме \EqRef{morphism h3}
является отображением ${}^*h_{i+2}$.
\ifx\texFuture\Defined
Чтобы получить дополнительную информацию о морфизме башни представлений,
изменим точку зрения на построенные диаграммы.

Согласно определению
\ref{definition: category of representations of F algebra from category}
мы можем определить категорию
башни представлений $\Omega$\Hyph алгебр.
Объектами этой категории являются башни представлений $\Omega$\Hyph алгебр.
Морфизмами этой категории являются морфизмы башни представлений
$\Omega$\Hyph алгебр.
Однако мы можем расширить рамки этого определения.
%Если мы на диаграмме \EqRef{morphism h3} перейдём от множества $A_{i+2}$
%к представлению $f_{i+1,i+2}$, то мы обратим внимание, что в нижней и верхней частях
%диаграммы представлены разные преобразования представления $f_{i+1,i+2}$, связанные
%друг с другом преобразованием представления $f_(i,i+2}$.

Пусть $(\Vector A,\Vector f)$ и $(\Vector B,\Vector g)$ -
башни представлений. Пусть
\begin{align*}
\Vector p:&(\Vector A,\Vector f)\rightarrow(\Vector B,\Vector g)
\\
\Vector r:&(\Vector A,\Vector f)\rightarrow(\Vector B,\Vector g)
\end{align*}
морфизмы башен представлений.
Вообще говоря, не существует непосредственной связи отображений
$p_i$, $p_{i+1}$ и отображений $r_i$, $r_{i+1}$. Однако картина меняется,
когда мы рассматриваем отображения $p_{i+2}$ и $r_{i+2}$.
Согласно
теореме \ref{theorem: morphism of representations and homomorphism of algebra}
отображения ${}^*p_{i+2}$ и ${}^*r_{i+2}$ являются гомоморфизмами $\Omega_{i+2}$\Hyph алгебры.
\fi

\begin{theorem}
\label{theorem: product of morphisms of tower of representations}
Рассмотрим множество $\Omega_i$\Hyph алгебр
$A_i$, $B_i$, $C_i$, $i=1$, ..., $n$.
Пусть определены
морфизмы башни представлений
\ShowEq{product of morphisms of tower of representations, 1}
Тогда определён морфизм представлений $\Omega$\Hyph алгебры
\ShowEq{product of morphisms of tower of representations, 2}
где
\ShowEq{product of morphisms of tower of representations, 3}
Мы будем называть морфизм $\Vector r$ башни представлений
из $\Vector f$ в $\Vector h$
\AddIndex{произведением морфизмов $\Vector p$ и $\Vector q$
башни представлений}
{product of morphisms of tower of representations}.
\end{theorem}
\begin{proof}
Для каждого $k$, $k=2$, ..., $n$,
мы можем представить утверждение теоремы,
пользуясь диаграммой
\ShowEq{product of morphisms of tower of representations, diagram}
Отображение $r_{k-1}$ является гомоморфизмом
$\Omega_{k-1}$\Hyph алгебры $A_{k-1}$ в
$\Omega_{k-1}$\Hyph алгебру $C_{k-1}$.
Нам надо показать, что пара отображений $(r_{k-1},r_k)$ удовлетворяет
\EqRef{morphism of tower of representations, level k}:
\ShowEq{product of morphisms of tower of representations, k-1 k}
\end{proof}

\section{Автоморфизм башни представлений}

\begin{definition}
\label{definition: endomorphism of tower of representations}
Пусть
$(\Vector A,\Vector f)$
- башня представлений $\Vector\Omega$\Hyph алгебр.
Морфизм башни представлений
\ShowEq{endomorphism of tower of representations}
такой, что для любого
\ShowEq{endomorphism of tower of representations, 1}
- эндоморфизм $\Omega_k$\Hyph алгебры $A_k$,
называется
\AddIndex{эндоморфизмом башни представлений}
{endomorphism of tower of representations} $\Vector f$.
\qed
\end{definition}

\begin{definition}
\label{definition: automorphism of tower of representations}
Пусть
$(\Vector A,\Vector f)$
- башня представлений $\Vector\Omega$\Hyph алгебр.
Морфизм башни представлений
\ShowEq{endomorphism of tower of representations}
такой, что для любого
\ShowEq{endomorphism of tower of representations, 1}
- автоморфизм $\Omega_k$\Hyph алгебры $A_k$,
называется
\AddIndex{автоморфизмом башни представлений}
{automorphism of tower of representations} $f$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: group of automorphisms of tower of representations}
Пусть
$(\Vector A,\Vector f)$
- башня представлений $\Vector\Omega$\Hyph алгебр.
Множество автоморфизмов представления $\Vector f$
порождает группу.
\end{theorem}
\begin{proof}
Пусть $\VX r$, $\VX p$ - автоморфизмы башни
представлений $\Vector f$.
Согласно определению
\ref{definition: automorphism of tower of representations}
для любого $k$, \Kn2,
отображения $r_k$, $p_k$ являются автоморфизмами
$\Omega_k$\Hyph алгебры $A_k$.
Согласно теореме II.3.2
(\citeBib{Cohn: Universal Algebra}, c. 60)
для любого $k$, \Kn2,
отображение $r_kp_k$ является автоморфизмом
$\Omega_k$\Hyph алгебры $A_k$.
Из теоремы
\ref{theorem: product of morphisms of tower of representations}
и определения
\ref{definition: automorphism of tower of representations}
следует, что произведение автоморфизмов
$\VX r\VX p$ башни представлений $\Vector f$
является автоморфизмом башни представлений $\Vector f$.

Согласно доказательству теоремы
\ref{theorem: group of automorphisms of representation},
для любого $k$, \Kn2,
произведение автоморфизмов $\Omega_i$\Hyph алгебры ассоциативно.
Следовательно, ассоциативно произведение
автоморфизмов башни представлений.

Пусть $\VX r$ - автоморфизм башни представлений $\Vector f$.
Согласно определению
\ref{definition: automorphism of tower of representations}
для любого $k$, \Kn2,
отображение $r_k$ является автоморфизмом
$\Omega_k$\Hyph алгебры $A_k$.
Следовательно,
для любого $k$, \Kn2,
отображение $r_k^{-1}$ является автоморфизмом
$\Omega_k$\Hyph алгебры $A_k$.
Для автоморфизма $\VX r$ справедливо равенство
\EqRef{morphism of tower of representations, levels k k+1}.
Положим
\ShowEq{morphism of tower of representations, level k, 1}
Так как
\ShowEq{morphism of tower of representations, level k, 2}
- автоморфизм,
то
\ShowEq{morphism of tower of representations, level k, 3}
и равенство
\EqRef{morphism of tower of representations, levels k k+1}
можно записать в виде
\ShowEq{morphism of tower of representations, levels k k+1, 1}
Так как отображение $h_{k+1}$
является автоморфизмом
$\Omega_{k+1}$\Hyph алгебры $A_{k+1}$,
то из равенства
\EqRef{morphism of tower of representations, levels k k+1, 1}
следует
\ShowEq{morphism of tower of representations, levels k k+1, 2}
Равенство
\EqRef{morphism of tower of representations, levels k k+1, 2}
соответствует равенству
\EqRef{morphism of tower of representations, levels k k+1}
для отображения $\VX r^{-1}$.
Следовательно, отображение $\VX r^{-1}$ является автоморфизмом
представления $\Vector f$.
\end{proof}

\ePrints{0906.0135}
\ifx\Semafor\ValueOff
\section{Примеры башни представлений}

\subsection{Аффинное пространство}
\label{subsection: Affine space is single transitive representation}
Пусть $\overset{\circ}{A}$ - множество точек.
Пусть $\Vector A$ - векторное пространство над полем $k$.
Однотранзитивное представление векторного пространства $\Vector A$
в множестве точек $\overset{\circ}{A}$
называется аффинным пространством.
Если $A\in\overset{\circ}{A}$ и $\Vector v\in\Vector A$,
то мы будем обозначать действие вектора $\Vector v$
на точку $A$ выражением $A+\Vector v$.

Однотранзитивность представления означает, что для любых точек
$A$, $B\in\overset{\circ}{A}$ существует единственный вектор
$\Vector v\in\Vector A$ такой, что
\ShowEq{action of vector at the point}
Если вектор $\Vector v$ удовлетворяет равенству
\EqRef{action of vector at the point},
то мы будем также пользоваться обозначением
$\overset{\longrightarrow}{AB}$
для вектора $\Vector v$
\ShowEq{action of vector at the point, 1}

Аффинное пространство является башней представлений, так как
векторное пространство $\Vector A$ является представлением
поля $k$ в абелевой группе $\Vector A$.

\subsection{Свободная алгебра над кольцом}
\label{subsection: Free Algebra over Ring}

Согласно определениям
\citeBib{Richard D. Schafer}, с. 1,
\citeBib{0105.155}, с. 4,
свободная алгебра $A$ над коммутативным кольцом $R$ - это
свободный $R$\Hyph модуль, в котором определено произведение,
являющееся билинейным отображением $R$\Hyph модуля $A$.
Это определение неудовлетворительно, так как эндоморфизмы, порождённые
представлением, не являются эндоморфизмами алгебры.
Однако мы можем изменить определение $R$\Hyph алгебры таким образом,
чтобы все требования к представлению были удовлетворены.

Согласно определению
\ePrints{8433-5163}
\ifx\Semafor\ValueOn
\xRef{8443-0072}{definition: polylinear map of modules},
\else
\xRef{1003.1544}{definition: polylinear map of modules},
\fi
отображение
\ShowEq{endomorphism of module from product}
является линейным отображением. Следовательно, отображение
\EqRef{endomorphism of module from product}
является эндоморфизмом $R$\Hyph модуля $A$.
Мы будем называть эндоморфизм
\EqRef{endomorphism of module from product}
\AddIndex{левым сдвигом $R$\Hyph модуля $A$}{left shift of module}.

\begin{theorem}
\label{theorem: Free Algebra over Ring}
Представление
\ShowEq{endomorphism of module from product, 1}
$R$\Hyph модуля $A$ в $R$\Hyph модуле $A$
эквивалентно структуре $R$\Hyph алгебры $A$.
\end{theorem}
\begin{proof}
Пусть структура $R$\Hyph модуля $A$ порождена эффективным представлением
\ShowEq{endomorphism of module from product, 2}
кольца $R$ в абелевой группе $A$.

Отображение $f_{2,3}(a)$ является левым сдвигом $R$\Hyph модуля $A$.
Поскольку левый сдвиг является эндоморфизмом $R$\Hyph модуля $A$, то
\ShowEq{endomorphism of module from product, 3}
Поскольку отображение
\EqRef{endomorphism of module from product, 1} -
гомоморфизм абелевых групп, то
\ShowEq{endomorphism of module from product, 4}

Согласно теореме
\ref{theorem: define map f13}
существует представление
\ShowEq{endomorphism of module from product, 5}
которое согласно равенству
\EqRef{define map f13}
определено правилом
\ShowEq{endomorphism of module from product, 6}
Мы не предполагаем представление $f_{2,3}$ эффективным.\footnote{Если
представление $f_{2,3}$ не эффективно, то $R$\Hyph алгебра $A$ имеет
делители нуля.}
Поэтому представление $f_{1,3}$ так же может быть не эффективным.
Однако мы можем, также как и в случае отображения $f_{1,2}$,
отождествлять $f_{1,3}(r)$ и $r$.
Из равенства
\EqRef{endomorphism of module from product, 6}
следует
\ShowEq{endomorphism of module from product, 7}
Из равенств
\EqRef{endomorphism of module from product, 3},
\EqRef{endomorphism of module from product, 4},
\EqRef{endomorphism of module from product, 7}
и определения
\ePrints{8443-0072}
\ifx\Semafor\ValueOn
\xRef{8433-5163}{definition: polylinear map of modules},
\else
\xRef{1003.1544}{definition: polylinear map of modules},
\fi
следует, что отображение $f_{2,3}$ является билинейным отображением.
Следовательно, отображение $f_{2,3}$ определяет произведение в
$R$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
\end{proof}

\begin{corollary}
Башня представлений
\ShowEq{tower representation, R algebra}
порождает структуру $R$\Hyph алгебры $A$.
\qed
\end{corollary}

Обратим внимание, что при определении $R$\Hyph алгебры $A$
область определения отображения $f_{2,3}$ - не всё множество
эндоморфизмов абелевой группы $A$, а множество эндоморфизмов
$R$\Hyph модуля $A$. Мы предполагаем, что в определении
\ref{definition: tower of representations}
каждый элемент башни представлений
является башней представлений.
В этом случае,
\AddIndex{диаграмма представлений}{diagram of representations}
для $R$\Hyph алгебры имеет вид
\ShowEq{algebra, diagram representation}
На диаграмме представлений
\EqRef{algebra, diagram representation}
предполагается, что мы сперва строим представление $g_{1,2}$,
порождающее структуру $R$\Hyph модуля $A$.
Представление $f_{1,2}$ порождает структуру $R$\Hyph модуля $A$.
Согласно определению, представление $f_{2,3}$ является гомоморфизмом
$R$\Hyph модуля $A$ в множество эндоморфизмов $R$\Hyph модуля $A$.

\subsection{Групповая алгебра}

Если $R$ - кольцо и $G$ - мультипликативная группа,
то свободный $R$\Hyph модуль $R[G]$ с базисом $G$
называется групповым кольцом (\citeBib{Mihalev Pilz: concise handbook of algebra}, с. 383).
Из теоремы
\xRef{0701.238}{theorem: free module with semigroup basis}
следует, что мы можем продолжить умножение с группы $G$ на модуль $R[G]$.
Следовательно, модуль $R[G]$ является свободной $R$\Hyph алгеброй.

Если $R$ - коммутативное кольцо,
то модуль $R[G]$
называется \AddIndex{групповой алгеброй}{group algebra} группы $G$
(\citeBib{Shafarevich: Basic notions of algebra}, с. 74).
Поскольку группа $G$ является базисом групповой алгебры,
мы можем записать элемент алгебры $R[G]$ в виде
\ShowEq{Group Algebra Expansion}
Произведение прроизвольных элементов $R[G]$ имеет вид
\ShowEq{Group Algebra Expansion, product}
Координаты элемента $a\in R[g]$ можно интерпретировать как отображение
\ShowEq{coordinates in Group Algebra}

\subsection{Модуль над алгеброй}
\label{subsection: Module over Algebra}

Пусть $A_2$ - свободная алгебра над полем $A_1$.
Рассматривая алгебру $A_2$ как кольцо, мы можем определить
свободный модуль $A_3$ над алгеброй $A_2$.
Мы можем описать модуль $A_3$ с помощью диаграммы представлений
\ShowEq{diagram representations, module over algebra}
\fi


==> Tstar.Basis.Russian.tex <==
%auto-ignore
\input{Tstar.Basis.Eq}

\ePrints{0912.3315,0906.0135}
\ifx\Semafor\ValueOff
\chapter{Базис представления универсальной алгебры}
\label{chapter: Basis of Representation of Universal Algebra}
\fi

\section{Множество образующих представления}
\label{section: generating set of representation}

\begin{definition}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Множество $N\subset M$ называется
\AddIndex{стабильным множеством представления}
{stable set of representation} $f$,
если $f(a)(m)\in N$ для любых $a\in A$, $m\in N$.
\qed
\end{definition}

Мы также будем говорить, что множество $M$
стабильно относительно представления $f$.

\begin{theorem}%
\label{theorem: subrepresentation of representation}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Пусть множество $N\subset M$ является
подалгеброй $\Omega_2$\Hyph алгебры $M$
и стабильным множеством представления $f$.
Тогда существует представление
\ShowEq{representation of algebra A in algebra N}
такое, что $f_N(a)=f(a)|_N$.
Представление $f_N$ называется
\AddIndex{подпредставлением представления}
{subrepresentation of representation} $f$.
\end{theorem}
\begin{proof}
Пусть $\omega_1$ - $n$\Hyph арная операция $\Omega_1$\Hyph алгебры $A$.
Тогда для любых
$a_1$, ..., $a_n\in A$
и любого $b\in N$
\ShowEq{representation of algebra A in algebra N, 1}
Пусть $\omega_2$ - $n$\Hyph арная операция $\Omega_2$\Hyph алгебры $M$.
Тогда для любых
$b_1$, ..., $b_n\in N$
и любого $a\in A$
\ShowEq{representation of algebra A in algebra N, 2}
Утверждение теоремы доказано.
\end{proof}

Из теоремы \ref{theorem: subrepresentation of representation}
следует, что если $f_N$ - подпредставление представления $f$,
то отображение $(id:A\rightarrow A,id_N:N\rightarrow M)$
является морфизмом представлений.

\begin{theorem}%
\label{theorem: lattice of subrepresentations}
Множество\footnote{Это определение
аналогично определению структуры подалгебр
(\citeBib{Cohn: Universal Algebra}, стр. 93, 94)}
\ShowEq{lattice of subrepresentations}
всех подпредставлений представления $f$ порождает
систему замыканий на $\Omega_2$\Hyph алгебре $M$
и, следовательно, является полной структурой.
\end{theorem}
\begin{proof}
Пусть $(K_{\lambda})_{\lambda\in\Lambda}$
- семейство подалгебр
$\Omega_2$\Hyph алгебры $M$,
стабильных относительно представления $f$.
Операцию пересечения на множестве $\mathcal B_f$
мы определим согласно правилу
\ShowEq{set of subrepresentations, intersection}
Операция пересечения подпредставлений определена корректно.
$\cap K_{\lambda}$ - подалгебра
$\Omega_2$\Hyph алгебры $M$.
Пусть $m\in \cap K_{\lambda}$.
%Если $K$ и $L$ - стабильные множества представления, то
Для любого $\lambda\in\Lambda$ и для любого $a\in A$,
$f(a)(m)\in K_{\lambda}$.
Следовательно, $f(a)(m)\in\cap K_{\lambda}$.
Следовательно, $\cap K_{\lambda}$ - стабильное множество представления $f$.
\end{proof}

Обозначим соответствующий оператор замыкания через
\ShowEq{closure operator, representation}
Таким образом, $J(f,X)$ является пересечением всех подалгебр
$\Omega_2$\Hyph алгебры $M$,
содержащих $X$ и стабильных относительно представления $f$.

\begin{theorem}%
\label{theorem: structure of subrepresentations}
Пусть\footnote{Утверждение теоремы аналогично
утверждению теоремы 5.1, \citeBib{Cohn: Universal Algebra}, стр. 94.}
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Пусть $X\subset M$.
Определим подмножество $X_k\subset M$ индукцией по $k$.
\ShowEq{structure of subrepresentations}
Тогда
\ShowEq{structure of subrepresentations, 1}
\end{theorem}
\begin{proof}
Если положим $U=\cup X_k$, то по определению $X_k$
имеем $X_0\subset J(f,X)$, и если $X_k\subset J(f,X)$, то
$X_{k+1}\subset J(f,X)$.
По индукции следует, что $X_k\subset J(f,X)$ для всех $k$.
Следовательно,
\ShowEq{structure of subrepresentations, U subset J_f}

Если $a\in U^n$, $a=(a_1,...,a_n)$, где $a_i\in X_{k_i}$, и
если $k=\max \{k_1,...,k_n\}$, то
\ShowEq{structure of subrepresentations, 2}
Следовательно,
$U$ является подалгеброй $\Omega_2$\Hyph алгебры $M$.

Если $m\in U$, то $m\in X_k$ для некоторого $k$. Следовательно,
$f(a)(m)\in X_{k+1}\subset U$ для любого $a\in A$.
Следовательно, $U$ - стабильное множество представления $f$.

Так как $U$ - подалгеброй $\Omega_2$\Hyph алгебры $M$
и стабильное множество представления $f$,
то определено подпредставление $f_U$.
Следовательно,
\ShowEq{structure of subrepresentations, J_f subset U}
Из \EqRef{structure of subrepresentations, U subset J_f},
\EqRef{structure of subrepresentations, J_f subset U},
следует $J(f,X)=U$.
\end{proof}

\begin{definition}
\label{definition: generating set of representation}
$J(f,X)$ называется
\AddIndex{подпредставлением, порождённым множеством $X$}
{subrepresentation generated by set},
а $X$ -
\AddIndex{множеством образующих подпредставления $J(f,X)$}
{generating set of subrepresentation}.
В частности,
\AddIndex{множеством образующих представления $f$}
{generating set of representation}
будет такое подмножество $X\subset M$,
что $J(f,X)=M$.
\qed
\end{definition}

Нетрудно видеть, что определение множества образующих
представления не зависит от того, эффективно представление или нет.
Поэтому в дальнейшем мы будем предполагать, что
представление эффективно и будем опираться на соглашение
для эффективного левостороннего представления в замечании
\ePrints{MRepro}
\ifx\Semafor\ValueOn
\xRef{8443-0072}{remark: notation for effective representation of algebra}.
\else
\ref{remark: notation for effective representation of algebra}.
\fi
Мы также будем пользоваться записью
\ShowEq{endomorphism image, effective representation}
для образа $m\in M$ при эндоморфизме эффективного представления.
Согласно определению произведения отображений,
для любых эндоморфизмов $R$, $S$ верно равенство
\ShowEq{endomorphism image, 1, effective representation}
Равенство
\EqRef{endomorphism image, 1, effective representation}
является законом ассоциативности для $\circ$ и позволяет
записать выражение
\ShowEq{endomorphism image, 2, effective representation}
без использования скобок.

Из теоремы \ref{theorem: structure of subrepresentations}
следует следующее определение.

\begin{definition}
\label{definition: word of element relative to set, representation}
Пусть $X\subset M$.
Для любого $x\in J(f,X)$ существует
$\Omega_2$\Hyph слово, определённое согласно следующему правилам.
\begin{enumerate}
\item Если $m\in X$, то $m$ - $\Omega_2$\Hyph слово.
\label{word of element relative to set, representation, m in X}
\item Если $m_1$, ..., $m_n$ - $\Omega_2$\Hyph слова и
$\omega\in\Omega_2(n)$, то $m_1...m_n\omega$
- $\Omega_2$\Hyph слово.
\label{word of element relative to set, representation, omega}
\item Если $m$ - $\Omega_2$\Hyph слово и
$a\in A$, то $am$
- $\Omega_2$\Hyph слово.
\label{word of element relative to set, representation, am}
\end{enumerate}
\AddIndex{$\Omega_2$\Hyph слово}
{word of element relative to generating set, representation}
\ShowEq{word of element relative to generating set, representation}
представляет данный элемент $m\in J(f,X)$.
Мы будем отождествлять элемент $m\in J(f,X)$
и соответствующее ему $\Omega_2$\Hyph слово, выражая это равенством
\ShowEq{identify element jf(X) and word}
Аналогично, для произвольного множества
\ShowEq{subset of representation}
рассмотрим множество $\Omega_2$\Hyph слов\footnote{Выражение $w(f,X,m)$
является частным случаем
выражения $w(f,X,B)$, а именно
\ShowEq{subset of words of representation, 2}
}
\ShowEq{subset of words of representation}
Мы будем также пользоваться записью
\ShowEq{subset of words of representation, 1}
Обозначим
\ShowEq{word set of representation}
\AddIndex{множество $\Omega_2$\Hyph слов представления $J(f,X)$}
{word set of representation}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: map of words of representation}
Эндоморфизм $R$ представления
\ShowEq{f:A->*M}
порождает отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation}
такое, что
\StartLabelItem
\begin{enumerate}
\item Если
\ShowEq{map of words of representation, m in X, 1}
то
\ShowEq{map of words of representation, m in X}
\item Если
\ShowEq{map of words of representation, omega, 1}
то для операции
$\omega\in\Omega_2(n)$ справедливо
\ShowEq{map of words of representation, omega}
\item Если
\ShowEq{map of words of representation, am, 1}
то
\ShowEq{map of words of representation, am}
\end{enumerate}
\end{theorem}
\begin{proof}
Утверждения
\RefItem{map of words of representation, m in X},
\RefItem{map of words of representation, omega}
справедливы в силу определения эндоморфизма $R$.
Утверждение
\\RefItem{map of words of representation, am}
следует из равенства
\ePrints{1111.6035}
\ifx\Semafor\ValueOn
\xEqRef{8443-0072}{morphism of representations of F algebra, definition, 2m},
\else
\EqRef{morphism of representations of F algebra, definition, 2m},
\fi
так как $r=\id$.
\end{proof}

\begin{remark}
\label{remark: coordinates of representation}
Пусть $R$ - эндоморфизм представления $f$.
Пусть
\ShowEq{map of words of representation 1}
Теорема
\ref{theorem: map of words of representation}
утверждает, что
\ShowEq{map of words of representation 2}.
Теорема
\ref{theorem: map of words of representation}
также утверждает, что
$\Omega_2$\Hyph слово, представляющее $m$, относительно $X$ и
$\Omega_2$\Hyph слово, представляющее $m'$, относительно $X'$
формируются согласно одному и тому же алгоритму.
Это позволяет рассматривать множество $\Omega_2$\Hyph слов $w(f,X',m')$
как отображение
\ShowEq{coordinates of representation 3}
такое, что, если для некоторого эндоморфизма $R$ 
\ShowEq{coordinates of representation 4}
то
\ShowEq{coordinates of representation 5}
Отображение
$\ShowSymbol{coordinates of element relative to generating set, representation}{}$
называется
\AddIndex{координатами элемента $m$ относительно множества $X$}
{coordinates of element relative to set, representation}.
Аналогично, мы можем рассмотреть координаты множества
\ShowEq{subset of representation}
относительно множества $X$
\ShowEq{subset of coordinates of representation}
Обозначим
\ShowEq{coordinate set of representation}
\AddIndex{множество координат представления $J(f,X)$}
{coordinate set of representation}.
\qed
\end{remark}

\begin{theorem}
\label{theorem: set of coordinates, representation, omega}
На множестве координат $W(f,X)$ определена структура $\Omega_2$\Hyph алгебры.
\end{theorem}
\begin{proof}
Пусть $\omega\in\Omega_2(n)$. Тогда для любых
\ShowEq{set of coordinates, 1, omega}
положим
\ShowEq{set of coordinates, omega}
Согласно замечанию
\ref{remark: coordinates of representation},
из равенства
\EqRef{set of coordinates, omega}
следует
\ShowEq{set of coordinates, 2, omega}
Согласно правилу
\eqref{word of element relative to set, representation, omega}
определения
\ref{definition: word of element relative to set, representation},
из равенства
\EqRef{set of coordinates, 2, omega}
следует
\ShowEq{set of coordinates, 3, omega}
Из равенства
\EqRef{set of coordinates, 3, omega}
следует корректность определения
\EqRef{set of coordinates, omega}
операции $\omega$ на множестве координат.
\end{proof}

\begin{theorem}
\label{theorem: set of coordinates, representation, am}
Определено представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $W(f,X)$.
\end{theorem}
\begin{proof}
Пусть $a\in A$. Тогда для любого
$m\in J(f,X)$
положим
\ShowEq{set of coordinates, am}
Согласно замечанию
\ref{remark: coordinates of representation},
из равенства
\EqRef{set of coordinates, am}
следует
\ShowEq{set of coordinates, 2, am}
Согласно правилу
\eqref{word of element relative to set, representation, am}
определения
\ref{definition: word of element relative to set, representation},
из равенства
\EqRef{set of coordinates, 2, am}
следует
\ShowEq{set of coordinates, 3, am}
Из равенства
\EqRef{set of coordinates, 3, am}
следует корректность определения
\EqRef{set of coordinates, am}
представления $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $W(f,X)$.
\end{proof}

\ePrints{0906.0135}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: map of words of representation, 1}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Для заданных множеств $X\subset M$, $X'\subset M$,
пусть отображение
\ShowEq{R1 X->}
согласовано со структурой представления $f$,
т. е.
\ShowEq{map of words of representation, 1}
Рассмотрим отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation, W}
удовлетворяющее условиям
\RefItem{map of words of representation, m in X},
\RefItem{map of words of representation, omega},
\RefItem{map of words of representation, am},
и такое, что
\ShowEq{map of words of representation, W in X}
Существует единственный эндоморфизм $\Omega_2$\Hyph алгебры $M$
\ShowEq{R:M->M}
определённый правилом
\ShowEq{endomorphism based on map of words of representation}
который является морфизмом представлнений
$J(f,X)$ и $J(f,X')$.
\end{theorem}
\begin{proof}
Мы будем доказывать теорему индукцией по сложности
$\Omega_2$\Hyph слова.

Если
\ShowEq{map of words of representation, w(m)=m}
то $m\in X$.
Согласно условию
\RefItem{map of words of representation, m in X},
\ShowEq{map of words of representation, R(m)=R1(m)}
Следовательно, на множестве $X$ отображения $R$ и $R_1$ совпадают,
и отображение $R$ согласовано со структурой представления $f$.

Пусть $\omega\in\Omega_2(n)$.
Пусть отображение $R$ определено для $m_1$, ..., $m_n\in J(f,X)$.
Пусть
\ShowEq{coordinates of representation, omega, 2}
Если $m=m_1...m_n\omega$, то согласно правилу
\eqref{word of element relative to set, representation, omega}
определения
\ref{definition: word of element relative to set, representation},
\ShowEq{coordinates of representation, omega}
Согласно условию
\RefItem{map of words of representation, omega},
\ShowEq{coordinates of representation, omega, 1}
Следовательно, отображение $R$ является эндоморфизмом
$\Omega_2$\Hyph алгебры $M$.

Пусть отображение $R$ определено для
\ShowEq{map of words of representation, a, m, 1}
Пусть $a\in A$.
Если $m=am_1$, то согласно правилу
\eqref{word of element relative to set, representation, am}
определения
\ref{definition: word of element relative to set, representation},
\ShowEq{map of words of representation, a, m, 2}
Согласно условию
\RefItem{map of words of representation, am},
\ShowEq{map of words of representation, a, m, 3}
Из равенства
\ePrints{1111.6035}
\ifx\Semafor\ValueOn
\xEqRef{8443-0072}{morphism of representations of F algebra, definition, 2m}
\else
\EqRef{morphism of representations of F algebra, definition, 2m}
\fi
следует, что отображение $R$ является морфизмом представления $f$.

Единственность эндоморфизма $R$, а следовательно, корректность
его определения, следует из следующего рассуждения.
Допустим, $m\in M$ имеет различные $\Omega_2$\Hyph слова относительно множества $X$,
например
\ShowEq{unique endomorphism, 1}
Так как $R$ - эндомоморфизм представления, то из равенства
\EqRef{unique endomorphism, 1}
следует
\ShowEq{unique endomorphism, 2}
Из равенства
\EqRef{unique endomorphism, 2}
следует
\ShowEq{unique endomorphism, 3}
Из равенств
\EqRef{unique endomorphism, 1},
\EqRef{unique endomorphism, 3}
следует, что равенство
\EqRef{unique endomorphism, 1}
сохраняется при отображении. Следовательно, образ $m$
не зависит от выбора координат.
\end{proof}

\begin{remark}
\label{remark: coordinates of representation, 1}
Теорема \ref{theorem: map of words of representation, 1}
- это теорема о продолжении отображения.
Единственное, что нам известно о множестве $X$ - это то, что
$X$ - множество образующих представления $f$.
Однако, между элементами множества $X$ могут существовать соотношения,
порождённые либо операциями $\Omega_2$\Hyph алгебры $M$, либо
преобразованиями представления $f$.
Поэтому произвольное отображение множества $X$, вообще говоря,
не может быть продолжено до эндоморфизма представления $f$.\footnote{В теореме
\ref{theorem: automorphism uniquely defined by image of basis},
требования к множеству образующих более жёсткие. Поэтому теорема
\ref{theorem: automorphism uniquely defined by image of basis}
говорит о продолжении произвольного отображения.
Более подробный анализ дан в замечании
\ref{remark: automorphism uniquely defined by image of basis}.}
Однако, если отображение $R_1$ согласованно со структурой представления на
множестве $X$, то мы можем построить продолжение этого отображения,
которое является эндоморфизмом представления $f$.
\qed
\end{remark}
\fi

\begin{definition}
Пусть $X$ - множество образующих представления $f$.
Пусть $R$ - эндоморфизм представления $f$.
Множество координат
\ShowEq{coordinates of endomorphism, 2, representation}
называется
\AddIndex{координатами эндоморфизма представления}
{coordinates of endomorphism, representation}.
\qed
\end{definition}

\begin{definition}
\label{definition: superposition of coordinates, representation}
Пусть $X$ - множество образующих представления $f$.
Пусть $R$ - эндоморфизм представления $f$.
Пусть $m\in M$.
Мы определим
\AddIndex{суперпозицию координат}
{superposition of coordinates, representation}
эндоморфизма представления $f$ и элемента $m$
как координаты, определённые согласно правилу
\ShowEq{superposition of coordinates, representation}
Пусть $Y\subset M$.
Мы определим
суперпозицию координат
эндоморфизма представления $f$ и множества $Y$
согласно правилу
\ShowEq{superposition of coordinates, 1, representation}
\qed
\end{definition}

\begin{theorem}
\label{theorem: map of coordinates of representation}
Эндоморфизм $R$ представления
\ShowEq{f:A->*M}
порождает отображение координат представления
\ShowEq{map of coordinates of representation}
такое, что
\ShowEq{map of coordinates of representation, 1}
\end{theorem}
\begin{proof}
Согласно замечанию
\ref{remark: coordinates of representation},
мы можем рассматривать равенства
\EqRef{superposition of coordinates, representation},
\EqRef{map of coordinates of representation}
относительно заданного множества образующих $X$.
При этом координатам $W(f,X,m)$ соответствует слово
\ShowEq{map of coordinates of representation, 2}
а координатам $W(f,X,R\circ m)$ соответствует слово
\ShowEq{map of coordinates of representation, 3}
Поэтому для того, чтобы доказать теорему,
нам достаточно показать, что отображению $W[f,X,R]$
соответствует отображение $w[f,X,R]$.
Мы будем доказывать это утверждение индукцией по сложности
$\Omega_2$\Hyph слова.

Если
\ShowEq{map of words of representation, m in X, 1}
то, согласно равенствам
\EqRef{map of coordinates of representation, 2},
\EqRef{map of coordinates of representation, 3},
отображения $W[f,X,R]$ и $w[f,X,R]$ согласованы.

Пусть для
\ShowEq{superposition of coordinates, representation, omega, 1}
отображения $W[f,X,R]$ и $w[f,X,R]$ согласованы.
Пусть $\omega\in\Omega_2(n)$.
Согласно теореме
\ref{theorem: set of coordinates, representation, omega}
\ShowEq{superposition of coordinates, representation, omega, 2}
Так как $R$ - эндоморфизм $\Omega_2$\Hyph алгебры $M$,
то из равенства
\EqRef{superposition of coordinates, representation, omega, 2}
следует
\ShowEq{superposition of coordinates, representation, omega, 3}
Из равенств
\EqRef{superposition of coordinates, representation, omega, 2},
\EqRef{superposition of coordinates, representation, omega, 3}
и предположения индукции следует, что
отображения $W[f,X,R]$ и $w[f,X,R]$ согласованы для $m=m_1...m_n\omega$.

Пусть для
$m_1\in M$
отображения $W[f,X,R]$ и $w[f,X,R]$ согласованы.
Пусть $a\in A$.
Согласно теореме
\ref{theorem: set of coordinates, representation, am}
\ShowEq{superposition of coordinates, representation, am, 1}
Так как $R$ - эндоморфизм представления $f$,
то из равенства
\EqRef{superposition of coordinates, representation, am, 1}
следует
\ShowEq{superposition of coordinates, representation, am, 2}
Из равенств
\EqRef{superposition of coordinates, representation, am, 1},
\EqRef{superposition of coordinates, representation, am, 2}
и предположения индукции следует, что
отображения $W[f,X,R]$ и $w[f,X,R]$ согласованы для $m=am_1$.
\end{proof}

\begin{corollary}
\label{corollary: map of coordinates of representation}
Пусть $X$ - множество образующих представления $f$.
Пусть $R$ - эндоморфизм представления $f$.
Отображение $W[f,X,R]$ является эндоморфизмом представления
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $W(f,X)$.
\qed
\end{corollary}

В дальнейшем мы будем отождествлять отображение $W[f,X,R]$
и множество координат $W(f,X,R\circ X)$.

\begin{theorem}
Пусть $X$ - множество образующих представления $f$.
Пусть $R$ - эндоморфизм представления $f$.
Пусть $Y\subset M$.
Тогда
\ShowEq{superposition of coordinates, 2, representation}
\end{theorem}
\begin{proof}
Равенство
\EqRef{superposition of coordinates, 2, representation}
является следствием равенства
\ShowEq{superposition of coordinates, 3, representation}
а также равенств
\EqRef{superposition of coordinates, representation},
\EqRef{superposition of coordinates, 1, representation}.
Равенство
\EqRef{superposition of coordinates, 2a, representation}
является следствием равенств
\EqRef{superposition of coordinates, 2, representation},
\EqRef{map of coordinates of representation, 1}.
\end{proof}

\begin{theorem}
Пусть $X$ - множество образующих представления $f$.
Пусть $R$, $S$ - эндоморфизмы представления $f$.
Тогда
\ShowEq{superposition of coordinates, 4, representation}
\end{theorem}
\begin{proof}
Равенство
\EqRef{superposition of coordinates, 4, representation}
следует из равенства
\EqRef{superposition of coordinates, 2, representation},
если положить $Y=\ScX$.
Равенство
\EqRef{superposition of coordinates, 4a, representation}
следует из равенства
\EqRef{superposition of coordinates, 4, representation}
и цепочки равенств
\ShowEq{superposition of coordinates, 4b, representation}
\end{proof}

Концепция суперпозиции координат очень проста
и напоминает своеобразную машину Тюринга.
Если элемент $m\in M$
имеет вид
\[m=m_1...m_n\omega\]
или
\[m=am_1\]
то мы ищем координаты элементов $m_i$, для того чтобы подставить
их в соответствующее выражение.
Как только элемент $m\in M$
принадлежит множеству образующих $\Omega_2$\Hyph алгебры $M$,
мы выбираем координаты соответствующего элемента из второго множителя.
Поэтому мы требуем, чтобы второй множитель в суперпозиции был
множеством координат образа множества образующих $X$.

Мы можем обобщить определение суперпозиции координат и предположить,
что один из множителей является множеством $\Omega_2$\Hyph слов.
Соответственно, определение суперпозиции координат имеет вид
\ShowEq{superposition of coordinates, 5, representation}

Следующие формы записи образа множества $Y$ при эндоморфизме $R$ эквивалентны.
\ShowEq{superposition of coordinates, 6, representation}
Из равенств
\EqRef{superposition of coordinates, 2, representation},
\EqRef{superposition of coordinates, 6, representation}
следует, что
\ShowEq{superposition of coordinates, 7, representation}
Равенство
\EqRef{superposition of coordinates, 7, representation}
является законом ассоциативности для операции композиции и позволяет
записать выражение
\ShowEq{superposition of coordinates, 8, representation}
без использования скобок.

Рассмотрим равенство
\EqRef{superposition of coordinates, 4, representation}
где мы видим изменение порядка эндоморфизмов в суперпозиции координат.
Это равенство также следует из цепочки равенств, где мы можем
непосредственно видеть, когда изменяется порядок эндоморфизмов
\ShowEq{superposition of coordinates, 9, representation}
Из равенства
\EqRef{superposition of coordinates, 9, representation}
следует, что координаты эндоморфизма действуют на координаты
элементы $\Omega_2$\Hyph алгебры $M$ справа.

\begin{definition}
\label{definition: endomorphism of representation, regular on set}
Пусть $X\subset M$ - множество образующих представления
\ShowEq{f:A->*M}
Пусть отображение
\ShowEq{automorphism of representation of algebra A in algebra M}
является эндоморфизмом представления $f$.
Пусть множество $X'=H\circ X$ является образом множества $X$
при отображении $H$.
Эндоморфизм $H$ представления $f$ называется
\AddIndex{невырожденным на множестве образующих}
{endomorphism of representation, regular on set} $X$,
если множество $X'$ является множеством образующих представления $f$.
В противном случае, эндоморфизм $H$ представления $f$ называется
\AddIndex{вырожденным на множестве образующих}
{endomorphism of representation, singular on set} $X$,
\qed
\end{definition}

\begin{definition}
\label{definition: regular endomorphism of representation}
Эндоморфизм представления $f$ называется
\AddIndex{невырожденным}
{regular endomorphism of representation},
если он невырожден на любом множестве образующих.
\qed
\end{definition}

\begin{theorem}
\label{theorem: Automorphism of representation is regular endomorphism}
Автоморфизм $R$ представления
\ShowEq{f:A->*M}
является невырожденным эндоморфизмом.
\end{theorem}
\begin{proof}
Пусть $X$ - множество образующих представления $f$.
Пусть $X'=\RcX$.

Согласно теореме
\ref{theorem: map of words of representation}
эндоморфизм $R$
порождает отображение $\Omega_2$\Hyph слов
$\wXR$.

Пусть $m'\in M$. Так как $R$ - автоморфизм, то существует
$m\in M$, $R\circ m=m'$. Согласно определению
\ref{definition: word of element relative to set, representation},
$\wXm$ - $\Omega_2$\Hyph слово,
представляющее $m$ относительно множества образующих $X$.
Согласно теореме
\ref{theorem: map of words of representation},
$w(f,X',m')$ - $\Omega_2$\Hyph слово,
представляющее $m'$ относительно множества образующих $X'$
\ShowEq{Automorphism of representation is regular endomorphism, 1}
Следовательно, $X'$ - множество образующих представления $f$.
Согласно определению
\ref{definition: regular endomorphism of representation},
автоморфизм $R$ - невырожден.
\end{proof}
%\fi

\section{Базис представления}
\label{section: Basis of representation}

\begin{definition}
\label{definition: basis of representation}
Если множество $X\subset M$ является множеством образующих
представления $f$, то любое множество $Y$, $X\subset Y\subset M$
также является множеством образующих представления $f$.
Если существует минимальное множество $X$, порождающее
представление $f$, то такое множество $X$ называется
\AddIndex{базисом представления}{basis of representation} $f$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: X is basis of representation}
Множество образующих $X$ представления $f$ является базисом
тогда и только тогда, когда для любого $m\in X$
множество $X\setminus\{m\}$ не является
множеством образующих представления $f$.
\end{theorem}
\begin{proof}
Пусть $X$ - множество образующих расслоения $f$.
Допустим для некоторого $m\in X$ существует $\Omega_2$\Hyph слово
\ShowEq{X is basis of representation, 1}
Рассмотрим элемент $m'$, для
которого $\Omega_2$\Hyph слово
\ShowEq{X is basis of representation, 2}
зависит от $m$.
Согласно определению
\ref{definition: word of element relative to set, representation},
любое вхождение $m$ в $\Omega_2$\Hyph слово $w'$ может быть заменено
$\Omega_2$\Hyph словом $w$. Следовательно,
$\Omega_2$\Hyph слово $w'$ не зависит от $m$,
а множество $X\setminus\{m\}$ является
множеством образующих представления $f$.
Следовательно, $X$ не является базисом расслоения $f$.
\end{proof}

\begin{remark}
\label{remark: X is basis of representation}
Доказательство теоремы
\ref{theorem: X is basis of representation}
даёт нам эффективный метод построения базиса представления $f$.
Выбрав произвольное множество образующих, мы шаг за шагом
исключаем те элементы множества, которые имеют координаты
относительно остальных элементов множества.
Если множество образующих представления бесконечно,
то рассмотренная операция может не иметь последнего шага.
Если представление имеет конечное множество образующих,
то за конечное число шагов мы можем построить базис этого представления.

Как отметил Кон в 
\citeBib{Cohn: Universal Algebra}, cтр. 96, 97,
представление может иметь неэквивалентные базисы.
Например, циклическая группа шестого порядка имеет
базисы $\{a\}$ и $\{a^2,a^3\}$, которые нельзя отобразить
один в другой эндоморфизмом представления.
\qed
\end{remark}

\begin{remark}
Мы будем записывать базис также в виде 
\ShowEq{notation for basis of representation 1}
Если базис - конечный, то мы будем также пользоваться записью
\ShowEq{notation for basis of representation 2}
\qed
\end{remark}

\begin{remark}
\label{remark: equivalence of representation}
Мы ввели $\Omega_2$\Hyph слово элемента $x\in M$ относительно множества образующих $X$
в определении
\ref{definition: word of element relative to set, representation}.
Из теоремы
\ref{theorem: X is basis of representation}
следует, что если множество образующих $X$ не является базисом,
то выбор $\Omega_2$\Hyph слова относительно множества образующих $X$ неоднозначен.
Но даже если множество образующих $X$ является базисом,
то представление $m\in M$ в виде $\Omega_2$\Hyph слова неоднозначно.
Если $m_1$, ..., $m_n$ - $\Omega_2$\Hyph слова,
$\omega\in\Omega_2(n)$ и $a\in A$, то\footnote{Например, пусть
$\{\Vector e_1,\Vector e_2\}$
- базис векторного пространства над полем $k$.
Равенство \EqRef{ambiguity of coordinates 1}
принимает форму закона дистрибутивности
\ShowEq{ambiguity of coordinates 2}
}
\ShowEq{ambiguity of coordinates 1}
Возможны равенства, связанные со спецификой представления.
Например, если $\omega$ является операцией
$\Omega_1$\Hyph алгебры $A$ и операцией
$\Omega_2$\Hyph алгебры $M$, то мы можем потребовать,
что $\Omega_2$\Hyph слова
$a_1...a_n\omega x$ и $a_1x...a_nx\omega$ описывают один и тот же
элемент $\Omega_2$\Hyph алгебры $M$.\footnote{Для векторного пространства
это требование принимает форму закона дистрибутивности
\[(a+b)\Vector e_1=a\Vector e_1+b\Vector e_1\]}

Помимо перечисленных равенств в $\Omega_2$\Hyph алгебре
могут существовать соотношения вида
\ShowEq{ambiguity of coordinates 3}
Особенностью равенства
\EqRef{ambiguity of coordinates 3}
является то, что это равенство не может быть приведенно к более
\ePrints{0906.0135}
\ifx\Semafor\ValueOff
простому виду.\footnote{Смотри, например, подразделы
\ePrints{1111.6035}
\ifx\Semafor\ValueOn
\xRef{8443-0072}{subsection: coordinates of vector in module},
\xRef{8443-0072}{subsection: Basis of R algebra}.
\else
\ref{subsection: coordinates of vector in module},
\ref{subsection: Basis of R algebra}.
\fi
}
\else
простому виду.
\fi

На множестве $\Omega_2$\Hyph слов
$w(f,X)$,
перечисленные выше равенства определяют
\AddIndex{отношение эквивалентности $\rho(f)$, порождённое представлением $f$}
{equivalence of representation}.
Очевидно, что для произвольного $m\in M$ выбор соответствующего
$\Omega_2$\Hyph слова однозначен с точностью до отношения эквивалентности
$\rho(f)$.
Тем не менее, если в процессе построений мы получим равенство двух $\Omega_2$\Hyph слов
относительно заданного базиса, мы можем утверждать, что эти $\Omega_2$\Hyph слова равны,
не заботясь об отношении эквивалентности
$\rho(f)$.%\footnote{С похожим явлением мы встретились
%в замечании
%\xRef{8433-5163}{remark: representation of tensor, ring}
%при изучении тензорного произведения.}

Аналогичное замечание касается отображения $W(f,X,m)$,
определённого в замечании
\ref{remark: coordinates of representation}.\footnote{Если базис
векторного пространства - конечен, то мы можем представить базис
в виде матрицы строки
\ShowEq{representation, vector space, basis}
Мы можем представить отображение $W(f,\Basis e,\Vector v)$
в виде матрицы столбца
\ShowEq{representation, vector space, coordinate}
Тогда
\ShowEq{representation, vector space, word}
имеет вид произведения матриц.
}
\qed
\end{remark}

\begin{theorem}
\label{theorem: Automorphism of representation maps a basis into basis}
Автоморфизм представления $f$ отображает базис
представления $f$ в базис.
\end{theorem}
\begin{proof}
Пусть отображение $R$ - автоморфизм представления $f$.
Пусть множество $X$ - базис представления $f$.
Пусть $X'=\RcX$.

Допустим множество $X'$ не является базисом.
Согласно теореме
\ref{theorem: X is basis of representation}
существует $m'\in X'$ такое, что $X'\setminus\{x'\}$
является множеством образующих представления $f$.
Согласно теореме
\ePrints{1111.6035}
\ifx\Semafor\ValueOn
\xRef{8443-0072}{theorem: group of automorphisms of representation}
\else
\ref{theorem: group of automorphisms of representation}
\fi
отображение $R^{-1}$ является автоморфизмом представления $f$.
Согласно теореме
\ref{theorem: Automorphism of representation is regular endomorphism}
и определению
\ref{definition: regular endomorphism of representation},
множество $X\setminus\{m\}$ является множеством образующих
представления $f$.
Полученное противоречие доказывает теорему.
\end{proof}

\ePrints{0912.3315,8443-0072,1111.6035}
\ifx\Semafor\ValueOn
\begin{theorem}
\label{theorem: automorphism uniquely defined by image of basis}
Пусть $X$ - базис представления $f$.
Пусть
\ShowEq{R1 X->}
произвольное отображение множества $X$.
Рассмотрим отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation, W}
удовлетворяющее условиям
\RefItem{map of words of representation, m in X},
\RefItem{map of words of representation, omega},
\RefItem{map of words of representation, am},
и такое, что
\ShowEq{map of words of representation, W in X}
Существует единственный эндоморфизм представлнения $f$\footnote{Это утверждение
похоже на теорему \citeBib{Serge Lang}-1, с. 104.}
\ShowEq{R:M->M}
определённый правилом
\ShowEq{endomorphism based on map of words of representation}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\ref{theorem: map of words of representation},
\ref{theorem: map of words of representation, 1}.
\end{proof}

\begin{corollary}
\label{corollary: automorphism uniquely defined by image of basis, representation}
Пусть $X$, $X'$ - базисы представления $f$.
Пусть $R$ - автоморфизм представления $f$
такой, что  $X'=\RcX$.
Автоморфизм $R$ определён однозначно.
\qed
\end{corollary}

\begin{remark}
\label{remark: automorphism uniquely defined by image of basis}
Теорема \ref{theorem: automorphism uniquely defined by image of basis},
так же как и
теорема \ref{theorem: map of words of representation, 1},
является теоремой о продолжении отображения.
Однако здесь $X$ - не произвольное множество образующих представления,
а базис.
Согласно замечанию
\ref{remark: X is basis of representation},
мы не можем определить координаты любого элемента базиса
через остальные элементы этого же базиса.
Поэтому отпадает необходимость в согласованности отображения базиса с представлением.
\qed
\end{remark}

\begin{theorem}
\label{theorem: coordinates of identity transformation, representation}
Набор координат $W(f,X,X)$
соответствует тождественному преобразованию
\ShowEq{identity transformation, representation}
\end{theorem}
\begin{proof}
Утверждение теоремы следует из равенства
\ShowEq{coordinates of identity transformation, representation}
\end{proof}

\begin{theorem}
\label{theorem: coordinates of inverse transformation, representation}
Пусть $W(f,X,\RcX)$ - множество координат автоморфизма $R$.
Определено множество координат $W(f,\RcX,X)$, соответствующее
автоморфизму $R^{-1}$. Множество координаты $W(f,\RcX,X)$ удовлетворяют равенству
\ShowEq{coordinates of inverse transformation, representation}
\ShowEq{coordinates of inverse transformation, a, representation}
\end{theorem}
\begin{proof}
Поскольку $R$ - автоморфизм представления $f$, то, согласно теореме
\ref{theorem: Automorphism of representation maps a basis into basis},
множество $\RcX$ - базис представления $f$. Следовательно, определено
множество координат $W(f,\RcX,X)$.
Равенство
\EqRef{coordinates of inverse transformation, representation}
следует из цепочки равенств
\ShowEq{coordinates of inverse transformation, 1, representation}
\end{proof}

\begin{remark}
\label{remark: coordinates of inverse transformation, representation}
В $\Omega_2$\Hyph алгебре $M$ не существует универсального алгоритма
определения множества координат $W(f,\RcX,X)$ для заданного множества
$W(f,X,\RcX)$.\footnote{В векторном пространстве линейному преобразованию
соответствует матрица чисел. Соответственно, обратному преобразованию
соответствует обратная матрица.
%
%Однако если мы рассмотрим представление
%алгебры Ли на группе Ли, то преобразование описывается вектором смещения.
%А именно, рассмотрим множество левоинвариантных полей группы Ли $G$
%(\citeBib)
}
Мы полагаем, что в теореме
\ref{theorem: coordinates of inverse transformation, representation}
этот алгоритм задан неявно.
Очевидно также, что множество $\Omega_2$\Hyph слов
\ShowEq{coordinates of inverse transformation, 2, representation}
вообще говоря, не совпадает с множеством $\Omega_2$\Hyph слов
\ShowEq{coordinates of inverse transformation, 3, representation}
Теорема
\ref{theorem: coordinates of inverse transformation, representation}
утверждает, что множества $\Omega_2$\Hyph слов
\EqRef{coordinates of inverse transformation, 2, representation}
и
\EqRef{coordinates of inverse transformation, 3, representation}
совпадают с точностью до отношения эквивалентности, порождённой представлением $f$.
\qed
\end{remark}

\begin{theorem}
Группа автоморфизмов $G(f)$ эффективного представления $f$
в $\Omega_2$\Hyph алгебре $M$ порождает эффективное представление
в $\Omega_2$\Hyph алгебре $M$.
\end{theorem}
\begin{proof}
Из следствия
\ref{corollary: automorphism uniquely defined by image of basis, representation}
следует, что если автоморфизм $R$ отображает базис $X$ в базис $X'$,
то множество координат $W(f,X,X')$ однозначно определяет автоморфизм $R$.
Из теоремы
\ref{theorem: map of coordinates of representation}
следует, что
множество координат $W(f,X,X')$ определяет правило
отображения координат относительно
базиса $X$ при автоморфизме представления $f$.
Из равенства
\EqRef{superposition of coordinates, 6, representation}
следует, что автоморфизм $R$ действует справа на элементы
$\Omega_2$\Hyph алгебры $M$.
Из равенства
\EqRef{superposition of coordinates, 4, representation}
следует, что представление группы является правосторонним представлением.
Согласно теореме
\ref{theorem: coordinates of identity transformation, representation}
набор координат $W(f,X,X)$
соответствует тождественному преобразованию.
Из теоремы
\ref{theorem: coordinates of inverse transformation, representation}
следует, что набор координат $W(f,\RcX,X)$
соответствует преобразованию, обратному преобразованию $W(f,X,\RcX)$.
\end{proof}

\ePrints{0912.3315}
\ifx\Semafor\ValueOff
\section{Многообразие базисов представления}
\label{section: Basis Manifold of Representation}

Множество
\ShowEq{basis manifold representation F algebra}
базисов представления $f$ называется
\AddIndex{многообразием базисов представления $f$}
{basis manifold representation F algebra}.

Согласно теореме
\ref{theorem: Automorphism of representation maps a basis into basis},
автоморфизм $R$ представления $f$
порождает преобразование
\ShowEq{active transformation, representation}
многообразия базисов представления.
Это преобразование называется
\AddIndex{активным}{active transformation of basis, representation}.
Согласно теореме
\ePrints{1111.6035}
\ifx\Semafor\ValueOn
\xRef{8443-0072}{theorem: group of automorphisms of representation},
\else
\ref{theorem: group of automorphisms of representation},
\fi
определено
\AddIndex{активное представление}{active representation in basis manifold}
\ShowEq{active representation in basis manifold}
группы $G(f)$
в многообразии базисов $\mathcal B(f)$.
Согласно следствию
\ref{corollary: automorphism uniquely defined by image of basis, representation},
это представление однотранзитивно.

\begin{remark}
Согласно замечанию
\ref{remark: X is basis of representation},
могут существовать базисы представления $f$, не связанные активным преобразованием.
В этом случае мы в качестве многообразия базисов будем рассматривать
орбиту выбранного базиса.
Следовательно, представление $f$ может иметь различные многообразия базисов.
Мы будем предполагать, что мы выбрали многообразие базисов.
\qed
\end{remark}

\ifx\texFuture\Defined
Чтобы понять нужно ли нам ограничиться автоморфизмами вида
$(id,R)$, или мы должны рассматривать произвольный автоморфизм
вида $(r,R)$, рассмотрими свободное векторное пространство $\Vector V$
над алгеброй $F$. Пусть $\Vector A$ - автоморфизм векторного пространства.
Согласно определению
\[
\Vector A(a\Vector v+b\Vector w)=
a\Vector A(\Vector v)+b\Vector A(\Vector w)
\]
Однако, если мы автоморфизм $id$ алгебры $F$ заменим на автоморфизм
\[
r(a)=dad^{-1}
\]
то приведенное равенство
примет вид
\[
\Vector A(a\Vector v+b\Vector w)=
dad^{-1}\Vector A(\Vector v)+dbd^{-1}\Vector A(\Vector w)
\]

\begin{theorem}
Если представление $f$ эффективно, то представлнение
$f_{\mathcal B}$ эффективно.
\end{theorem}
\begin{proof}
Допустим представление $f_{\mathcal B}$ неэффективно.
Следовательно, существуют
\ShowEq{effective map of basis manifold, 1}
Рассмотрим базис $X$.
Из равенства
\EqRef{effective map of basis manifold, 1}
следует
\ShowEq{effective map of basis manifold, 2}
Из равенства
\EqRef{effective map of basis manifold, 2}
и теоремы
\ref{theorem: coordinates of automorphism of representation}
следует, что координаты автоморфизмов $R_1$ и $R_2$ совпадают.
\end{proof}
\fi

\begin{definition}
\label{definition: passive transformation of basis, representation}
Автоморфизм $S$ представления $A(f)$ называется
\AddIndex{пассивным преобразованием многообразия базисов представления}
{passive transformation of basis, representation}.
Мы будем пользоваться записью
\ShowEq{passive transformation of basis, representation}
для обозначения образа базиса $X$ при пассивном преобразовании $S$.
\qed
\end{definition}

\begin{theorem}
Пассивное преобразование базиса имеет вид
\ShowEq{passive transformation, representation}
\end{theorem}
\begin{proof}
Согласно равенству
\EqRef{active transformation, representation},
активное преобразование действует на координаты
базиса справа.
Равенство
\EqRef{passive transformation, representation}
следует из теорем
\ePrints{1111.6035}
\ifx\Semafor\ValueOn
\xRef{8443-0072}{theorem: shift is automorphism of representation},
\xRef{8443-0072}{theorem: two representations of group},
\xRef{8443-0072}{theorem: twin representations of group, automorphism},
\else
ref{theorem: shift is automorphism of representation},
\ref{theorem: two representations of group},
\ref{theorem: twin representations of group, automorphism},
\fi
согласно которым
пассивное преобразование действует на координаты
базиса слева.
\end{proof}

\begin{theorem}
\label{theorem: select second basis of representation}
Пусть $S$ - пассивное преобразование
многообразия базисов представления $f$.
Пусть $X$ - базис представления $f$, $X'=\SsX$.
Пусть для базиса $Y$ существует активное преобразование $R$ такое,
что $Y=\RcX$. Положим
\ShowEq{select second basis of representation, 1}
Тогда $S\star Y=Y'$.
\end{theorem}
\begin{proof}
Согласно равенству
\EqRef{active transformation, representation},
активное преобразование координат базиса $Y$ имеет вид
\ShowEq{active transformation, representation, 1}
Пусть $Y''=S\star Y$.
Из равенства
\EqRef{passive transformation, representation}
следует, что
\ShowEq{passive transformation, representation, 1}
Из совпадения выражений в равенствах
\EqRef{active transformation, representation, 1},
\EqRef{passive transformation, representation, 1}
следует, что
\ShowEq{passive and active maps, representation, 1}
Следовательно, коммутативна диаграмма
\ShowEq{passive and active maps}
\end{proof}

\begin{theorem}
\label{theorem: passive representation in basis manifold}
Существует однотранзитивное
\AddIndex{пассивное представление}{passive representation in basis manifold}
\ShowEq{passive representation in basis manifold}
\end{theorem}
\begin{proof}
Поскольку $A(f)$ - однотранзитивное представление группы $G(f)$,
то согласно определению
\ref{definition: passive transformation of basis, representation}
и теореме
\ePrints{1111.6035}
\ifx\Semafor\ValueOn
\xRef{8443-0072}{theorem: group of automorphisms of representation},
\else
\ref{theorem: group of automorphisms of representation},
\fi
множество пассивных преобразований порождает группу.
\end{proof}

Пусть пассивное преобразование $S$ отображает базис $Y$ в базис
\ShowEq{passive transformation S, representation}
Пусть пассивное преобразование $T$ отображает базис $Y'$ в базис
\ShowEq{passive transformation T, representation}
Обозначим $T\star S$ произведение пассивных преобразований $T$ и $S$
\ShowEq{passive transformation T S 1, representation}
Из равенств
\EqRef{passive transformation S, representation},
\EqRef{passive transformation T, representation}
следует, что
\ShowEq{passive transformation T S 2, representation}
Из равенств
\EqRef{passive transformation T S 1, representation},
\EqRef{passive transformation T S 2, representation}
и теоремы
\ref{theorem: passive representation in basis manifold}
следует, что
\ShowEq{passive transformation T S 3, representation}

\section{Геометрический объект представления универсальной алгебры}
\label{section: Geometric Object of Representation of Universal Algebra}

Активное преобразование изменяет базисы и
элементы $\Omega_2$\Hyph алгебры согласовано
и координаты элемента относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к изменению
координат элемента относительно базиса.

Допустим пассивное преобразование $S\in G(f)$ отображает
базис $Y\in\mathcal{B}(f)$
в базис $Y'\in\mathcal{B}(f)$
\ShowEq{passive transformation of representation}
Допустим элемент $m\in M$ имеет $\Omega_2$\Hyph слово
\ShowEq{Omega_2 word in representation, basis Y}
относительно базиса $Y$ и имеет $\Omega_2$\Hyph слово
\ShowEq{Omega_2 word in representation, basis Y prim}
относительно базиса $Y'$.
Из \EqRef{passive transformation of representation}
и \EqRef{Omega_2 word in representation, basis Y prim} следует, что
\ShowEq{Omega_2 word in representation, basis Y, 1}
Сравнивая \EqRef{Omega_2 word in representation, basis Y}
и \EqRef{Omega_2 word in representation, basis Y, 1} получаем, что
\ShowEq{coordinate transformation in representation, 1}
Так как $S$ - автоморфизм представления, то
из \EqRef{coordinate transformation in representation, 1}
и теоремы
\ref{theorem: coordinates of inverse transformation, representation}
следует
\ShowEq{coordinate transformation in representation}
Преобразование координат \EqRef{coordinate transformation in representation}
не зависит от элемента $m$ или базиса $Y$, а
определенно исключительно координатами элемента $m$
относительно базиса $Y$.

\begin{theorem}
Преобразования координат \EqRef{coordinate transformation in representation}
порождают эффективное
правостороннее представление группы $G(f)$, называемое
\AddIndex{координатным представлением в $\Omega_2$\Hyph алгебре}
{coordinate representation, Omega_2 algebra}.
\end{theorem}
\begin{proof}
Согласно следствию
\ref{corollary: map of coordinates of representation},
преобразование
\EqRef{coordinate transformation in representation}
является эндоморфизмом представления
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $W(f,X)$.\footnote{Это преобразование
не порождает эндоморфизма представления $f$. Координаты меняются, поскольку меняется
базис, относительно которого мы определяем координаты. Однако элемент
$\Omega_2$\Hyph алгебры $M$, координаты которого мы рассматриваем, не меняется.}

Допустим мы имеем два последовательных пассивных преобразования
$S$ и $T$. Преобразование координат
\EqRef{coordinate transformation in representation}
соответствует пассивному преобразованию $S$.
Преобразование координат
\ShowEq{coordinate transformation in representation, T}
соответствует пассивному преобразованию $T$. Произведение
преобразований координат \EqRef{coordinate transformation in representation}
и \EqRef{coordinate transformation in representation, T} имеет вид
\ShowEq{coordinate transformation in representation, TS}
и является координатным преобразованием,
соответствующим пассивному преобразованию
\ShowEq{coordinate transformation in representation, TS 1}
Это доказывает, что преобразования координат
порождают
правостороннее представление группы $G(f)$.

Если координатное преобразование не изменяет координаты выбранного базиса,
то ему соответствует единица группы $G(f)$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
\end{proof}

Пусть $f$ - представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Пусть $g$ - представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_3$\Hyph алгебре $N$.
Пассивное представление $g_p$ согласовано
с пассивным представлением $f_p$,
если существует гомоморфизм $h$ группы $G(f)$ в группу $G(g)$.
Рассмотрим диаграмму\footnote{Мы можем ослабить определение согласованности
представлений и предположить, что $N$ - $\Omega_2$\Hyph алгебра.
Тогда нам достаточно потребовать, чтобы отображение $(h,H)$
было морфизмом представлений. Но тогда элементы аффинного представления
не могут быть геометрическим объектом векторного пространства.}
\ShowEq{passive representation coordinated with passive representation}
Так как отображения $P(f)$, $P(g)$ являются изоморфизмами группы,
то отображение $H$ является гомоморфизмом групп.
Следовательно, отображение $f'$ является представлением группы $G(f)$
в многообразии базисов $\mathcal B(g)$.
Согласно построению, пассивному преобразованию $S$
$\Omega_2$\Hyph алгебры $M$
соответствует пассивное преобразование $H(S)$
$\Omega_3$\Hyph алгебры $N$.
\ShowEq{passive transformation of representation g}
Тогда координатное преобразование в $N$ принимает вид
\ShowEq{coordinate transformation, representation g}

\begin{definition}
\label{definition: geometric object, coordinate representation, representation g}
Мы будем называть орбиту
\ShowEq{geometric object, coordinate representation g}%
\AddIndex{геометрическим объектом в координатном представлении,
определённом в $\Omega_2$\Hyph алгебре $M$}
{geometric object, coordinate representation g}.
Для любого базиса
\ShowEq{geometric object 1, coordinate representation}
соответствующая точка \EqRef{coordinate transformation, representation g}
орбиты  определяет
\AddIndex{координаты геометрического объекта в координатном пространстве представления}
{coordinates of geometric object, coordinate representation}
относительно базиса $Y'_M$.
\qed
\end{definition}

\begin{definition}
\label{definition: geometric object, representation g}
Мы будем называть орбиту
\ShowEq{geometric object, representation g}%
\AddIndex{геометрическим объектом, определённым в $\Omega_2$\Hyph алгебре}
{geometric object, representation g}
$M$.
Для любого базиса
\ShowEq{geometric object 1, representation}
соответствующая точка \EqRef{coordinate transformation, representation g}
орбиты  определяет
\AddIndex{координаты геометрического объекта в $\Omega_2$\Hyph алгбре}
{coordinates of geometric object, representation g} $M$
относительно базиса $Y'_M$
и соответствующий вектор
\ShowEq{geometric object 2, representation g}%
называется
\AddIndex{представителем геометрического объекта в $\Omega_2$\Hyph алгбре}
{representative of geometric object, representation g}
$M$.
\qed
\end{definition}

Так как геометрический объект - это орбита представления,
то согласно теореме
\ePrints{MRepro}
\ifx\Semafor\ValueOn
\xRef{8443-0072}{theorem: proper definition of orbit}
\else
\ref{theorem: proper definition of orbit}
\fi
определение геометрического объекта корректно.

Мы будем также говорить, что $p$ - это
\AddIndex{геометрический объект типа $H$}{geometric object of type H, representation g}

Определение \ref{definition: geometric object, coordinate representation, representation g}
строит геометрический объект в координатном пространстве.
Определение \ref{definition: geometric object, representation g} предполагает,
что мы выбрали базис представления $g$.
Это позволяет использовать представитель геометрического объекта
вместо его координат.

\begin{theorem}[\AddIndex{принцип инвариантности}{invariance principle, representation g}]
\label{theorem: invariance principle, representation g}
Представитель геометрического объекта не зависит от выбора
базиса $Y'_M$.
\end{theorem}
\begin{proof}
Чтобы определить представителя геометрического объекта,
мы должны выбрать базис $Y_M$,
базис
$Y_P$
и координаты геометрического объекта
$W(g,Y_P,p)$. Соответствующий представитель геометрического
объекта имеет вид
\ShowEq{invariance principle 1, representation}
Базис $Y'_M$ связан с базисом
$Y_M$ пассивным преобразованием
\ShowEq{invariance principle 2, representation}
Согласно построению это порождает пассивное преобразование
\EqRef{passive transformation of representation g}
и координатное преобразование
\EqRef{coordinate transformation, representation g}. Соответствующий
представитель геометрического объекта имеет вид
\ShowEq{invariance principle 3, representation}
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
\end{proof}

\begin{theorem}
Множество геометрических объектов типа $H$
является $\Omega_3$\Hyph алгеброй.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{geometric object, 1, omega}
Для операции
\ShowEq{geometric object, 2, omega}
мы положим
\ShowEq{geometric object, 3, omega}
Так как для произвольного эндоморфизма $S$ $\Omega_2$\Hyph алгебры
$M$ отображение $W(g,H(S)\star Y_N,Y_N)$ является эндоморфизмом
$\Omega_3$\Hyph алгебры $N$, то определение
\EqRef{geometric object, 3, omega}
корректно.
\end{proof}

\begin{theorem}
Определено представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_3$\Hyph алгебре $N$ геометрических объектов типа $H$.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{geometric object, 1, am}
Для $a\in A$
мы положим
\ShowEq{geometric object, 3, am}
Так как для произвольного эндоморфизма $S$ $\Omega_2$\Hyph алгебры
$M$ отображение $W(g,H(S)\star Y_N,Y_N)$ является эндоморфизмом
представления $g$, то определение
\EqRef{geometric object, 3, am}
корректно.
\end{proof}
\fi

\section{Примеры базиса представления универсальной алгебры}

\subsection{Векторное пространство}
Рассмотрим векторное пространство $\Vector V$ над полем $F$.
Если дано множество векторов
\ShowEq{representation, set of vectors}
то, согласно алгоритму построения координат над векторным пространством,
координаты включают такие элементы как $\Vector e_1+\Vector e_2$ и
$a\Vector e_1$.
Рекурсивно применяя правила, приведенные в определении
\ref{definition: word of element relative to set, representation},
мы придём к выводу, что множество векторов
\ShowEq{representation, set of vectors}
порождает множество линейных комбинаций
\ShowEq{representation, set of vectors, linear combination}
Согласно теореме \ref{theorem: X is basis of representation},
множество векторов
\ShowEq{representation, set of vectors}
является базисом при условии, если для любого $i$, $i=1$, ..., $n$,
вектор $\Vector e_i$ не является линейной комбинацией остальных векторов.
Это требование равносильно требованию линейной независимости векторов.

\subsection{Представление группы на множестве}
\label{subsection: representation of group on the set, basis}
Рассмотрим представление из примера
\ePrints{1111.6035}
\ifx\Semafor\ValueOn
\xRef{8443-0072}{subsection: representation of group on the set}.
\else
\ref{subsection: representation of group on the set}.
\fi
Мы можем рассматривать множество $M$ как объединение орбит представления группы $G$.
В качестве базиса представления можно выбрать
множество точек таким образом, что одна и только одна точка
принадлежит каждой орбите представления.
Если $X$ - базис представления, $A\in X$, $g\in G$, то $\Omega_2$\Hyph слово
имеет вид $A+g$. Поскольку на множестве $M$ не определены операции,
то не существует $\Omega_2$\Hyph слово, содержащее различные элементы базиса.
Если представление группы $G$ однотранзитивно,
то базис представления состоит из одной точки.
Этой точкой может быть любая точка множества $M$.
\fi

\ifx\texFuture\Defined
\begin{theorem}
Пусть представление абелевой группы $G$ на множестве $M$ не однотранзитивно.
Существует  абелевая группа $G_1$, $G\subset G$, такая, что для $g\in G$ действие групп
$G$ и $G_1$ совпадают, но представление группы $G_1$ однотранзитивно.
\end{theorem}
\begin{proof}
Пусть $X$ - базис представления группы $G$ на множестве $M$.
Рассмотрим множество кортежей
\ShowEq{representation of group on the set, extension}
Мы определим сложение на множестве $G_2$
\ShowEq{representation of group on the set, extension sum}
порождает абелевую группу.
\end{proof}
\fi

%\section{Теорема о существовании базиса}

\ifx\texFuture\Defined
\section{Тензорное произведение алгебр}
\section{парные представления универсальной алгебры}
\fi


==> Tstar.Representation.Russian.tex <==
%auto-ignore
\input{Tstar.Representation.Eq}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\chapter{Представление универсальной алгебры}
\label{chapter: Representation of Algebra}
\else
\chapter{Представление группы}
\label{chapter: Representation of Group}
\fi

\section{Представление универсальной алгебры}

\begin{definition}
\label{definition: transformation of universal algebra}
\ePrints{0906.0135}
\ifx\Semafor\ValueOn
Пусть\footnote{Определения и теоремы из этой главы
включены также в главы
\xRef{8443-0072}{chapter: Representation of Algebra},
\xRef{8443-0072}{chapter: Basis of Representation of Universal Algebra}.
}
\else
Пусть
\fi
на множестве $M$ определена структура $\Omega_2$\Hyph алгебры
(\citeBib{Burris Sankappanavar,Cohn: Universal Algebra}).
Эндоморфизм
$\Omega_2$\Hyph алгебры
\ShowEq{t:M->M}
называется \AddIndex{преобразованием универсальной алгебры}
{transformation of universal algebra} $M$.\footnote{Если множество
операций $\Omega_2$\Hyph алгебры пусто, то
\ShowEq{t:M->M}
является отображением.}
\qed
\end{definition}

Мы будем обозначать
\symb{\delta}{identical transformation}1
тождественное преобразование.

\begin{definition}
\label{definition: left-side representation of algebra} 
Пусть
\ShowEq{set of left-side transformations}
- множество
\AddIndex{левосторонних преобразований}{left-side transformation}
\[
u'=t u
\]
$\Omega_2$\Hyph алгебры $M$.
Пусть на множестве ${}^*M$ определена структура $\Omega_1$\Hyph алгебры.
Гомоморфизм
\ShowEq{left-side representation of algebra}
$\Omega_1$\Hyph алгебры $A$ в
$\Omega_1$\Hyph алгебру ${}^*M$
называется
\AddIndex{левосторонним представлением $\Omega_1$\Hyph алгебры $A$}
{left-side representation of algebra}
или
\AddIndex{\Ts{A}представлением}{A* representation of algebra}
в $\Omega_2$\Hyph алгебре $M$.
\qed
\end{definition}

\begin{definition}
\label{definition: right-side representation of algebra} 
Пусть
\ShowEq{set of right-side transformations}
- множество
\AddIndex{правосторонних преобразований}{right-side transformation}
\[
u'= ut
\]
$\Omega_2$\Hyph алгебры $M$.
Пусть на множестве $M^*$ определена структура $\Omega_1$\Hyph алгебры.
Гомоморфизм
\ShowEq{right-side representation of algebra}
$\Omega_1$\Hyph алгебры $A$ в
$\Omega_1$\Hyph алгебру $M^*$
называется
\AddIndex{правосторонним представлением $\Omega_1$\Hyph алгебры $A$}
{right-side representation of algebra} или
\AddIndex{\sT{A}представлением}{*A representation of algebra}
в $\Omega_2$\Hyph алгебре $M$.
\qed
\end{definition}

\ePrints{4993-2400}
\ifx\Semafor\ValueOff
Мы распространим на теорию представлений соглашение, описанное в
\ePrints{0912.3315,0906.0135}
\ifx\Semafor\ValueOn
замечаниях
\xRef{0701.238}{remark: left and right matrix notation},
\xRef{4776-3181}{remark: left and right matrix notation}.
\else
замечании
\ePrints{0803.2620}
\ifx\Semafor\ValueOn
\xRef{0701.238}{remark: left and right matrix notation}.
\else
\ePrints{0501.237}
\ifx\Semafor\ValueOn
\xRef{0612.111}{remark: left and right matrix notation}.
\else
\ref{remark: left and right matrix notation}.
\fi
\fi
\fi
Мы можем записать принцип двойственности
в следующей форме
\fi

\begin{theorem}[принцип двойственности]
\label{theorem: duality principle, algebra representation}
Любое утверждение, справедливое для
левостороннего представления $\Omega_1$\Hyph алгебры $A$,
будет справедливо для правостороннего представления $\Omega_1$\Hyph алгебры $A$.
\end{theorem}

\begin{remark}
\label{remark: duality principle, algebra representation}
Существует две формы записи преобразования $\Omega_2$\Hyph алгебры $M$.
Если мы пользуемся операторной записью, то преобразование $A$
записывается в виде $Aa$ или $aA$, что соответствует
левостороннему преобразованию или правостороннему преобразованию.
Если мы пользуемся функциональной записью, то преобразование $A$
записывается в виде $A(a)$ независимо от того, это
левостороннее или правостороннее преобразование.
Эта запись согласована с принципом двойственности.

Это замечание является основой следующего соглашения.
Когда мы пользуемся функциональной записью, мы не различаем
левостороннее и правостороннее преобразование.
Мы будем обозначать
\symb{{}^* M}{set of transformations}1
множество преобразований $\Omega_2$\Hyph алгебры $M$.
Пусть на множестве ${}^* M$ определена структура $\Omega_1$\Hyph алгебры.
Пусть $A$ является $\Omega_1$\Hyph алгеброй.
Мы будем называть гомоморфизм
\begin{equation}
f:A\rightarrow {}^* M
\EqLabel{representation of algebra}
\end{equation}
\AddIndex{представлением $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$}
{representation of algebra}.
Мы будем также пользоваться записью
\ShowEq{representation A in M}
для обозначения представления $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.

Соответствие между операторной записью и функциональной записью однозначно.
Мы можем выбирать любую форму записи, которая удобна для изложения конкретной темы.
\qed
\end{remark}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
Существует несколько способов описать представление.
Мы можем указать отображение $f$, имея в виду что область определения -
это $\Omega_1$\Hyph алгебра $A$ и область значений - это $\Omega_1$\Hyph алгебра ${}^*M$.
Либо мы можем указать $\Omega_1$\Hyph алгебру $A$
и $\Omega_2$\Hyph алгебру $M$, имея в виду что нам известна структура
отображения $f$.\footnote{Например, мы рассматриваем векторное пространство $\Vector V$ над
полем $D$ (
\ePrints{0906.0135,0912.3315}
\ifx\Semafor\ValueOn
определение \xRef{0701.238}{definition: Tstar vector space}
\else
\ePrints{4993-2400,0701.238}
\ifx\Semafor\ValueOff
подраздел \ref{subsection: Vector Space}
\else
definition \ref{definition: Tstar vector space}
\fi
\fi
).
}

Диаграмма
\[
\xymatrix{
M\ar[rr]^{f(a)}&&M\\
&A\ar@{=>}[u]^f&
}
\]
означает, что мы рассматриваем представление $\Omega_1$\Hyph алгебры $A$.
Отображение $f(a)$ является образом $a\in A$.
\fi

\begin{definition}
\label{definition: effective representation of algebra}
Мы будем называть представление $\Omega_1$\Hyph алгебры $A$
\AddIndex{эффективным}{effective representation of algebra},
если отображение \EqRef{representation of algebra} -
изоморфизм $\Omega_1$\Hyph алгебры $A$ в ${}^* M$.
\qed
\end{definition}

\begin{remark}
\label{remark: notation for effective representation of algebra}
Если левостороннее представление $\Omega_1$\Hyph алгебры эффективно, мы можем отождествлять
элемент $\Omega_1$\Hyph алгебры с его образом и записывать левостороннее преобразование,
порождённое элементом $a\in A$,
в форме
\[v'=av\]
Если правостороннее представление $\Omega_1$\Hyph алгебры эффективно, мы можем отождествлять
элемент $\Omega_1$\Hyph алгебры с его образом и записывать правостороннее преобразование,
порождённое элементом $a\in A$,
в форме
\[v'=va\]
\qed
\end{remark}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{definition}
\label{definition: transitive representation of algebra}
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{транзитивным}{transitive representation of algebra},
если для любых $a, b \in V$ существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of algebra},
если оно транзитивно и эффективно.
\qed
\end{definition}

\begin{theorem}%однотранзитивное
\label{theorem: Representation is single transitive iff}
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in M$
существует одно и только одно $g\in A$ такое, что $a=f(g)(b)$
\end{theorem}
\begin{proof}
Следствие определений \ref{definition: effective representation of algebra}
и \ref{definition: transitive representation of algebra}.
\end{proof}

\section{Морфизм представлений
универсальной алгебры}

\begin{theorem}
Пусть $A$ и $B$ - $\Omega_1$\Hyph алгебры.
Представление $\Omega_1$\Hyph алгебры $B$
\[
g:B\rightarrow {}^\star M
\]
и гомоморфизм $\Omega_1$\Hyph алгебры
\begin{equation}
h:A\rightarrow B
\EqLabel{homomorphism of algebra F}
\end{equation}
определяют представление $f$ $\Omega_1$\Hyph алгебры $A$
\[
\xymatrix{
A\ar[dr]^h\ar[rr]^f&&{}^* M\\
&B\ar[ur]^g&
}
\]
\end{theorem}
\begin{proof}
Отображение $f$ является гомоморфизмом $\Omega_1$\Hyph алгебры $A$ в
$\Omega_1$\Hyph алгебру ${}^* M$,
так как отображение $g$ является гомоморфизмом $\Omega_1$\Hyph алгебры $B$ в
$\Omega_1$\Hyph алгебру ${}^* M$.
\end{proof}

Если мы изучаем представление $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебрах $M$ и $N$, то нас интересуют отображения
из $M$ в $N$, сохраняющие структуру представления.
\fi

\begin{definition}
\label{definition: morphism of representations of F algebra}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$ и 
\ShowEq{g:B->*N}
представление $\Omega_1$\Hyph алгебры $B$
в $\Omega_2$\Hyph алгебре $N$.
Пара отображений
\ShowEq{morphism of representations of F algebra, definition, 1}
таких, что
\begin{itemize}
\item $r$ - гомоморфизм $\Omega_1$\Hyph алгебры
\item $R$ - гомоморфизм $\Omega_2$\Hyph алгебры
\item
\ShowEq{morphism of representations of F algebra, definition, 2}
\end{itemize}
называется
\AddIndex{морфизмом представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре}
{morphism of representations of Omega1 algebra in Omega2 algebra}.
\qed
\end{definition}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{remark}
Мы можем рассматривать пару отображений $r$, $R$ как отображение
\[
F:A\cup M\rightarrow B\cup N
\] такое, что
\[
F(A)=B \ \ \ \ F(M)=N
\]
Поэтому в дальнейшем мы будем говорить, что дано отображение $(r,R)$.
\qed
\end{remark}

\begin{definition}
Если представления $f$ и $g$ совпадают, то морфизм представлений $(r,R)$ называется
\AddIndex{морфизмом представления $f$}{morphism of representation f}.
\qed
\end{definition}

Для произвольного $m\in M$ равенство
\EqRef{morphism of representations of F algebra, definition, 2}
имеет вид
\ShowEq{morphism of representations of F algebra, definition, 2m}

\ePrints{8443-0072}
\ifx\Semafor\ValueOff
\begin{remark}
Рассмотрим морфизм представлений
\EqRef{morphism of representations of F algebra, definition, 1}.
Мы можем обозначать элементы множества $B$, пользуясь буквой по образцу $b\in B$.
Но если мы хотим показать, что $b$ является образом элемента $a\in A$,
мы будем пользоваться обозначением $\RedText{r(a)}$.
Таким образом, равенство
\[
\RedText{r(a)}=r(a)
\]
означает, что $\RedText{r(a)}$ (в левой части равенства)
является образом $a\in A$ (в правой части равенства).
Пользуясь подобными соображениями, мы будем обозначать
элемент множества $N$ в виде $\BlueText{R(m)}$.
Мы будем следовать этому соглащению, изучая соотношения
между гомоморфизмами $\Omega_1$\Hyph алгебр
и отображениями между множествами,
где определены соответствующие представления.
\qed
\end{remark}
\fi

\begin{remark}
\label{remark: morphism of representations of F algebra}
Мы можем интерпретировать
\EqRef{morphism of representations of F algebra, definition, 2m}
двумя способами
\begin{itemize}
\item Пусть преобразование $\BlueText{f(a)}$ отображает $m\in M$
в $\BlueText{f(a)}(m)$.
Тогда преобразование $g(\RedText{r(a)})$ отображает
$\BlueText{R(m)}\in N$ в $\BlueText{R(f(a)(m))}$.
\item Мы можем представить морфизм представлений из $f$ в $g$,
пользуясь диаграммой
\ShowEq{morphism of representations of F algebra, definition, 2m 1}
Из \EqRef{morphism of representations of F algebra, definition, 2}
следует, что диаграмма $(1)$ коммутативна.
\end{itemize}
\qed
\end{remark}

\begin{theorem}
\label{theorem: morphism of representations and algebra}
Рассмотрим представление
\ShowEq{f:A->*M}
$\Omega_1$\Hyph алгебры $A$ 
и представление
\ShowEq{g:B->*N}
$\Omega_1$\Hyph алгебры $B$.
Морфизм
\[
\xymatrix{
h:A\ar[r]&B&H:M\ar[r]&N
}
\]
представлений из $f$ в $g$
удовлетворяет соотношению
\ShowEq{morphism of representations of F algebra, 1}
для произвольной $n$-арной операции $\omega$ $\Omega_1$\Hyph алгебры.
\end{theorem}
\begin{proof}
Так как $f$ - гомоморфизм, мы имеем
\ShowEq{morphism of representations of F algebra, 2}
Из \EqRef{morphism of representations of F algebra, definition, 2} и
\EqRef{morphism of representations of F algebra, 2} следует
\ShowEq{morphism of representations of F algebra, 3}
Так как $h$ - гомоморфизм, из
\EqRef{morphism of representations of F algebra, 3} следует
\ShowEq{morphism of representations of F algebra, 4}
Так как $g$ - гомоморфизм, из
\EqRef{morphism of representations of F algebra, 4} следует
\EqRef{morphism of representations of F algebra, 1}.
\end{proof}

\begin{theorem}
\label{theorem: morphism of representations and homomorphism of algebra}
Пусть отображение
\ShowEq{morphism representation hH}
является морфизмом из представления
\ShowEq{f:A->*M}
$\Omega_1$\Hyph алгебры $A$ в представление
\ShowEq{g:B->*N}
$\Omega_1$\Hyph алгебры $B$.
Если представление $f$ эффективно, то отображение
\[
{}^*H:{}^* M\rightarrow{}^* N
\]
определённое равенством
\ShowEq{morphism of representations, star morphism}
является гомоморфизмом $\Omega_1$\Hyph алгебры.
\end{theorem}
\begin{proof}
Так как представление $f$ эффективно, то для выбранного преобразования
$\BlueText{f(a)}$ выбор элемента $a$ определён однозначно.
Следовательно, преобразование $\RedText{g(h(a))}$
в равенстве \EqRef{morphism of representations, star morphism}
определено корректно.

Так как $f$ - гомоморфизм, мы имеем
\begin{equation}
{}^*H(\omega(f(a_1),...,f(a_n)))={}^*H(f(\omega(a_1,...,a_n)))
\EqLabel{morphism of representations, star morphism, 2}
\end{equation}
Из \EqRef{morphism of representations, star morphism} и
\EqRef{morphism of representations, star morphism, 2} следует
\begin{equation}
{}^*H(\omega(f(a_1),...,f(a_n)))=g(h(\omega(a_1,...,a_n)))
\EqLabel{morphism of representations, star morphism, 3}
\end{equation}
Так как $h$ - гомоморфизм, из
\EqRef{morphism of representations, star morphism, 3} следует
\begin{equation}
{}^*H(\omega(f(a_1),...,f(a_n)))=g(\omega(h(a_1),...,h(a_n)))
\EqLabel{morphism of representations, star morphism, 4}
\end{equation}
Так как $g$ - гомоморфизм,
\[
{}^*H(\omega(f(a_1),...,f(a_n)))=\omega(g(h(a_1)),...,g(h(a_n)))
=\omega({}^*H(f(a_1)),...,{}^*H(f(a_n)))
\]
следует из
\EqRef{morphism of representations, star morphism, 4}.
Следовательно, отображение ${}^*H$ является гомоморфизмом $\Omega_1$\Hyph алгебры.
\end{proof}

\begin{theorem}
\label{theorem: morphism of representations of F algebra}
Пусть
\ShowEq{f:A->*M}
однотранзитивное представление $\Omega_1$\Hyph алгебры $A$ и
\ShowEq{g:B->*N}
однотранзитивное представление $\Omega_1$\Hyph алгебры $B$.
Если отображение
\ShowEq{h:A->B}
является гомоморфизмом $\Omega_1$\Hyph алгебры,
то существует морфизм
представлений из $f$ в $g$
\ShowEq{morphism representation hH}
\end{theorem}
\begin{proof}
Выберем гомоморфизм $h$.
Выберем элемент $m\in M$
и элемент $n\in N$. 
Чтобы построить отображение $H$, рассмотрим следующую диаграмму
\ShowEq{morphism representation hH, diagram}
Из коммутативности диаграммы $(1)$ следует
\ShowEq{morphism representation =}
Для произвольного $m'\in M$ однозначно определён $a\in A$ такой, что
\ShowEq{m'=.m}
Следовательно, мы построили отображении $H$,
которое удовлетворяет равенству
\EqRef{morphism of representations of F algebra, definition, 2}.
\end{proof}

\begin{theorem}
\label{theorem: unique morphism of representations of F algebra}
Если представление
\ShowEq{f:A->*M}
$\Omega_1$\Hyph алгебры $A$ однотранзитивно
и представление
\ShowEq{g:B->*N}
$\Omega_1$\Hyph алгебры $B$ однотранзитивно,
то для заданного гомоморфизма $\Omega_1$\Hyph алгебры
\[
\xymatrix{
h:A\ar[r]&B
}
\]
гомоморфизм $\Omega_2$\Hyph алгебры
\[
\xymatrix{
H:M\ar[r]&N
}
\]
такой, что $(h,H)$ является морфизмом
представлений из $f$ в $g$,
определён однозначно
с точностью до выбора образа $n=H(m)\in N$
заданного элемента $m\in M$.
\end{theorem}
\begin{proof}
Из доказательства теоремы
\ref{theorem: morphism of representations of F algebra}
следует, что выбор гомоморфизма $h$ и элементов
$m\in M$, $n\in N$ однозначно определяет отображение $H$.
\end{proof}

\begin{theorem}
Если представление
\ShowEq{f:A->*M}
$\Omega_1$\Hyph алгебры $A$ однотранзитивно,
то для любого эндоморфизма $h$ $\Omega_1$\Hyph алгебры $A$ существует морфизм
представления $f$
\ShowEq{morphism representation hH AA}
\end{theorem}
\begin{proof}
Рассмотрим следующую диаграмму
\ShowEq{morphism representation hH diagram}
Утверждение теоремы является следствием теоремы
\ref{theorem: morphism of representations of F algebra}.
\end{proof}

\begin{theorem}
\label{theorem: product of morphisms of representations of F algebra}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$,
\ShowEq{g:B->*N}
представление $\Omega_1$\Hyph алгебры $B$,
\[
h:C\rightarrow {}^* L
\]
представление $\Omega_1$\Hyph алгебры $C$.
Пусть определены морфизмы представлений $\Omega_1$\Hyph алгебры
\[
\xymatrix{
p:A\ar[r]&B&P:M\ar[r]&N
}
\]
\[
\xymatrix{
q:B\ar[r]&C&Q:N\ar[r]&L
}
\]
Тогда определён морфизм представлений $\Omega_1$\Hyph алгебры
\[
\xymatrix{
r:A\ar[r]&C&R:M\ar[r]&L
}
\]
где $r=qp$, $R=QP$.
Мы будем называть морфизм $(r,R)$ представлений из $f$ в $h$
\AddIndex{произведением морфизмов $(p,P)$ и $(q,Q)$
представлений универсальной алгебры}
{product of morphisms of representations of universal algebra}.
\end{theorem}
\begin{proof}
Мы можем представить утверждение теоремы,
пользуясь диаграммой
\ShowEq{product of morphisms of representations of F algebra}
Отображение $r$ является гомоморфизмом $\Omega_1$\Hyph алгебры $A$ в
$\Omega_1$\Hyph алгебру $C$.
Нам надо показать, что пара отображений $(r,R)$ удовлетворяет
\EqRef{morphism of representations of F algebra, definition, 2}:
\ShowEq{product of morphisms of representations of F algebra, 1}
\end{proof}

\begin{definition}
\label{definition: category of representations of F algebra from category}
Допустим $\mathcal A$ категория $\Omega_1$\Hyph алгебр.
Мы определим \AddIndex{категорию
\ShowEq{category of left-side representations}
$\ $ левосторонних представлений}
{category of left-side representations}
универсальной алгебры из категории $\mathcal A$.
Объектами этой категории являются левосторонние представлениями $\Omega_1$\Hyph алгебры.
Морфизмами этой категории являются морфизмы левосторонних представлений $\Omega_1$\Hyph алгебры.
\qed
\end{definition}

\begin{definition}
\label{definition: transformation coordinated with equivalence}
Пусть на множестве $M$ определена эквивалентность $S$.
Преобразование $f$ называется
\AddIndex{согласованным с эквивалентностью}{transformation coordinated with equivalence} $S$,
если из условия
\ShowEq{m1 m2 modS}
следует
$f(m_1)\equiv f(m_2)(\mathrm{mod}\ S)$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: transformation correlated with equivalence}
Пусть на множестве $M$ определена эквивалентность $S$.
Пусть на множестве ${}^* M$ определена $\Omega_1$\Hyph алгебра.
Если любое преобразование $f\in{}^* M$ согласованно с эквивалентностью $S$,
то мы можем определить структуру $\Omega_1$\Hyph алгебры
на множестве ${}^*(M/S)$.
\end{theorem}
\begin{proof}
Пусть $h=\mathrm{nat}\ S$. Если
\ShowEq{m1 m2 modS},
то $h(m_1)=h(m_2)$. Поскольку
$f\in{}^* M$ согласованно с эквивалентностью $S$,
то $h(f(m_1))=h(f(m_2))$. Это позволяет определить
преобразование $F$ согласно правилу
\ShowEq{morphism of representations and equivalence, 0}

Пусть $\omega$ - n\Hyph арная операция $\Omega_1$\Hyph алгебры.
Пусть $f_1$, ..., $f_n\in{}^\star M$ и
\ShowEq{morphism of representations and equivalence}
Согласно условию теоремы, преобразование
\ShowEq{morphism of representations and equivalence, 1}
согласованно с эквивалентностью $S$.
Следовательно, из условия
\ShowEq{m1 m2 modS}
и определения
\ref{definition: transformation coordinated with equivalence}
следует
\ShowEq{morphism of representations and equivalence, 2}
Следовательно, мы можем определить операцию $\omega$ на множестве ${}^\star(M/S)$ по правилу
\ShowEq{morphism of representations and equivalence, 3}
Из определения
\EqRef{morphism of representations and equivalence, 0}
и равенства
\EqRef{morphism of representations and equivalence, 2}
следует, что мы корректно определили
операцию $\omega$ на множестве ${}^\star(M/S)$.
\end{proof}

\begin{theorem}
\label{theorem: decompositions of morphism of representations}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$,
\ShowEq{g:B->*N}
представление $\Omega_1$\Hyph алгебры $B$.
Пусть
\[
\xymatrix{
r:A\ar[r]&B&R:M\ar[r]&N
}
\]
морфизм представлений из $f$ в $g$.
Положим
\begin{align*}
s&=rr^{-1}&S&=RR^{-1}
\end{align*}
Тогда для отображений $r$, $R$ существуют разложения,
которые можно описать диаграммой
\ShowEq{decompositions of morphism of representations, diagram}
\begin{enumerate}
\item $s=\mathrm{ker}\ r$ является конгруэнцией на $A$.
Существует разложение гомоморфизма $r$
\ShowEq{morphism of representations of algebra, homomorphism, 1}
$j=\mathrm{nat}\ s$ - естественный гомоморфизм
\ePrints{8443-0072}
\ifx\Semafor\ValueOff
\ShowEq{morphism of representations of algebra, homomorphism, 2}
\else
\newline
\fi
$t$ - изоморфизм
\ShowEq{morphism of representations of algebra, homomorphism, 3}
$i$ - вложение
\ShowEq{morphism of representations of algebra, homomorphism, 4}
\item $S=\mathrm{ker}\ R$ является эквивалентностью на $M$.
Существует разложение отображения $R$
\begin{equation}
R=ITJ
\EqLabel{morphism of representations of algebra, map, 1}
\end{equation}
$J=\mathrm{nat}\ S$ - сюръекция
\ePrints{8443-0072}
\ifx\Semafor\ValueOff
\ShowEq{morphism of representations of algebra, map, 2}
\else
\newline
\fi
$T$ - биекция
\ShowEq{morphism of representations of algebra, map, 3}
$I$ - вложение
\ShowEq{morphism of representations of algebra, map, 4}
\item $F$ - левостороннее представление $\Omega_1$\Hyph алгебры $A/s$ в $M/S$
\item $G$ - левостороннее представление $\Omega_1$\Hyph алгебры $rA$ в $RM$
\item $(j,J)$ - морфизм представлений $f$ и $F$
\label{theorem: (j,J) is morphism of representations}
\item $(t,T)$ - морфизм представлений $F$ и $G$
\label{theorem: (t,T) is morphism of representations}
\item $(t^{-1},T^{-1})$ - морфизм представлений $G$ и $F$
\label{theorem: (t-1,T-1) is morphism of representations}
\item $(i,I)$ - морфизм представлений $G$ и $g$
\label{theorem: (i,I) is morphism of representations}
\item Существует разложение морфизма представлений
\ShowEq{decompositions of morphism of representations}
\label{theorem: exists decompositions of morphism of representations}
\end{enumerate} 
\end{theorem}
\begin{proof}
Существование диаграмм $(1)$ и $(2)$ следует из теоремы II.3.7
(\citeBib{Cohn: Universal Algebra}, с. 74).
%Существование диаграммы $(2)$ следует из теоремы I.3.1
%(\citeBib{Cohn: Universal Algebra}, с. 28).

Мы начнём с диаграммы $(4)$.

Пусть $m_1\equiv m_2(\mathrm{mod}\ S)$.
%Тогда $J(m_1)=J(m_2)$,
Следовательно,
\ShowEq{morphism of representations of algebra, (4), 1}
%$JT(m_1)=JT(m_2)$,
%так как $JT$ - отображение на $MR$.
Если $a_1\equiv a_2(\mathrm{mod}\ s)$, то
\ShowEq{morphism of representations of algebra, (4), 2}
Следовательно,
$j(a_1)=j(a_2)$.
Так как $(r,R)$ - морфизм представлений, то
\ShowEq{morphism of representations of algebra, (4), 3 4}
Из \EqRef{morphism of representations of algebra, (4), 1},
\EqRef{morphism of representations of algebra, (4), 2},
\EqRef{morphism of representations of algebra, (4), 3},
\EqRef{morphism of representations of algebra, (4), 4}
следует
\ShowEq{morphism of representations of algebra, (4), 5}
Из \EqRef{morphism of representations of algebra, (4), 5}
следует
\begin{equation}
f(a_1)(m_1)\equiv f(a_2)(m_2)(\mathrm{mod}\ S)
\EqLabel{morphism of representations of algebra, (4), 6}
\end{equation}
и, следовательно,
\ShowEq{morphism of representations of algebra, (4), 7}
Из \EqRef{morphism of representations of algebra, (4), 7}
следует, что отображение
\ShowEq{morphism of representations of algebra, (4), 8}
определено корректно и является преобразованием множества $M/S$.

Из равенства
\EqRef{morphism of representations of algebra, (4), 6}
(в случае $a_1=a_2$) следует, что для любого $a$ преобразование
согласованно с эквивалентностью $S$.
Из теоремы
\ref{theorem: transformation correlated with equivalence} следует,
что на множестве ${}^*(M/S)$ определена структура $\Omega_1$\Hyph алгебры.
Рассмотрим $n$\Hyph арную операцию $\omega$ и $n$
преобразований
\ShowEq{transformation correlated with equivalence, 1}
пространства $M/S$. Мы положим
\ShowEq{morphism of representations of algebra, (4), 9}
Следовательно, отображение $F$ является представлением
$\Omega_1$\Hyph алгебры $A/s$.

Из \EqRef{morphism of representations of algebra, (4), 8}
следует, что $(j,J)$ является морфизмом представлений $f$ и $F$
(утверждение \eqref{theorem: (j,J) is morphism of representations}
теоремы).

Рассмотрим диаграмму $(5)$.

Так как $T$ - биекция, то мы можем отождествить элементы множества
$M/S$ и множества $MR$, причём это отождествление имеет вид
\ShowEq{morphism of representations of algebra, (5), 1}
Мы можем записать преобразование $F(\RedText{j(a)})$
множества $M/S$ в виде
\ShowEq{morphism of representations of algebra, (5), 2}
Так как $T$ - биекция, то мы можем определить преобразование
\ShowEq{morphism of representations of algebra, (5), 3}
множества $RM$. Преобразование
\EqRef{morphism of representations of algebra, (5), 3}
зависит от $\RedText{j(a)}\in A/s$.
Так как $t$ - биекция, то мы можем отождествить элементы множества
$A/s$ и множества $rA$, причём это отождествление имеет вид
\ShowEq{morphism of representations of algebra, (5), 6}
Следовательно, мы определили отображение
\[
G:rA\rightarrow{}^\star RM
\]
согласно равенству
\ShowEq{morphism of representations of algebra, (5), 4}

Рассмотрим $n$\Hyph арную операцию $\omega$ и $n$
преобразований
\ShowEq{morphism of representations of algebra, (5), 7}
пространства $RM$. Мы положим
\ShowEq{morphism of representations of algebra, (5), 5}
Согласно \EqRef{morphism of representations of algebra, (5), 4}
операция $\omega$ корректно определена на множестве ${}^\star RM$.
Следовательно, отображение $G$ является представлением
$\Omega_1$\Hyph алгебры.

Из \EqRef{morphism of representations of algebra, (5), 4}
следует, что $(t,T)$ является морфизмом представлений $F$ и $G$
(утверждение \eqref{theorem: (t,T) is morphism of representations}
теоремы).

Так как $T$ - биекция, то из равенства
\EqRef{morphism of representations of algebra, (5), 1}
следует
\ShowEq{morphism of representations of algebra, (5), 1a}
Мы можем записать преобразование $G(\RedText{r(a)})$
множества $RM$ в виде
\ShowEq{morphism of representations of algebra, (5), 2a}
Так как $T$ - биекция, то мы можем определить преобразование
\ShowEq{morphism of representations of algebra, (5), 3a}
множества $M/S$. Преобразование
\EqRef{morphism of representations of algebra, (5), 3a}
зависит от $\RedText{r(a)}\in rA$.
Так как $t$ - биекция, то из равенства
\EqRef{morphism of representations of algebra, (5), 6}
следует
\ShowEq{morphism of representations of algebra, (5), 6a}
Так как по построению диаграмма $(5)$ коммутативна, то преобразование
\EqRef{morphism of representations of algebra, (5), 3a}
совпадает с преобразованием
\EqRef{morphism of representations of algebra, (5), 2}.
Равенство
\EqRef{morphism of representations of algebra, (5), 5}
можно записать в виде
\ShowEq{morphism of representations of algebra, (5), 5a}
Следовательно, $(t^{-1},T^{-1})$ является морфизмом представлений $G$ и $F$
(утверждение \eqref{theorem: (t-1,T-1) is morphism of representations}
теоремы).

Диаграмма $(6)$ является самым простым случаем в нашем доказательстве.
Поскольку отображение $I$ является вложением и диаграмма $(2)$
коммутативна, мы можем отождествить $n\in N$ и $\BlueText{R(m)}$,
если $n\in\textrm{Im}R$. Аналогично, мы можем отождествить
соответствующие преобразования.
\ShowEq{morphism of representations of algebra, (6), 1}
Следовательно,
$(i,I)$ является морфизмом представлений $G$ и $g$
(утверждение \eqref{theorem: (i,I) is morphism of representations}
теоремы).

Для доказательства утверждения
\eqref{theorem: exists decompositions of morphism of representations}
теоремы осталось показать, что определённое
в процессе доказательства представление $g'$ совпадает
с представлением $g$, а операции над преобразованиями совпадают
с соответствующими операциями на ${}^* N$.
\ShowEq{morphism of representations of algebra, (6), 2}
\end{proof}

\begin{definition}
\label{definition: isomorphism of repesentations of Omega algebra}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$,
\ShowEq{g:B->*N}
представление $\Omega_1$\Hyph алгебры $B$.
Пусть
\[
\xymatrix{
r:A\ar[r]&B&R:M\ar[r]&N
}
\]
морфизм представлений из $r$ в $R$ такой, что
$f$ - изоморфизм $\Omega_1$\Hyph алгебры и $g$
- изоморфизм $\Omega_2$\Hyph алгебры.
Тогда отображение $(r,R)$ называется
\AddIndex{изоморфизмом представлений}
{isomorphism of repesentations of Omega algebra}.
\qed
\end{definition}

\begin{theorem}
В разложении
\EqRef{decompositions of morphism of representations}
отображение $(t,T)$ является изоморфизмом представлений $F$ и $G$.
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: isomorphism of repesentations of Omega algebra}
и утверждений \eqref{theorem: (t,T) is morphism of representations}
и \eqref{theorem: (t-1,T-1) is morphism of representations}
теоремы \ref{theorem: decompositions of morphism of representations}.
\end{proof}

\section{Приведенный морфизм представлений}

Из теоремы \ref{theorem: decompositions of morphism of representations}
следует, что мы можем свести задачу изучения морфизма представлений
$\Omega_1$\Hyph алгебры
к случаю, описываемому диаграммой
\ShowEq{morphism of representations of algebra, reduce, 1}

\begin{theorem}
\label{theorem: morphism of representations of algebra, reduce}
Диаграмма \EqRef{morphism of representations of algebra, reduce, 1}
может быть дополнена представлением $F_1$
$\Omega_1$\Hyph алгебры $A$ в множестве $M/S$ так,
что диаграмма
\ShowEq{morphism of representations of algebra, reduce, 2}
коммутативна. При этом множество преобразований представления $F$ и
множество преобразований представления $F_1$ совпадают.
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно положить
\[F_1(a)=F(\RedText{j(a)})\]
Так как отображение $j$ - сюрьекция, то $\mathrm{Im}F_1=\mathrm{Im}F$.
Так как $j$ и $F$ - гомоморфизмы $\Omega_1$\Hyph алгебры, то $F_1$
- также гомоморфизм $\Omega_1$\Hyph алгебры.
\end{proof}

\begin{remark}
\label{remark: reduced morphism of representations}
Теорема \ref{theorem: morphism of representations of algebra, reduce}
завершает цикл теорем, посвящённых структуре морфизма представлений
$\Omega_1$\Hyph алгебры.
Из этих теорем следует, что мы можем упростить задачу
изучения морфизма представлений
$\Omega_1$\Hyph алгебры и ограничиться морфизмом представлений вида
\[
\xymatrix{
id:A\ar[r]&A&R:M\ar[r]&N
}
\]
В этом случае мы можем отождествить морфизм $(\id,R)$ представлений
$\Omega_1$\Hyph алгебры и соответствующий гомоморфизм $R$ $\Omega_2$\Hyph алгебры
и будем называть гомоморфизм $R$
\AddIndex{приведенным морфизмом представлений}
{reduced morphism of representations}.
Мы будем пользоваться диаграммой
\ShowEq{morphism id,R of representations}
для представления приведенного морфизма $R$ представлений
$\Omega_1$\Hyph алгебры.
Из диаграммы следует
\ShowEq{morphism of representations of F algebra}
\qed
\end{remark}

\begin{theorem}
\label{theorem: reduced morphism of representations and homomorphism of algebra}
Пусть отображение
\ShowEq{H:M->N}
является приведенным морфизмом из представления
\ShowEq{f:A->*M}
$\Omega_1$\Hyph алгебры $A$ в представление
\ShowEq{g:A->*N}
$\Omega_1$\Hyph алгебры $A$.
Если представление $f$ эффективно, то отображение
\[
{}^*H:{}^* M\rightarrow{}^* N
\]
определённое равенством
\ShowEq{reduced morphism of representations, star morphism}
является гомоморфизмом $\Omega_1$\Hyph алгебры.
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: morphism of representations and homomorphism of algebra},
если мы положим
$h=id$.
\end{proof}

\begin{theorem}
\label{theorem: reduced morphism of representations of F algebra}
Пусть представления
\ShowEq{f:A->*M}
\ShowEq{g:A->*N}
$\Omega_1$\Hyph алгебры $A$ однотранзитивны.
Существует приведенный морфизм
представлений из $f$ в $g$
\ShowEq{H:M->N}
\end{theorem}
\begin{proof}
Выберем гомоморфизм $h$.
Выберем элемент $m\in M$
и элемент $n\in N$. 
Чтобы построить отображение $H$, рассмотрим следующую диаграмму
\ShowEq{reduced morphism representation H, diagram}
Из коммутативности диаграммы $(1)$ следует
\ShowEq{reduced morphism representation =}
Для произвольного $m'\in M$ однозначно определён $a\in A$ такой, что
\ShowEq{m'=.m}
Следовательно, мы построили отображении $H$,
которое удовлетворяет равенству
\EqRef{morphism of representations of F algebra}.
\end{proof}

\begin{theorem}
\label{theorem: unique reduced morphism of representations of F algebra}
Пусть представления
\ShowEq{f:A->*M}
\ShowEq{g:A->*N}
$\Omega_1$\Hyph алгебры $A$ однотранзитивны.
Приведенный морфизм представлений из $f$ в $g$
\[
\xymatrix{
H:M\ar[r]&N
}
\]
определён однозначно
с точностью до выбора образа $n=H(m)\in N$
заданного элемента $m\in M$.
\end{theorem}
\begin{proof}
Из доказательства теоремы
\ref{theorem: reduced morphism of representations of F algebra}
следует, что выбор элементов
$m\in M$, $n\in N$ однозначно определяет отображение $H$.
\end{proof}

Мы дадим следующее определение
по аналогии с определением
\ref{definition: category of representations of F algebra from category}.

\begin{definition}
\label{definition: category of left-side representations of Omega1 algebra}
Мы определим \AddIndex{категорию
\symb{A*}{category of left-side representations of Omega1 algebra}1
$\ $ левосторонних представлений $\Omega_1$\Hyph алгебры $A$}
{category of left-side representations of Omega1 algebra}.
Объектами этой категории являются
левосторонними представлениями $\Omega_1$\Hyph алгебры $A$.
Морфизмами этой категории являются морфизмы $(id,R)$
левосторонних представлений $\Omega_1$\Hyph алгебры $A$.
\qed
\end{definition}

\section{Автоморфизм представления универсальной алгебры}

\begin{definition}
\label{definition: endomorphism of representation of F algebra}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Приведенный морфизм представлений $\Omega_1$\Hyph алгебры
\ShowEq{morphism of representation of A in M}
такой, что $R$ - эндоморфизм $\Omega_2$\Hyph алгебры
называется
\AddIndex{эндоморфизмом представления}
{endomorphism of representation} $f$.
\qed
\end{definition}

\begin{theorem}
Если представление
\ShowEq{f:A->*M}
$\Omega_1$\Hyph алгебры $A$ однотранзитивно,
то для любых $p$, $q\in M$ существует единственный эндоморфизм
\ShowEq{endomorphism representation H}
представления $f$
такой, что $H(p)=q$.
\end{theorem}
\begin{proof}
Рассмотрим следующую диаграмму
\ShowEq{endomorphism representation H diagram}
Существование эндоморфизма является следствием теоремы
\ref{theorem: morphism of representations of F algebra}.
Единственность эндоморфизма для заданных $p$, $q\in M$
является следствием теоремы
\ref{theorem: unique morphism of representations of F algebra},
когда $h=\id$.
\end{proof}

\begin{theorem}
Эндоморфизмы представления $f$ порождают полугруппу.
\end{theorem}
\begin{proof}
Из теоремы
\ref{theorem: product of morphisms of representations of F algebra}
следует, что произведение эндоморфизмов $(p,P)$, $(r,R)$ представления $f$
является эндоморфизмом $(pr,PR)$ представления $f$.
\end{proof}

\begin{definition}
\label{definition: automorphism of representation of F algebra}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Морфизм представлений $\Omega_1$\Hyph алгебры
\ShowEq{morphism of representation of A in M}
такой, что $R$ - автоморфизм $\Omega_2$\Hyph алгебры
называется
\AddIndex{автоморфизмом представления}
{automorphism of representation} $f$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: group of automorphisms of representation}
Пусть
\ShowEq{f:A->*M}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Множество автоморфизмов представления $f$
порождает \AddIndex{группу}{group of automorphisms of representation}
\ShowEq{group of automorphisms of representation}.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{automorphisms R P}
- автоморфизмы представления $f$.
Согласно определению
\ref{definition: automorphism of representation of F algebra},
отображения $R$, $P$
являются автоморфизмами
$\Omega_2$\Hyph алгебры $M$.
Согласно теореме II.3.2,
(\citeBib{Cohn: Universal Algebra}, c. 60),
отображение $R\circ P$
является автоморфизмом
$\Omega_2$\Hyph алгебры $M$.
Из теоремы
\ref{theorem: product of morphisms of representations of F algebra}
и определения
\ref{definition: automorphism of representation of F algebra}
следует, что произведение автоморфизмов
$R\circ P$ представления $f$ является автоморфизмом представления $f$.

Пусть
\ShowEq{automorphisms R P Q}
- автоморфизмы представления $f$.
Из цепочки равенств
\ShowEq{associativity of product of automorphisms of representation}
следует ассоциативность произведения для отображений $R$, $P$, $Q$.\footnote{При
доказательстве ассоциативности произведения
я следую примеру полугруппы
из \citeBib{Kurosh: General Algebra}, с. 20, 21.}

Пусть $R$ - автоморфизм представления $f$.
Согласно определению
\ref{definition: automorphism of representation of F algebra}
отображение $R$
является автоморфизмом
$\Omega_2$\Hyph алгебры $M$.
Следовательно, отображение $R^{-1}$
является автоморфизмом
$\Omega_2$\Hyph алгебры $M$.
Для автоморфизма $R$ представления справедливо равенство
\EqRef{morphism of representations of F algebra, definition, 2m}.
Положим $m'=R(m)$. Так как $R$ - автоморфизм $\Omega_2$\Hyph алгебры,
то $m=R^{-1}(m')$
и равенство
\EqRef{morphism of representations of F algebra, definition, 2m}
можно записать в виде
\ShowEq{morphism of representations of F algebra, definition, 2m-1}
Так как отображение $R$
является автоморфизмом
$\Omega_2$\Hyph алгебры $M$,
то из равенства
\EqRef{morphism of representations of F algebra, definition, 2m-1}
следует
\ShowEq{morphism of representations of F algebra, definition, 2m-1, 1}
Равенство
\EqRef{morphism of representations of F algebra, definition, 2m-1, 1}
соответствует равенству
\EqRef{morphism of representations of F algebra, definition, 2m}
для отображения $R^{-1}$.
Следовательно, отображение $R^{-1}$ является автоморфизмом
представления $f$.
\end{proof}

\ePrints{4993-2400,0701.238,0906.0135}
\ifx\Semafor\ValueOff
\section{Примеры представления универсальной алгебры}

\subsection{Векторное пространство}
\label{subsection: Vector Space}
\ePrints{0912.3315}
\ifx\Semafor\ValueOn
Согласно определениям
\xRef{0701.238}{definition: Tstar vector space},
\xRef{4776-3181}{definition: Tstar vector space},
эффективное левостороннее представление тела $D$ в абелевой группе
называется
\AddIndex{левым $D$\hyph векторным пространством}{left vector space}.
\else
Согласно определениям
\ref{definition: vector space 1},
\ref{definition: vector space 2},
эффективное представление поля $D$ в абелевой группе
называется
\AddIndex{векторным пространством над полем}{vector space over field} $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D-vector space}.
\fi
Аналогично эффективное представление ассоциативного кольца $R$
в абелевой группе называется \AddIndex{модулем над кольцом}{module over ring} $R$
или \AddIndex{$R$\Hyph модулем}{R- module}.

\subsection{Представление группы на множестве}
\label{subsection: representation of group on the set}
Пусть $G$ - абелевая группа, и $M$ - множество.
Рассмотрим эфективное представление группы $G$ на множестве $M$.
Для заданных $a\in G$, $A\in M$ положим
$A\rightarrow A+a$.
Мы будем также пользоваться
записью $a=\overset{\rightarrow}{AB}$, если
\ShowEq{representation of group on the set, 1}
Тогда действие группы можно представить в виде
\ShowEq{representation of group on the set, 2}
Поскольку представление эффективно, то из равенств
\EqRef{representation of group on the set, 1},
\EqRef{representation of group on the set, 2}
и равенства
\ShowEq{representation of group on the set, 3}
следует, что
\ShowEq{representation of group on the set, 4}
\fi
\else %4776-3181

Я рассматриваю
представление универсальной алгебры в книге
\citeBib{0912.3315}.
В этой главе я рассматриваю представление групп.
В главе
\ref{chapter: Vector Space Over Division Ring}
я рассматриваю представление тела в абелевой группе.
\fi

